HATNet Field G205: Follow-Up Observations of 28 Transiting-Planet candidates and Confirmation of the Planet HAT-P-8b

We report the identification of 32 transiting-planet candidates in HATNet field G205. We describe the procedures that we have used to follow up these candidates with spectroscopic and photometric observations, and we present a status report on our interpretation of the 28 candidates for which we have follow-up observations. Eight are eclipsing binaries with orbital solutions whose periods are consistent with their photometric ephemerides; two of these spectroscopic orbits are singled-lined and six are double-lined. For one of the candidates, a nearby but fainter eclipsing binary proved to be the source for the HATNet light curve, due to blending in the HATNet images. Four of the candidates were found to be rotating more rapidly than vsini = 50 km/s and were not pursued further. Thirteen of the candidates showed no significant velocity variation at the level of 0.5 to 1.0 km/s . Seven of these were eventually withdrawn as photometric false alarms based on an independent reanalysis using more sophisticated tools. Of the remaining six, one was put aside because a close visual companion proved to be a spectroscopic binary, and two were not followed up because the host stars were judged to be too large. Two of the remaining candidates are members of a visual binary, one of which was previously confirmed as the first HATNet transiting planet, HAT-P-1b. In this paper we confirm that the last of this set of candidates is also a a transiting planet, which we designate HAT-P-8b, with mass Mp = 1.52 +/- 0.18/0.16 Mjup, radius Rp = 1.50 +/- 0.08/0.06 Rjup, and photometric period P = 3.076320 +/- 0.000004 days. HAT-P-8b has an inflated radius for its mass, and a large mass for its period. The host star is a solar-metallicity F dwarf, with mass M* = 1.28 +/- 0.04 Msun and Rp = 1.58 +/- 0.08/0.06 Rsun.

==> tab10.tex <==
\begin{deluxetable}{ccc}
\tablewidth{0pc}
\tablenum{10}\tablecaption{KeplerCam Photometry for HTR205-024}
\tablehead{
\colhead{BJD} &
\colhead{Mag} &
\colhead{Error}}
\startdata
2454403.69847 &$ 0.00311 $&  0.00101 \\
2454403.69883 &$ 0.00133 $&  0.00104 \\
2454403.69916 &$ 0.00580 $&  0.00107 \\
2454403.69949 &$ 0.00011 $&  0.00103 \\
2454403.69984 &$-0.01672 $&  0.00111 \\
2454403.70019 &$-0.00314 $&  0.00104 \\
2454403.70050 &$ 0.00075 $&  0.00105 \\
2454403.70086 &$ 0.00257 $&  0.00105 \\
2454403.70118 &$ 0.00124 $&  0.00109 \\
2454403.70152 &$-0.00116 $&  0.00111 \\
2454403.70185 &$-0.00138 $&  0.00104 \\
2454403.70215 &$ 0.00049 $&  0.00105 \\
2454403.70249 &$ 0.00149 $&  0.00108 \\
2454403.70282 &$-0.00273 $&  0.00111 \\
2454403.70314 &$-0.00024 $&  0.00113 \\
2454403.70347 &$ 0.00932 $&  0.00119 \\
2454403.70377 &$-0.00055 $&  0.00120 \\
2454403.70411 &$-0.00021 $&  0.00116 \\
2454403.70445 &$ 0.00228 $&  0.00113 \\
2454403.70478 &$ 0.00158 $&  0.00114 \\
2454403.70510 &$ 0.00074 $&  0.00120 \\
2454403.70544 &$ 0.00237 $&  0.00124 \\
2454403.70576 &$-0.01014 $&  0.00127 \\
2454403.70610 &$ 0.00622 $&  0.00126 \\
2454403.70645 &$-0.00137 $&  0.00111 \\
2454403.70677 &$ 0.00112 $&  0.00108 \\
2454403.70710 &$ 0.00016 $&  0.00104 \\
2454403.70744 &$ 0.00240 $&  0.00104 \\
2454403.70777 &$ 0.00411 $&  0.00103 \\
2454403.70810 &$ 0.00248 $&  0.00103 \\
2454403.70843 &$ 0.00135 $&  0.00103 \\
2454403.70875 &$-0.00337 $&  0.00102 \\
2454403.70909 &$-0.00116 $&  0.00101 \\
2454403.70942 &$-0.00176 $&  0.00100 \\
2454403.70976 &$-0.00094 $&  0.00100 \\
2454403.71008 &$-0.00086 $&  0.00099 \\
2454403.71041 &$ 0.00235 $&  0.00099 \\
2454403.71074 &$-0.00027 $&  0.00099 \\
2454403.71107 &$-0.00043 $&  0.00100 \\
2454403.71140 &$-0.00083 $&  0.00100 \\
2454403.71173 &$ 0.00021 $&  0.00099 \\
2454403.71207 &$-0.00031 $&  0.00099 \\
2454403.71238 &$-0.00078 $&  0.00100 \\
2454403.71273 &$-0.00047 $&  0.00099 \\
2454403.71307 &$ 0.00242 $&  0.00100 \\
2454403.71338 &$-0.00255 $&  0.00101 \\
2454403.71370 &$ 0.00127 $&  0.00098 \\
2454403.71404 &$ 0.00161 $&  0.00098 \\
2454403.71436 &$ 0.00251 $&  0.00099 \\
2454403.71468 &$-0.00100 $&  0.00101 \\
2454403.71502 &$ 0.00869 $&  0.00113 \\
2454403.71536 &$ 0.00731 $&  0.00115 \\
2454403.71570 &$-0.00353 $&  0.00119 \\
2454403.71602 &$-0.00694 $&  0.00107 \\
2454403.71635 &$-0.00538 $&  0.00099 \\
2454403.71668 &$-0.00283 $&  0.00099 \\
2454403.71700 &$ 0.00039 $&  0.00101 \\
2454403.71735 &$-0.00176 $&  0.00100 \\
2454403.71766 &$-0.00017 $&  0.00099 \\
2454403.71800 &$-0.00272 $&  0.00098 \\
2454403.71832 &$ 0.00031 $&  0.00099 \\
2454403.71866 &$ 0.00052 $&  0.00099 \\
2454403.71899 &$ 0.00068 $&  0.00098 \\
2454403.71934 &$ 0.00530 $&  0.00099 \\
2454403.71969 &$-0.00040 $&  0.00098 \\
2454403.72003 &$ 0.00152 $&  0.00099 \\
2454403.72036 &$ 0.00266 $&  0.00099 \\
2454403.72070 &$-0.00469 $&  0.00099 \\
2454403.72103 &$ 0.00142 $&  0.00098 \\
2454403.72137 &$-0.00217 $&  0.00099 \\
2454403.72169 &$-0.00098 $&  0.00099 \\
2454403.72204 &$-0.00024 $&  0.00099 \\
2454403.72237 &$ 0.00215 $&  0.00099 \\
2454403.72267 &$-0.00158 $&  0.00100 \\
2454403.72302 &$ 0.00188 $&  0.00099 \\
2454403.72334 &$ 0.00074 $&  0.00099 \\
2454403.72367 &$ 0.00078 $&  0.00098 \\
2454403.72400 &$ 0.00013 $&  0.00098 \\
2454403.72433 &$-0.00061 $&  0.00098 \\
2454403.72466 &$ 0.00028 $&  0.00098 \\
2454403.72500 &$-0.00043 $&  0.00098 \\
2454403.72531 &$ 0.00095 $&  0.00099 \\
2454403.72565 &$ 0.00056 $&  0.00099 \\
2454403.72597 &$ 0.00354 $&  0.00100 \\
2454403.72632 &$ 0.00164 $&  0.00100 \\
2454403.72664 &$ 0.00266 $&  0.00107 \\
2454403.72698 &$-0.00036 $&  0.00109 \\
2454403.72731 &$ 0.00035 $&  0.00111 \\
2454403.72766 &$-0.00184 $&  0.00116 \\
2454403.72799 &$-0.00085 $&  0.00113 \\
2454403.72832 &$-0.00703 $&  0.00110 \\
2454403.72866 &$ 0.00224 $&  0.00105 \\
2454403.72900 &$ 0.00087 $&  0.00105 \\
2454403.72933 &$-0.00312 $&  0.00108 \\
2454403.72968 &$-0.00192 $&  0.00104 \\
2454403.73001 &$ 0.00043 $&  0.00105 \\
2454403.73035 &$ 0.00006 $&  0.00114 \\
2454403.73068 &$ 0.01047 $&  0.00124 \\
2454403.73100 &$ 0.00252 $&  0.00114 \\
2454403.73133 &$ 0.00155 $&  0.00106 \\
2454403.73167 &$ 0.00009 $&  0.00104 \\
2454403.73198 &$-0.00037 $&  0.00103 \\
2454403.73230 &$ 0.00183 $&  0.00103 \\
2454403.73265 &$ 0.00101 $&  0.00102 \\
2454403.73299 &$ 0.00090 $&  0.00100 \\
2454403.73333 &$ 0.00260 $&  0.00101 \\
2454403.73367 &$ 0.00198 $&  0.00100 \\
2454403.73399 &$-0.00140 $&  0.00103 \\
2454403.73433 &$-0.00168 $&  0.00101 \\
2454403.73468 &$-0.00099 $&  0.00099 \\
2454403.73501 &$-0.00244 $&  0.00098 \\
2454403.73536 &$ 0.00169 $&  0.00098 \\
2454403.73569 &$ 0.00010 $&  0.00097 \\
2454403.73603 &$ 0.00202 $&  0.00097 \\
2454403.73634 &$ 0.00100 $&  0.00097 \\
2454403.73668 &$ 0.00203 $&  0.00098 \\
2454403.73701 &$ 0.00061 $&  0.00097 \\
2454403.73734 &$ 0.00250 $&  0.00097 \\
2454403.73766 &$-0.00097 $&  0.00097 \\
2454403.73800 &$ 0.00218 $&  0.00097 \\
2454403.73830 &$-0.00034 $&  0.00097 \\
2454403.73863 &$-0.00231 $&  0.00097 \\
2454403.73896 &$ 0.00206 $&  0.00097 \\
2454403.73928 &$ 0.00216 $&  0.00097 \\
2454403.73961 &$-0.00230 $&  0.00097 \\
2454403.73994 &$-0.00308 $&  0.00097 \\
2454403.74030 &$ 0.00053 $&  0.00097 \\
2454403.74064 &$-0.00390 $&  0.00097 \\
2454403.74097 &$-0.00040 $&  0.00097 \\
2454403.74127 &$ 0.00035 $&  0.00097 \\
2454403.74161 &$-0.00075 $&  0.00097 \\
2454403.74195 &$-0.00208 $&  0.00097 \\
2454403.74229 &$ 0.00032 $&  0.00097 \\
2454403.74263 &$ 0.00112 $&  0.00097 \\
2454403.74293 &$-0.00024 $&  0.00097 \\
2454403.74327 &$-0.00230 $&  0.00097 \\
2454403.74360 &$-0.00008 $&  0.00097 \\
2454403.74393 &$-0.00055 $&  0.00097 \\
2454403.74426 &$ 0.00000 $&  0.00097 \\
2454403.74459 &$-0.00172 $&  0.00097 \\
2454403.74494 &$-0.00253 $&  0.00097 \\
2454403.74528 &$-0.00106 $&  0.00097 \\
2454403.74559 &$-0.00260 $&  0.00097 \\
2454403.74592 &$-0.00143 $&  0.00097 \\
2454403.74625 &$-0.00117 $&  0.00097 \\
2454403.74658 &$-0.00214 $&  0.00097 \\
2454403.74691 &$-0.00108 $&  0.00097 \\
2454403.74723 &$-0.00232 $&  0.00097 \\
2454403.74759 &$-0.00209 $&  0.00097 \\
2454403.74792 &$ 0.00261 $&  0.00097 \\
2454403.74826 &$-0.00406 $&  0.00097 \\
2454403.74860 &$ 0.00223 $&  0.00097 \\
2454403.74895 &$ 0.00137 $&  0.00097 \\
2454403.74928 &$-0.00320 $&  0.00097 \\
2454403.74963 &$ 0.00179 $&  0.00097 \\
2454403.74998 &$-0.00399 $&  0.00096 \\
2454403.75032 &$ 0.00012 $&  0.00097 \\
2454403.75066 &$-0.00187 $&  0.00097 \\
2454403.75101 &$-0.00159 $&  0.00096 \\
2454403.75133 &$ 0.00025 $&  0.00097 \\
2454403.75168 &$ 0.00124 $&  0.00097 \\
2454403.75201 &$ 0.00144 $&  0.00097 \\
2454403.75234 &$ 0.00289 $&  0.00097 \\
2454403.75266 &$ 0.00220 $&  0.00098 \\
2454403.75300 &$ 0.00036 $&  0.00097 \\
2454403.75333 &$-0.00063 $&  0.00097 \\
2454403.75367 &$-0.00006 $&  0.00096 \\
2454403.75399 &$-0.00069 $&  0.00097 \\
2454403.75430 &$-0.00040 $&  0.00097 \\
2454403.75464 &$ 0.00246 $&  0.00097 \\
2454403.75498 &$-0.00133 $&  0.00097 \\
2454403.75531 &$-0.00103 $&  0.00097 \\
2454403.75562 &$ 0.00239 $&  0.00097 \\
2454403.75597 &$ 0.00147 $&  0.00097 \\
2454403.75631 &$ 0.00364 $&  0.00098 \\
2454403.75665 &$ 0.00029 $&  0.00097 \\
2454403.75699 &$ 0.00285 $&  0.00097 \\
2454403.75734 &$ 0.00430 $&  0.00097 \\
2454403.75767 &$ 0.00503 $&  0.00097 \\
2454403.75803 &$ 0.00043 $&  0.00098 \\
2454403.75834 &$ 0.00347 $&  0.00097 \\
2454403.75868 &$ 0.00597 $&  0.00098 \\
2454403.75900 &$ 0.00331 $&  0.00097 \\
2454403.75934 &$ 0.00490 $&  0.00097 \\
2454403.75967 &$ 0.00535 $&  0.00097 \\
2454403.76000 &$ 0.00604 $&  0.00097 \\
2454403.76033 &$ 0.00766 $&  0.00097 \\
2454403.76067 &$ 0.00373 $&  0.00098 \\
2454403.76101 &$ 0.00520 $&  0.00097 \\
2454403.76134 &$ 0.00041 $&  0.00097 \\
2454403.76169 &$ 0.00466 $&  0.00097 \\
2454403.76202 &$ 0.00511 $&  0.00098 \\
2454403.76235 &$ 0.00469 $&  0.00098 \\
2454403.76268 &$ 0.00663 $&  0.00098 \\
2454403.76302 &$ 0.00254 $&  0.00098 \\
2454403.76337 &$ 0.00999 $&  0.00098 \\
2454403.76370 &$ 0.00714 $&  0.00098 \\
2454403.76404 &$ 0.00664 $&  0.00098 \\
2454403.76438 &$ 0.00967 $&  0.00098 \\
2454403.76472 &$ 0.00290 $&  0.00098 \\
2454403.76508 &$ 0.00730 $&  0.00098 \\
2454403.76539 &$ 0.00717 $&  0.00098 \\
2454403.76573 &$ 0.00494 $&  0.00097 \\
2454403.76606 &$ 0.01041 $&  0.00097 \\
2454403.76640 &$ 0.00696 $&  0.00098 \\
2454403.76672 &$ 0.01034 $&  0.00097 \\
2454403.76707 &$ 0.00633 $&  0.00097 \\
2454403.76739 &$ 0.00784 $&  0.00098 \\
2454403.76773 &$ 0.00664 $&  0.00098 \\
2454403.76805 &$ 0.00812 $&  0.00098 \\
2454403.76838 &$ 0.00618 $&  0.00097 \\
2454403.76875 &$ 0.00926 $&  0.00098 \\
2454403.76907 &$ 0.00857 $&  0.00097 \\
2454403.76941 &$ 0.00932 $&  0.00097 \\
2454403.76973 &$ 0.00986 $&  0.00097 \\
2454403.77007 &$ 0.00752 $&  0.00098 \\
2454403.77040 &$ 0.01073 $&  0.00098 \\
2454403.77075 &$ 0.00726 $&  0.00098 \\
2454403.77109 &$ 0.00744 $&  0.00097 \\
2454403.77141 &$ 0.00857 $&  0.00098 \\
2454403.77172 &$ 0.00789 $&  0.00098 \\
2454403.77206 &$ 0.00992 $&  0.00098 \\
2454403.77238 &$ 0.01084 $&  0.00098 \\
2454403.77273 &$ 0.00672 $&  0.00098 \\
2454403.77305 &$ 0.00934 $&  0.00098 \\
2454403.77337 &$ 0.00809 $&  0.00098 \\
2454403.77367 &$ 0.00831 $&  0.00098 \\
2454403.77401 &$ 0.00988 $&  0.00098 \\
2454403.77435 &$ 0.01000 $&  0.00098 \\
2454403.77467 &$ 0.01365 $&  0.00098 \\
2454403.77501 &$ 0.00857 $&  0.00097 \\
2454403.77534 &$ 0.00612 $&  0.00098 \\
2454403.77569 &$ 0.00946 $&  0.00098 \\
2454403.77600 &$ 0.00845 $&  0.00098 \\
2454403.77635 &$ 0.01088 $&  0.00098 \\
2454403.77668 &$ 0.00578 $&  0.00098 \\
2454403.77698 &$ 0.00857 $&  0.00099 \\
2454403.77731 &$ 0.01079 $&  0.00098 \\
2454403.77766 &$ 0.01370 $&  0.00098 \\
2454403.77800 &$ 0.00803 $&  0.00099 \\
2454403.77833 &$ 0.01291 $&  0.00098 \\
2454403.77868 &$ 0.00870 $&  0.00098 \\
2454403.77901 &$ 0.00870 $&  0.00099 \\
2454403.77934 &$ 0.01162 $&  0.00098 \\
2454403.77967 &$ 0.00898 $&  0.00098 \\
2454403.78002 &$ 0.00970 $&  0.00098 \\
2454403.78034 &$ 0.01012 $&  0.00098 \\
2454403.78067 &$ 0.00886 $&  0.00098 \\
2454403.78099 &$ 0.01144 $&  0.00098 \\
2454403.78131 &$ 0.00754 $&  0.00098 \\
2454403.78163 &$ 0.00817 $&  0.00099 \\
2454403.78197 &$ 0.01187 $&  0.00099 \\
2454403.78229 &$ 0.00803 $&  0.00098 \\
2454403.78265 &$ 0.01042 $&  0.00099 \\
2454403.78298 &$ 0.00966 $&  0.00098 \\
2454403.78332 &$ 0.00952 $&  0.00098 \\
2454403.78369 &$ 0.01191 $&  0.00098 \\
2454403.78402 &$ 0.01118 $&  0.00098 \\
2454403.78437 &$ 0.00748 $&  0.00098 \\
2454403.78470 &$ 0.00908 $&  0.00098 \\
2454403.78503 &$ 0.00794 $&  0.00098 \\
2454403.78537 &$ 0.01135 $&  0.00098 \\
2454403.78570 &$ 0.00570 $&  0.00098 \\
2454403.78604 &$ 0.01194 $&  0.00098 \\
2454403.78637 &$ 0.01529 $&  0.00097 \\
2454403.78672 &$ 0.00743 $&  0.00097 \\
2454403.78706 &$ 0.01007 $&  0.00098 \\
2454403.78738 &$ 0.01149 $&  0.00098 \\
2454403.78772 &$ 0.00882 $&  0.00097 \\
2454403.78806 &$ 0.01409 $&  0.00098 \\
2454403.78840 &$ 0.01364 $&  0.00098 \\
2454403.78872 &$ 0.01278 $&  0.00098 \\
2454403.78905 &$ 0.01279 $&  0.00098 \\
2454403.78938 &$ 0.01143 $&  0.00097 \\
2454403.78973 &$ 0.01058 $&  0.00098 \\
2454403.79005 &$ 0.00911 $&  0.00097 \\
2454403.79037 &$ 0.01017 $&  0.00098 \\
2454403.79068 &$ 0.01094 $&  0.00097 \\
2454403.79099 &$ 0.01354 $&  0.00098 \\
2454403.79133 &$ 0.01215 $&  0.00098 \\
2454403.79166 &$ 0.01197 $&  0.00097 \\
2454403.79199 &$ 0.01054 $&  0.00098 \\
2454403.79231 &$ 0.01213 $&  0.00098 \\
2454403.79266 &$ 0.01141 $&  0.00097 \\
2454403.79299 &$ 0.01003 $&  0.00098 \\
2454403.79334 &$ 0.01047 $&  0.00097 \\
2454403.79367 &$ 0.01124 $&  0.00098 \\
2454403.79400 &$ 0.01043 $&  0.00097 \\
2454403.79433 &$ 0.01200 $&  0.00097 \\
2454403.79465 &$ 0.01388 $&  0.00098 \\
2454403.79499 &$ 0.01298 $&  0.00098 \\
2454403.79532 &$ 0.01345 $&  0.00098 \\
2454403.79568 &$ 0.01495 $&  0.00098 \\
2454403.79603 &$ 0.01077 $&  0.00098 \\
2454403.79634 &$ 0.01437 $&  0.00097 \\
2454403.79667 &$ 0.01363 $&  0.00098 \\
2454403.79699 &$ 0.00978 $&  0.00098 \\
2454403.79733 &$ 0.01398 $&  0.00098 \\
2454403.79767 &$ 0.01136 $&  0.00097 \\
2454403.79799 &$ 0.01624 $&  0.00098 \\
2454403.79834 &$ 0.01072 $&  0.00097 \\
2454403.79870 &$ 0.01092 $&  0.00097 \\
2454403.79904 &$ 0.01533 $&  0.00097 \\
2454403.79936 &$ 0.01109 $&  0.00098 \\
2454403.79972 &$ 0.01341 $&  0.00098 \\
2454403.80008 &$ 0.00977 $&  0.00098 \\
2454403.80041 &$ 0.01288 $&  0.00098 \\
2454403.80076 &$ 0.01174 $&  0.00098 \\
2454403.80110 &$ 0.00986 $&  0.00098 \\
2454403.80147 &$ 0.00974 $&  0.00098 \\
2454403.80178 &$ 0.00495 $&  0.00098 \\
2454403.80210 &$ 0.01259 $&  0.00098 \\
2454403.80242 &$ 0.00839 $&  0.00098 \\
2454403.80275 &$ 0.00943 $&  0.00098 \\
2454403.80310 &$ 0.00730 $&  0.00098 \\
2454403.80343 &$ 0.00645 $&  0.00098 \\
2454403.80378 &$ 0.01458 $&  0.00098 \\
2454403.80411 &$ 0.01026 $&  0.00098 \\
2454403.80444 &$ 0.01287 $&  0.00098 \\
2454403.80475 &$ 0.00886 $&  0.00098 \\
2454403.80508 &$ 0.01316 $&  0.00098 \\
2454403.80541 &$ 0.00866 $&  0.00098 \\
2454403.80574 &$ 0.00678 $&  0.00098 \\
2454403.80608 &$ 0.01040 $&  0.00098 \\
2454403.80642 &$ 0.01454 $&  0.00098 \\
2454403.80674 &$ 0.00558 $&  0.00098 \\
2454403.80707 &$ 0.01143 $&  0.00098 \\
2454403.80740 &$ 0.00898 $&  0.00098 \\
2454403.80773 &$ 0.01486 $&  0.00098 \\
2454403.80806 &$ 0.01173 $&  0.00098 \\
2454403.80838 &$ 0.01141 $&  0.00098 \\
2454403.80870 &$ 0.01944 $&  0.00098 \\
2454403.80902 &$ 0.00992 $&  0.00098 \\
2454403.80935 &$ 0.01047 $&  0.00098 \\
2454403.80968 &$ 0.01435 $&  0.00099 \\
2454403.81002 &$ 0.00457 $&  0.00098 \\
2454403.81035 &$ 0.01087 $&  0.00098 \\
2454403.81070 &$ 0.02322 $&  0.00099 \\
2454403.81103 &$ 0.01280 $&  0.00098 \\
2454403.81135 &$ 0.01161 $&  0.00098 \\
2454403.81170 &$ 0.01219 $&  0.00098 \\
2454403.81204 &$ 0.01987 $&  0.00099 \\
2454403.81236 &$ 0.00920 $&  0.00098 \\
2454403.81267 &$ 0.00966 $&  0.00098 \\
2454403.81302 &$ 0.00987 $&  0.00098 \\
2454403.81333 &$ 0.01137 $&  0.00098 \\
2454403.81366 &$ 0.01247 $&  0.00098 \\
2454403.81400 &$ 0.01139 $&  0.00098 \\
2454403.81434 &$ 0.00749 $&  0.00099 \\
2454403.81468 &$ 0.01123 $&  0.00097 \\
2454403.81501 &$ 0.01383 $&  0.00098 \\
2454403.81535 &$ 0.00784 $&  0.00098 \\
2454403.81568 &$ 0.00643 $&  0.00098 \\
2454403.81601 &$ 0.01011 $&  0.00098 \\
2454403.81635 &$ 0.00864 $&  0.00098 \\
2454403.81669 &$ 0.01188 $&  0.00098 \\
2454403.81702 &$ 0.01424 $&  0.00098 \\
2454403.81736 &$ 0.01402 $&  0.00098 \\
2454403.81769 &$ 0.01420 $&  0.00098 \\
2454403.81800 &$ 0.00911 $&  0.00098 \\
2454403.81834 &$ 0.01161 $&  0.00099 \\
2454403.81868 &$ 0.01498 $&  0.00098 \\
2454403.81902 &$ 0.01225 $&  0.00099 \\
2454403.81935 &$ 0.01294 $&  0.00098 \\
2454403.81967 &$ 0.01549 $&  0.00099 \\
2454403.82000 &$ 0.01179 $&  0.00099 \\
2454403.82032 &$ 0.01205 $&  0.00099 \\
2454403.82068 &$ 0.00946 $&  0.00099 \\
2454403.82101 &$ 0.01239 $&  0.00099 \\
2454403.82135 &$ 0.01158 $&  0.00099 \\
2454403.82167 &$ 0.01213 $&  0.00099 \\
2454403.82200 &$ 0.00849 $&  0.00099 \\
2454403.82233 &$ 0.00800 $&  0.00099 \\
2454403.82266 &$ 0.01248 $&  0.00099 \\
2454403.82300 &$ 0.00983 $&  0.00099 \\
2454403.82333 &$ 0.00775 $&  0.00099 \\
2454403.82366 &$ 0.01588 $&  0.00099 \\
2454403.82399 &$ 0.00883 $&  0.00099 \\
2454403.82431 &$ 0.01330 $&  0.00100 \\
2454403.82464 &$ 0.00927 $&  0.00099 \\
2454403.82495 &$ 0.00901 $&  0.00099 \\
2454403.82529 &$ 0.01046 $&  0.00099 \\
2454403.82561 &$ 0.01289 $&  0.00099 \\
2454403.82596 &$ 0.01241 $&  0.00099 \\
2454403.82628 &$ 0.01045 $&  0.00099 \\
2454403.82662 &$ 0.01402 $&  0.00099 \\
2454403.82695 &$ 0.01235 $&  0.00099 \\
2454403.82729 &$ 0.01072 $&  0.00099 \\
2454403.82763 &$ 0.01077 $&  0.00100 \\
2454403.82795 &$ 0.00982 $&  0.00099 \\
2454403.82829 &$ 0.01057 $&  0.00100 \\
2454403.82862 &$ 0.01158 $&  0.00099 \\
2454403.82896 &$ 0.01637 $&  0.00100 \\
2454403.82930 &$ 0.01010 $&  0.00099 \\
2454403.82962 &$ 0.01207 $&  0.00100 \\
2454403.82995 &$ 0.01209 $&  0.00100 \\
2454403.83030 &$ 0.01106 $&  0.00100 \\
2454403.83061 &$ 0.01124 $&  0.00100 \\
2454403.83096 &$ 0.00984 $&  0.00100 \\
2454403.83130 &$ 0.01248 $&  0.00100 \\
2454403.83164 &$ 0.01138 $&  0.00099 \\
2454403.83203 &$ 0.00624 $&  0.00100 \\
2454403.83238 &$ 0.00909 $&  0.00100 \\
2454403.83273 &$ 0.00785 $&  0.00099 \\
2454403.83306 &$ 0.01225 $&  0.00100 \\
2454403.83341 &$ 0.00994 $&  0.00100 \\
2454403.83373 &$ 0.00767 $&  0.00100 \\
2454403.83407 &$ 0.01212 $&  0.00100 \\
2454403.83442 &$ 0.00672 $&  0.00099 \\
2454403.83473 &$ 0.01262 $&  0.00100 \\
2454403.83506 &$ 0.01053 $&  0.00100 \\
2454403.83539 &$ 0.01122 $&  0.00100 \\
2454403.83572 &$ 0.00653 $&  0.00099 \\
2454403.83605 &$ 0.00904 $&  0.00100 \\
2454403.83638 &$ 0.01358 $&  0.00100 \\
2454403.83671 &$ 0.01418 $&  0.00100 \\
2454403.83704 &$ 0.01201 $&  0.00100 \\
2454403.83738 &$ 0.01209 $&  0.00100 \\
2454403.83771 &$ 0.01405 $&  0.00100 \\
2454403.83806 &$ 0.01147 $&  0.00100 \\
2454403.83840 &$ 0.00810 $&  0.00100 \\
2454403.83871 &$ 0.01302 $&  0.00100 \\
2454403.83906 &$ 0.01251 $&  0.00100 \\
2454403.83937 &$ 0.00964 $&  0.00100 \\
2454403.83969 &$ 0.01461 $&  0.00100 \\
2454403.84002 &$ 0.01245 $&  0.00100 \\
2454403.84035 &$ 0.01527 $&  0.00100 \\
2454403.84067 &$ 0.01023 $&  0.00100 \\
2454403.84101 &$ 0.00825 $&  0.00100 \\
2454403.84134 &$ 0.01099 $&  0.00100 \\
2454403.84170 &$ 0.01164 $&  0.00100 \\
2454403.84202 &$ 0.00956 $&  0.00101 \\
2454403.84238 &$ 0.01338 $&  0.00100 \\
2454403.84271 &$ 0.01371 $&  0.00100 \\
2454403.84304 &$ 0.00974 $&  0.00100 \\
2454403.84336 &$ 0.01205 $&  0.00100 \\
2454403.84370 &$ 0.00980 $&  0.00101 \\
2454403.84405 &$ 0.01517 $&  0.00101 \\
2454403.84438 &$ 0.01146 $&  0.00101 \\
2454403.84472 &$ 0.01335 $&  0.00101 \\
2454403.84505 &$ 0.00882 $&  0.00101 \\
2454403.84539 &$ 0.00990 $&  0.00100 \\
2454403.84571 &$ 0.00756 $&  0.00101 \\
2454403.84606 &$ 0.00815 $&  0.00101 \\
2454403.84637 &$ 0.00822 $&  0.00100 \\
2454403.84673 &$ 0.01080 $&  0.00101 \\
2454403.84705 &$ 0.01185 $&  0.00101 \\
2454403.84740 &$ 0.00620 $&  0.00100 \\
2454403.84775 &$ 0.01360 $&  0.00101 \\
2454403.84810 &$ 0.00798 $&  0.00101 \\
2454403.84842 &$ 0.01127 $&  0.00102 \\
2454403.84878 &$ 0.00808 $&  0.00101 \\
2454403.84910 &$ 0.01561 $&  0.00100 \\
2454403.84943 &$ 0.01159 $&  0.00100 \\
2454403.84976 &$ 0.01473 $&  0.00100 \\
2454403.85009 &$ 0.01201 $&  0.00100 \\
2454403.85041 &$ 0.01538 $&  0.00100 \\
2454403.85075 &$ 0.01185 $&  0.00101 \\
2454403.85108 &$ 0.00588 $&  0.00100 \\
2454403.85142 &$ 0.00605 $&  0.00100 \\
2454403.85176 &$ 0.00785 $&  0.00100 \\
2454403.85210 &$ 0.00635 $&  0.00100 \\
2454403.85244 &$ 0.00957 $&  0.00101 \\
2454403.85278 &$ 0.00755 $&  0.00100 \\
2454403.85313 &$ 0.01148 $&  0.00100 \\
2454403.85347 &$ 0.01045 $&  0.00101 \\
2454403.85380 &$ 0.00634 $&  0.00100 \\
2454403.85413 &$ 0.01196 $&  0.00101 \\
2454403.85446 &$ 0.01108 $&  0.00102 \\
2454403.85479 &$ 0.01184 $&  0.00102 \\
2454403.85513 &$ 0.01198 $&  0.00101 \\
2454403.85547 &$ 0.01074 $&  0.00101 \\
2454403.85579 &$ 0.00976 $&  0.00101 \\
2454403.85614 &$ 0.00946 $&  0.00101 \\
2454403.85646 &$ 0.01064 $&  0.00101 \\
2454403.85681 &$ 0.00983 $&  0.00101 \\
2454403.85712 &$ 0.01228 $&  0.00101 \\
2454403.85746 &$ 0.00719 $&  0.00101 \\
2454403.85779 &$ 0.01308 $&  0.00101 \\
2454403.85812 &$ 0.01259 $&  0.00101 \\
2454403.85847 &$ 0.00607 $&  0.00101 \\
2454403.85879 &$ 0.00935 $&  0.00101 \\
2454403.85913 &$ 0.01015 $&  0.00102 \\
2454403.85945 &$ 0.01458 $&  0.00102 \\
2454403.85979 &$ 0.01161 $&  0.00102 \\
2454403.86012 &$ 0.01133 $&  0.00102 \\
2454403.86047 &$ 0.01094 $&  0.00101 \\
2454403.86080 &$ 0.00826 $&  0.00101 \\
2454403.86114 &$ 0.00844 $&  0.00102 \\
2454403.86145 &$ 0.00744 $&  0.00101 \\
2454403.86180 &$ 0.00746 $&  0.00101 \\
2454403.86215 &$ 0.00740 $&  0.00102 \\
2454403.86247 &$ 0.00834 $&  0.00101 \\
2454403.86279 &$ 0.01498 $&  0.00102 \\
2454403.86314 &$ 0.01564 $&  0.00102 \\
2454403.86345 &$ 0.00398 $&  0.00101 \\
2454403.86376 &$ 0.01017 $&  0.00102 \\
2454403.86409 &$ 0.00330 $&  0.00102 \\
2454403.86441 &$ 0.01147 $&  0.00101 \\
2454403.86476 &$ 0.00902 $&  0.00102 \\
2454403.86511 &$ 0.01553 $&  0.00102 \\
2454403.86548 &$ 0.01038 $&  0.00102 \\
2454403.86580 &$ 0.00693 $&  0.00102 \\
2454403.86617 &$ 0.01171 $&  0.00102 \\
2454403.86650 &$ 0.00759 $&  0.00102 \\
2454403.86683 &$ 0.01243 $&  0.00101 \\
2454403.86719 &$ 0.01302 $&  0.00101 \\
2454403.86753 &$ 0.01096 $&  0.00101 \\
2454403.86786 &$ 0.01204 $&  0.00101 \\
2454403.86821 &$ 0.01186 $&  0.00102 \\
2454403.86855 &$ 0.00888 $&  0.00102 \\
2454403.86887 &$ 0.01573 $&  0.00103 \\
2454403.86920 &$ 0.00994 $&  0.00102 \\
2454403.86952 &$ 0.01405 $&  0.00102 \\
2454403.86987 &$ 0.01232 $&  0.00102 \\
2454403.87020 &$ 0.01528 $&  0.00101 \\
2454403.87054 &$ 0.00951 $&  0.00102 \\
2454403.87088 &$ 0.01362 $&  0.00102 \\
2454403.87121 &$ 0.01184 $&  0.00102 \\
2454403.87153 &$ 0.00742 $&  0.00102 \\
2454403.87187 &$ 0.01556 $&  0.00102 \\
2454403.87219 &$ 0.00753 $&  0.00101 \\
2454403.87250 &$ 0.00747 $&  0.00102 \\
2454403.87283 &$ 0.00924 $&  0.00101 \\
2454403.87318 &$ 0.01023 $&  0.00102 \\
2454403.87350 &$ 0.00824 $&  0.00102 \\
2454406.76967 &$-0.00030 $&  0.00096 \\
2454406.76999 &$-0.00030 $&  0.00096 \\
2454406.77031 &$ 0.00131 $&  0.00096 \\
2454406.77064 &$-0.00239 $&  0.00096 \\
2454406.77095 &$ 0.00065 $&  0.00097 \\
2454406.77127 &$ 0.00349 $&  0.00096 \\
2454406.77158 &$ 0.00142 $&  0.00096 \\
2454406.77190 &$-0.00058 $&  0.00095 \\
2454406.77224 &$ 0.00469 $&  0.00097 \\
2454406.77257 &$-0.00057 $&  0.00096 \\
2454406.77290 &$-0.00089 $&  0.00098 \\
2454406.77322 &$-0.00181 $&  0.00097 \\
2454406.77356 &$-0.00451 $&  0.00096 \\
2454406.77390 &$-0.00093 $&  0.00096 \\
2454406.77423 &$-0.00148 $&  0.00096 \\
2454406.77459 &$ 0.00098 $&  0.00097 \\
2454406.77491 &$-0.00032 $&  0.00096 \\
2454406.77524 &$-0.00379 $&  0.00097 \\
2454406.77557 &$ 0.00095 $&  0.00097 \\
2454406.77588 &$-0.00066 $&  0.00096 \\
2454406.77622 &$-0.00012 $&  0.00096 \\
2454406.77654 &$ 0.00038 $&  0.00096 \\
2454406.77687 &$-0.00236 $&  0.00096 \\
2454406.77719 &$-0.00206 $&  0.00096 \\
2454406.77752 &$ 0.00140 $&  0.00097 \\
2454406.77786 &$ 0.00118 $&  0.00096 \\
2454406.77819 &$-0.00158 $&  0.00097 \\
2454406.77853 &$ 0.00018 $&  0.00096 \\
2454406.77888 &$ 0.00142 $&  0.00095 \\
2454406.77919 &$ 0.00033 $&  0.00096 \\
2454406.77953 &$-0.00035 $&  0.00098 \\
2454406.77984 &$-0.00328 $&  0.00098 \\
2454406.78019 &$ 0.00081 $&  0.00097 \\
2454406.78050 &$ 0.00017 $&  0.00097 \\
2454406.78084 &$-0.00020 $&  0.00096 \\
2454406.78118 &$-0.00116 $&  0.00096 \\
2454406.78150 &$-0.00017 $&  0.00096 \\
2454406.78184 &$-0.00216 $&  0.00096 \\
2454406.78216 &$-0.00072 $&  0.00096 \\
2454406.78252 &$ 0.00029 $&  0.00096 \\
2454406.78285 &$ 0.00064 $&  0.00096 \\
2454406.78319 &$ 0.00148 $&  0.00096 \\
2454406.78351 &$ 0.00064 $&  0.00096 \\
2454406.78384 &$-0.00139 $&  0.00096 \\
2454406.78416 &$ 0.00035 $&  0.00096 \\
2454406.78451 &$-0.00458 $&  0.00096 \\
2454406.78484 &$ 0.00457 $&  0.00098 \\
2454406.78517 &$ 0.00089 $&  0.00097 \\
2454406.78549 &$-0.00055 $&  0.00097 \\
2454406.78584 &$ 0.00079 $&  0.00098 \\
2454406.78617 &$-0.00252 $&  0.00096 \\
2454406.78651 &$-0.00147 $&  0.00096 \\
2454406.78682 &$-0.00008 $&  0.00096 \\
2454406.78715 &$ 0.00099 $&  0.00098 \\
2454406.78748 &$ 0.00246 $&  0.00098 \\
2454406.78782 &$ 0.00196 $&  0.00097 \\
2454406.78813 &$ 0.00162 $&  0.00097 \\
2454406.78845 &$-0.00053 $&  0.00097 \\
2454406.78878 &$-0.00023 $&  0.00096 \\
2454406.78910 &$-0.00050 $&  0.00095 \\
2454406.78944 &$-0.00263 $&  0.00096 \\
2454406.78978 &$ 0.00070 $&  0.00096 \\
2454406.79012 &$ 0.00220 $&  0.00097 \\
2454406.79046 &$ 0.00267 $&  0.00096 \\
2454406.79079 &$-0.00018 $&  0.00096 \\
2454406.79114 &$-0.00056 $&  0.00096 \\
2454406.79147 &$-0.00287 $&  0.00098 \\
2454406.79180 &$ 0.00015 $&  0.00098 \\
2454406.79214 &$-0.00064 $&  0.00098 \\
2454406.79246 &$ 0.00141 $&  0.00097 \\
2454406.79279 &$-0.00322 $&  0.00098 \\
2454406.79312 &$-0.00150 $&  0.00098 \\
2454406.79344 &$-0.00129 $&  0.00099 \\
2454406.79376 &$-0.00116 $&  0.00096 \\
2454406.79411 &$-0.00029 $&  0.00096 \\
2454406.79442 &$-0.00008 $&  0.00097 \\
2454406.79476 &$ 0.00044 $&  0.00096 \\
2454406.79511 &$-0.00278 $&  0.00096 \\
2454406.79543 &$-0.00239 $&  0.00096 \\
2454406.79578 &$-0.00025 $&  0.00096 \\
2454406.79611 &$-0.00101 $&  0.00097 \\
2454406.79646 &$-0.00344 $&  0.00097 \\
2454406.79681 &$-0.00287 $&  0.00097 \\
2454406.79714 &$-0.00114 $&  0.00097 \\
2454406.79746 &$ 0.00285 $&  0.00097 \\
2454406.79782 &$-0.00194 $&  0.00096 \\
2454406.79815 &$-0.00126 $&  0.00097 \\
2454406.79845 &$ 0.00140 $&  0.00097 \\
2454406.79879 &$ 0.00216 $&  0.00097 \\
2454406.79911 &$-0.00218 $&  0.00096 \\
2454406.79945 &$ 0.00231 $&  0.00097 \\
2454406.79977 &$-0.00248 $&  0.00097 \\
2454406.80011 &$ 0.00124 $&  0.00098 \\
2454406.80044 &$-0.00352 $&  0.00102 \\
2454406.80078 &$ 0.00022 $&  0.00097 \\
2454406.80111 &$-0.00153 $&  0.00097 \\
2454406.80146 &$ 0.00194 $&  0.00098 \\
2454406.80180 &$-0.00065 $&  0.00097 \\
2454406.80213 &$-0.00177 $&  0.00096 \\
2454406.80247 &$ 0.00136 $&  0.00097 \\
2454406.80283 &$ 0.00170 $&  0.00096 \\
2454406.80316 &$ 0.00090 $&  0.00096 \\
2454406.80351 &$-0.00046 $&  0.00096 \\
2454406.80385 &$ 0.00069 $&  0.00096 \\
2454406.80416 &$-0.00094 $&  0.00096 \\
2454406.80448 &$ 0.00313 $&  0.00097 \\
2454406.80481 &$ 0.00154 $&  0.00096 \\
2454406.80514 &$-0.00144 $&  0.00096 \\
2454406.80548 &$ 0.00162 $&  0.00097 \\
2454406.80580 &$-0.00020 $&  0.00097 \\
2454406.80613 &$ 0.00106 $&  0.00097 \\
2454406.80647 &$-0.00221 $&  0.00097 \\
2454406.80681 &$ 0.00109 $&  0.00097 \\
2454406.80714 &$ 0.00002 $&  0.00097 \\
2454406.80747 &$ 0.00188 $&  0.00097 \\
2454406.80780 &$-0.00273 $&  0.00097 \\
2454406.80814 &$-0.00021 $&  0.00097 \\
2454406.80848 &$ 0.00040 $&  0.00097 \\
2454406.80879 &$ 0.00083 $&  0.00098 \\
2454406.80912 &$ 0.00233 $&  0.00097 \\
2454406.80946 &$-0.00083 $&  0.00097 \\
2454406.80977 &$ 0.00222 $&  0.00098 \\
2454406.81011 &$ 0.00082 $&  0.00097 \\
2454406.81045 &$-0.00177 $&  0.00097 \\
2454406.81078 &$ 0.00151 $&  0.00097 \\
2454406.81111 &$ 0.00416 $&  0.00097 \\
2454406.81145 &$-0.00181 $&  0.00096 \\
2454406.81177 &$-0.00058 $&  0.00097 \\
2454406.81212 &$ 0.00399 $&  0.00097 \\
2454406.81244 &$ 0.00018 $&  0.00097 \\
2454406.81277 &$-0.00060 $&  0.00097 \\
2454406.81309 &$-0.00128 $&  0.00097 \\
2454406.81344 &$-0.00268 $&  0.00097 \\
2454406.81378 &$-0.00078 $&  0.00097 \\
2454406.81411 &$ 0.00378 $&  0.00097 \\
2454406.81443 &$ 0.00334 $&  0.00097 \\
2454406.81476 &$ 0.00098 $&  0.00097 \\
2454406.81508 &$ 0.00165 $&  0.00097 \\
2454406.81542 &$ 0.00530 $&  0.00098 \\
2454406.81577 &$-0.00458 $&  0.00097 \\
2454406.81609 &$ 0.00193 $&  0.00098 \\
2454406.81644 &$ 0.00165 $&  0.00097 \\
2454406.81676 &$ 0.00067 $&  0.00097 \\
2454406.81710 &$-0.00108 $&  0.00097 \\
2454406.81744 &$ 0.00895 $&  0.00097 \\
2454406.81778 &$ 0.00010 $&  0.00097 \\
2454406.81810 &$-0.00041 $&  0.00097 \\
2454406.81844 &$ 0.00011 $&  0.00097 \\
2454406.81878 &$ 0.00232 $&  0.00097 \\
2454406.81912 &$-0.00047 $&  0.00098 \\
2454406.81946 &$-0.00189 $&  0.00097 \\
2454406.81977 &$ 0.00190 $&  0.00097 \\
2454406.82009 &$ 0.00201 $&  0.00098 \\
2454406.82043 &$ 0.00074 $&  0.00097 \\
2454406.82078 &$-0.00286 $&  0.00097 \\
2454406.82110 &$ 0.00026 $&  0.00098 \\
2454406.82144 &$ 0.00032 $&  0.00097 \\
2454406.82176 &$ 0.00105 $&  0.00096 \\
2454406.82211 &$-0.00060 $&  0.00097 \\
2454406.82244 &$ 0.00040 $&  0.00098 \\
2454406.82277 &$-0.00095 $&  0.00097 \\
2454406.82310 &$-0.00085 $&  0.00098 \\
2454406.82343 &$-0.00306 $&  0.00097 \\
2454406.82376 &$ 0.00363 $&  0.00097 \\
2454406.82411 &$-0.00434 $&  0.00097 \\
2454406.82445 &$ 0.00033 $&  0.00097 \\
2454406.82476 &$ 0.00197 $&  0.00097 \\
2454406.82506 &$ 0.00247 $&  0.00097 \\
2454406.82538 &$ 0.00265 $&  0.00097 \\
2454406.82572 &$-0.00148 $&  0.00096 \\
2454406.82606 &$ 0.00192 $&  0.00097 \\
2454406.82638 &$ 0.00068 $&  0.00097 \\
2454406.82670 &$ 0.00035 $&  0.00096 \\
2454406.82704 &$ 0.00367 $&  0.00097 \\
2454406.82735 &$-0.00124 $&  0.00097 \\
2454406.82769 &$-0.00066 $&  0.00097 \\
2454406.82800 &$-0.00365 $&  0.00097 \\
2454406.82834 &$ 0.00018 $&  0.00097 \\
2454406.82867 &$ 0.00051 $&  0.00097 \\
2454406.82902 &$-0.00068 $&  0.00097 \\
2454406.82935 &$ 0.00194 $&  0.00097 \\
2454406.82968 &$-0.00092 $&  0.00097 \\
2454406.83003 &$ 0.00259 $&  0.00097 \\
2454406.83034 &$-0.00232 $&  0.00097 \\
2454406.83067 &$-0.00489 $&  0.00097 \\
2454406.83100 &$ 0.00201 $&  0.00098 \\
2454406.83134 &$ 0.00095 $&  0.00098 \\
2454406.83167 &$ 0.00169 $&  0.00100 \\
2454406.83200 &$-0.00037 $&  0.00098 \\
2454406.83233 &$-0.00423 $&  0.00097 \\
2454406.83265 &$ 0.00123 $&  0.00097 \\
2454406.83296 &$ 0.00239 $&  0.00097 \\
2454406.83330 &$ 0.00194 $&  0.00097 \\
2454406.83361 &$ 0.00197 $&  0.00097 \\
2454406.83395 &$ 0.00478 $&  0.00097 \\
2454406.83428 &$ 0.00191 $&  0.00098 \\
2454406.83461 &$ 0.00219 $&  0.00097 \\
2454406.83494 &$ 0.00521 $&  0.00097 \\
2454406.83527 &$ 0.00746 $&  0.00098 \\
2454406.83559 &$ 0.00145 $&  0.00098 \\
2454406.83593 &$ 0.00304 $&  0.00097 \\
2454406.83625 &$ 0.00578 $&  0.00097 \\
2454406.83659 &$ 0.00806 $&  0.00098 \\
2454406.83695 &$ 0.00836 $&  0.00098 \\
2454406.83730 &$ 0.00742 $&  0.00098 \\
2454406.83759 &$-0.00130 $&  0.00097 \\
2454406.83794 &$ 0.00391 $&  0.00098 \\
2454406.83828 &$ 0.00721 $&  0.00098 \\
2454406.83860 &$ 0.00579 $&  0.00098 \\
2454406.83892 &$ 0.00861 $&  0.00098 \\
2454406.83926 &$ 0.00402 $&  0.00098 \\
2454406.83958 &$ 0.00307 $&  0.00097 \\
2454406.83992 &$ 0.00516 $&  0.00098 \\
2454406.84026 &$ 0.00614 $&  0.00098 \\
2454406.84057 &$ 0.00464 $&  0.00098 \\
2454406.84090 &$ 0.00167 $&  0.00097 \\
2454406.84123 &$ 0.00596 $&  0.00097 \\
2454406.84159 &$ 0.01063 $&  0.00097 \\
2454406.84191 &$ 0.01204 $&  0.00098 \\
2454406.84226 &$ 0.00868 $&  0.00098 \\
2454406.84259 &$ 0.01038 $&  0.00098 \\
2454406.84292 &$ 0.00905 $&  0.00098 \\
2454406.84324 &$ 0.00653 $&  0.00098 \\
2454406.84358 &$ 0.01165 $&  0.00098 \\
2454406.84390 &$ 0.01007 $&  0.00098 \\
2454406.84424 &$ 0.00634 $&  0.00098 \\
2454406.84458 &$ 0.01240 $&  0.00098 \\
2454406.84490 &$ 0.00745 $&  0.00098 \\
2454406.84523 &$ 0.01587 $&  0.00098 \\
2454406.84557 &$ 0.01255 $&  0.00098 \\
2454406.84590 &$ 0.01845 $&  0.00099 \\
2454406.84623 &$ 0.00988 $&  0.00098 \\
2454406.84659 &$ 0.01004 $&  0.00098 \\
2454406.84690 &$ 0.00520 $&  0.00098 \\
2454406.84723 &$ 0.00613 $&  0.00098 \\
2454406.84755 &$ 0.00674 $&  0.00098 \\
2454406.84789 &$ 0.00915 $&  0.00099 \\
2454406.84824 &$ 0.00496 $&  0.00098 \\
2454406.84855 &$ 0.00997 $&  0.00097 \\
2454406.84889 &$ 0.01300 $&  0.00098 \\
2454406.84921 &$ 0.00881 $&  0.00099 \\
2454406.84955 &$ 0.00792 $&  0.00098 \\
2454406.84986 &$ 0.01325 $&  0.00099 \\
2454406.85019 &$ 0.00804 $&  0.00098 \\
2454406.85052 &$ 0.00532 $&  0.00098 \\
2454406.85085 &$ 0.00980 $&  0.00098 \\
2454406.85118 &$ 0.00530 $&  0.00098 \\
2454406.85149 &$ 0.00362 $&  0.00098 \\
2454406.85183 &$ 0.01065 $&  0.00098 \\
2454406.85214 &$ 0.01321 $&  0.00098 \\
2454406.85249 &$ 0.01174 $&  0.00098 \\
2454406.85280 &$ 0.01349 $&  0.00098 \\
2454406.85315 &$ 0.01169 $&  0.00098 \\
2454406.85348 &$ 0.01090 $&  0.00099 \\
2454406.85381 &$ 0.00696 $&  0.00098 \\
2454406.85414 &$ 0.01154 $&  0.00099 \\
2454406.85449 &$ 0.00621 $&  0.00098 \\
2454406.85484 &$ 0.01359 $&  0.00099 \\
2454406.85517 &$ 0.00740 $&  0.00098 \\
2454406.85550 &$ 0.00340 $&  0.00098 \\
2454406.85583 &$ 0.01553 $&  0.00099 \\
2454406.85618 &$ 0.00882 $&  0.00099 \\
2454406.85650 &$ 0.01300 $&  0.00099 \\
2454406.85684 &$ 0.01353 $&  0.00099 \\
2454406.85715 &$ 0.00924 $&  0.00099 \\
2454406.85749 &$ 0.01040 $&  0.00099 \\
2454406.85784 &$ 0.01065 $&  0.00099 \\
2454406.85817 &$ 0.01147 $&  0.00098 \\
2454406.85850 &$ 0.01001 $&  0.00099 \\
2454406.85884 &$ 0.01225 $&  0.00098 \\
2454406.85919 &$ 0.01042 $&  0.00098 \\
2454406.85953 &$ 0.00750 $&  0.00099 \\
2454406.85985 &$ 0.01208 $&  0.00099 \\
2454406.86020 &$ 0.01037 $&  0.00099 \\
2454406.86053 &$ 0.00908 $&  0.00099 \\
2454406.86085 &$ 0.01297 $&  0.00099 \\
2454406.86118 &$ 0.01003 $&  0.00099 \\
2454406.86150 &$ 0.01316 $&  0.00099 \\
2454406.86181 &$ 0.00571 $&  0.00099 \\
2454406.86214 &$ 0.01445 $&  0.00099 \\
2454406.86248 &$ 0.01488 $&  0.00099 \\
2454406.86280 &$ 0.00923 $&  0.00099 \\
2454406.86314 &$ 0.00435 $&  0.00099 \\
2454406.86344 &$ 0.01232 $&  0.00099 \\
2454406.86377 &$ 0.01637 $&  0.00098 \\
2454406.86410 &$ 0.01583 $&  0.00099 \\
2454406.86443 &$ 0.00568 $&  0.00099 \\
2454406.86479 &$ 0.00834 $&  0.00099 \\
2454437.55774 &$ 0.00251 $&  0.00097 \\
2454437.55807 &$-0.00100 $&  0.00097 \\
2454437.55842 &$-0.00005 $&  0.00097 \\
2454437.55874 &$ 0.00128 $&  0.00097 \\
2454437.55904 &$ 0.00087 $&  0.00098 \\
2454437.55937 &$-0.00077 $&  0.00097 \\
2454437.55971 &$ 0.00032 $&  0.00097 \\
2454437.56004 &$-0.00111 $&  0.00098 \\
2454437.56036 &$ 0.00113 $&  0.00097 \\
2454437.56071 &$ 0.00169 $&  0.00096 \\
2454437.56103 &$-0.00010 $&  0.00096 \\
2454437.56137 &$ 0.00075 $&  0.00097 \\
2454437.56169 &$ 0.00098 $&  0.00098 \\
2454437.56203 &$-0.00102 $&  0.00097 \\
2454437.56236 &$ 0.00028 $&  0.00098 \\
2454437.56268 &$ 0.00003 $&  0.00096 \\
2454437.56300 &$ 0.00111 $&  0.00097 \\
2454437.56334 &$-0.00140 $&  0.00097 \\
2454437.56368 &$ 0.00164 $&  0.00097 \\
2454437.56402 &$-0.00133 $&  0.00098 \\
2454437.56435 &$ 0.00013 $&  0.00097 \\
2454437.56469 &$ 0.00224 $&  0.00097 \\
2454437.56501 &$-0.00040 $&  0.00097 \\
2454437.56535 &$-0.00228 $&  0.00096 \\
2454437.56569 &$-0.00033 $&  0.00096 \\
2454437.56600 &$-0.00082 $&  0.00097 \\
2454437.56635 &$ 0.00232 $&  0.00096 \\
2454437.56666 &$ 0.00467 $&  0.00097 \\
2454437.56700 &$-0.00110 $&  0.00097 \\
2454437.56733 &$ 0.00079 $&  0.00096 \\
2454437.56766 &$ 0.00228 $&  0.00097 \\
2454437.56799 &$-0.00064 $&  0.00096 \\
2454437.56834 &$ 0.00093 $&  0.00097 \\
2454437.56866 &$ 0.00083 $&  0.00097 \\
2454437.56898 &$ 0.00113 $&  0.00096 \\
2454437.56933 &$ 0.00140 $&  0.00097 \\
2454437.56967 &$ 0.00104 $&  0.00097 \\
2454437.57001 &$-0.00068 $&  0.00096 \\
2454437.57034 &$-0.00079 $&  0.00097 \\
2454437.57067 &$-0.00283 $&  0.00096 \\
2454437.57101 &$-0.00080 $&  0.00098 \\
2454437.57135 &$-0.00060 $&  0.00099 \\
2454437.57168 &$-0.00287 $&  0.00097 \\
2454437.57200 &$ 0.00120 $&  0.00098 \\
2454437.57235 &$-0.00156 $&  0.00097 \\
2454437.57268 &$-0.00194 $&  0.00097 \\
2454437.57300 &$-0.00243 $&  0.00097 \\
2454437.57334 &$-0.00147 $&  0.00097 \\
2454437.57366 &$ 0.00212 $&  0.00097 \\
2454437.57401 &$ 0.00104 $&  0.00097 \\
2454437.57437 &$-0.00026 $&  0.00096 \\
2454437.57468 &$-0.00006 $&  0.00096 \\
2454437.57503 &$-0.00076 $&  0.00097 \\
2454437.57536 &$ 0.00192 $&  0.00098 \\
2454437.57569 &$ 0.00688 $&  0.00097 \\
2454437.57601 &$ 0.00103 $&  0.00097 \\
2454437.57637 &$-0.00132 $&  0.00097 \\
2454437.57668 &$-0.00028 $&  0.00097 \\
2454437.57703 &$-0.00174 $&  0.00097 \\
2454437.57736 &$ 0.00182 $&  0.00098 \\
2454437.57770 &$-0.00025 $&  0.00097 \\
2454437.57802 &$ 0.00091 $&  0.00097 \\
2454437.57837 &$-0.00177 $&  0.00096 \\
2454437.57869 &$ 0.00141 $&  0.00098 \\
2454437.57905 &$ 0.00163 $&  0.00097 \\
2454437.57936 &$-0.00247 $&  0.00098 \\
2454437.57971 &$ 0.00062 $&  0.00098 \\
2454437.58004 &$ 0.00076 $&  0.00097 \\
2454437.58038 &$-0.00050 $&  0.00097 \\
2454437.58071 &$-0.00288 $&  0.00097 \\
2454437.58103 &$ 0.00063 $&  0.00097 \\
2454437.58138 &$-0.00207 $&  0.00098 \\
2454437.58170 &$ 0.00077 $&  0.00098 \\
2454437.58204 &$-0.00115 $&  0.00097 \\
2454437.58239 &$-0.00064 $&  0.00097 \\
2454437.58273 &$-0.00075 $&  0.00097 \\
2454437.58306 &$ 0.00117 $&  0.00097 \\
2454437.58340 &$-0.00197 $&  0.00097 \\
2454437.58373 &$ 0.00088 $&  0.00097 \\
2454437.58406 &$-0.00064 $&  0.00097 \\
2454437.58440 &$ 0.00245 $&  0.00098 \\
2454437.58474 &$-0.00182 $&  0.00097 \\
2454437.58504 &$ 0.00027 $&  0.00098 \\
2454437.58538 &$-0.00044 $&  0.00099 \\
2454437.58571 &$-0.00170 $&  0.00097 \\
2454437.58603 &$-0.00112 $&  0.00101 \\
2454437.58638 &$-0.00106 $&  0.00097 \\
2454437.58670 &$ 0.00087 $&  0.00098 \\
2454437.58704 &$-0.00185 $&  0.00098 \\
2454437.58736 &$ 0.00173 $&  0.00099 \\
2454437.58770 &$-0.00118 $&  0.00098 \\
2454437.58802 &$-0.00132 $&  0.00097 \\
2454437.58835 &$-0.00078 $&  0.00097 \\
2454437.58868 &$-0.00038 $&  0.00098 \\
2454437.58901 &$ 0.00032 $&  0.00096 \\
2454437.58933 &$ 0.00184 $&  0.00097 \\
2454437.58964 &$-0.00289 $&  0.00097 \\
2454437.58998 &$-0.00052 $&  0.00096 \\
2454437.59030 &$ 0.00008 $&  0.00097 \\
2454437.59065 &$-0.00005 $&  0.00097 \\
2454437.59098 &$-0.00090 $&  0.00096 \\
2454437.59133 &$-0.00029 $&  0.00096 \\
2454437.59167 &$-0.00005 $&  0.00096 \\
2454437.59199 &$-0.00106 $&  0.00096 \\
2454437.59234 &$ 0.00098 $&  0.00097 \\
2454437.59266 &$-0.00087 $&  0.00096 \\
2454437.59298 &$-0.00046 $&  0.00096 \\
2454437.59331 &$ 0.00100 $&  0.00097 \\
2454437.59362 &$-0.00025 $&  0.00096 \\
2454437.59396 &$-0.00030 $&  0.00097 \\
2454437.59429 &$ 0.00284 $&  0.00097 \\
2454437.59462 &$ 0.00211 $&  0.00096 \\
2454437.59494 &$ 0.00236 $&  0.00097 \\
2454437.59528 &$ 0.00085 $&  0.00098 \\
2454437.59561 &$ 0.00155 $&  0.00096 \\
2454437.59596 &$ 0.00223 $&  0.00096 \\
2454437.59633 &$ 0.00299 $&  0.00097 \\
2454437.59668 &$ 0.00085 $&  0.00097 \\
2454437.59700 &$ 0.00395 $&  0.00097 \\
2454437.59732 &$ 0.00279 $&  0.00097 \\
2454437.59766 &$ 0.00334 $&  0.00097 \\
2454437.59800 &$ 0.00259 $&  0.00097 \\
2454437.59832 &$ 0.00192 $&  0.00097 \\
2454437.59866 &$ 0.00215 $&  0.00098 \\
2454437.59899 &$ 0.00512 $&  0.00098 \\
2454437.59932 &$ 0.00174 $&  0.00097 \\
2454437.59962 &$ 0.00476 $&  0.00097 \\
2454437.59997 &$ 0.00591 $&  0.00097 \\
2454437.60030 &$ 0.00230 $&  0.00098 \\
2454437.60061 &$ 0.00559 $&  0.00098 \\
2454437.60093 &$ 0.00574 $&  0.00098 \\
2454437.60127 &$ 0.00522 $&  0.00098 \\
2454437.60161 &$ 0.00482 $&  0.00097 \\
2454437.60193 &$ 0.00488 $&  0.00097 \\
2454437.60227 &$ 0.00868 $&  0.00098 \\
2454437.60263 &$ 0.00424 $&  0.00097 \\
2454437.60295 &$ 0.00662 $&  0.00097 \\
2454437.60328 &$ 0.00455 $&  0.00097 \\
2454437.60362 &$ 0.00574 $&  0.00098 \\
2454437.60395 &$ 0.00755 $&  0.00097 \\
2454437.60428 &$ 0.00844 $&  0.00097 \\
2454437.60459 &$ 0.00671 $&  0.00097 \\
2454437.60493 &$ 0.00748 $&  0.00098 \\
2454437.60525 &$ 0.00702 $&  0.00098 \\
2454437.60558 &$ 0.00840 $&  0.00097 \\
2454437.60591 &$ 0.00891 $&  0.00098 \\
2454437.60624 &$ 0.00745 $&  0.00098 \\
2454437.60659 &$ 0.00738 $&  0.00097 \\
2454437.60691 &$ 0.01052 $&  0.00098 \\
2454437.60724 &$ 0.00967 $&  0.00097 \\
2454437.60905 &$ 0.00886 $&  0.00097 \\
2454437.60939 &$ 0.00731 $&  0.00097 \\
2454437.60972 &$ 0.00962 $&  0.00097 \\
2454437.61005 &$ 0.00761 $&  0.00098 \\
2454437.61039 &$ 0.00893 $&  0.00098 \\
2454437.61075 &$ 0.00839 $&  0.00098 \\
2454437.61108 &$ 0.00911 $&  0.00098 \\
2454437.61140 &$ 0.00829 $&  0.00097 \\
2454437.61175 &$ 0.00883 $&  0.00098 \\
2454437.61211 &$ 0.00432 $&  0.00098 \\
2454437.61243 &$ 0.00774 $&  0.00097 \\
2454437.61275 &$ 0.01217 $&  0.00099 \\
2454437.61309 &$ 0.01046 $&  0.00098 \\
2454437.61340 &$ 0.00856 $&  0.00098 \\
2454437.61371 &$ 0.01002 $&  0.00097 \\
2454437.61404 &$ 0.00661 $&  0.00100 \\
2454437.61437 &$ 0.00630 $&  0.00098 \\
2454437.61471 &$ 0.00612 $&  0.00097 \\
2454437.61503 &$ 0.01141 $&  0.00099 \\
2454437.61537 &$ 0.00702 $&  0.00098 \\
2454437.61571 &$ 0.00645 $&  0.00097 \\
2454437.61604 &$ 0.00877 $&  0.00097 \\
2454437.61638 &$ 0.01036 $&  0.00100 \\
2454437.61671 &$ 0.01146 $&  0.00098 \\
2454437.61706 &$ 0.01056 $&  0.00099 \\
2454437.61738 &$ 0.00942 $&  0.00098 \\
2454437.61773 &$ 0.01124 $&  0.00098 \\
2454437.61805 &$ 0.01113 $&  0.00097 \\
2454437.61840 &$ 0.01070 $&  0.00099 \\
2454437.61871 &$ 0.00919 $&  0.00098 \\
2454437.61905 &$ 0.00903 $&  0.00098 \\
2454437.61940 &$ 0.00861 $&  0.00097 \\
2454437.61974 &$ 0.00812 $&  0.00097 \\
2454437.62009 &$ 0.00982 $&  0.00097 \\
2454437.62040 &$ 0.00850 $&  0.00098 \\
2454437.62074 &$ 0.01224 $&  0.00099 \\
2454437.62107 &$ 0.01050 $&  0.00099 \\
2454437.62140 &$ 0.01018 $&  0.00097 \\
2454437.62173 &$ 0.01033 $&  0.00098 \\
2454437.62208 &$ 0.00866 $&  0.00097 \\
2454437.62241 &$ 0.00662 $&  0.00097 \\
2454437.62273 &$ 0.01038 $&  0.00098 \\
2454437.62305 &$ 0.00690 $&  0.00100 \\
2454437.62339 &$ 0.00867 $&  0.00098 \\
2454437.62373 &$ 0.01150 $&  0.00098 \\
2454437.62406 &$ 0.01196 $&  0.00097 \\
2454437.62439 &$ 0.00866 $&  0.00098 \\
2454437.62469 &$ 0.01130 $&  0.00098 \\
2454437.62501 &$ 0.01048 $&  0.00098 \\
2454437.62536 &$ 0.01053 $&  0.00098 \\
2454437.62570 &$ 0.01016 $&  0.00098 \\
2454437.62603 &$ 0.01198 $&  0.00098 \\
2454437.62636 &$ 0.00919 $&  0.00098 \\
2454437.62669 &$ 0.01234 $&  0.00105 \\
2454437.62701 &$ 0.00893 $&  0.00098 \\
2454437.62734 &$ 0.00864 $&  0.00100 \\
2454437.62766 &$ 0.01007 $&  0.00098 \\
2454437.62801 &$ 0.01144 $&  0.00098 \\
2454437.62833 &$ 0.01115 $&  0.00098 \\
2454437.62866 &$ 0.00997 $&  0.00097 \\
2454437.62899 &$ 0.01197 $&  0.00097 \\
2454437.62933 &$ 0.01433 $&  0.00097 \\
2454437.62965 &$ 0.01191 $&  0.00098 \\
2454437.63000 &$ 0.01125 $&  0.00097 \\
2454437.63029 &$ 0.01130 $&  0.00097 \\
2454437.63062 &$ 0.01058 $&  0.00097 \\
2454437.63098 &$ 0.01038 $&  0.00096 \\
2454437.63133 &$ 0.01118 $&  0.00097 \\
2454437.63164 &$ 0.00932 $&  0.00097 \\
2454437.63199 &$ 0.01053 $&  0.00097 \\
2454437.63231 &$ 0.00865 $&  0.00097 \\
2454437.63265 &$ 0.00991 $&  0.00097 \\
2454437.63300 &$ 0.01339 $&  0.00097 \\
2454437.63333 &$ 0.01306 $&  0.00097 \\
2454437.63368 &$ 0.01100 $&  0.00097 \\
2454437.63401 &$ 0.01094 $&  0.00097 \\
2454437.63434 &$ 0.01124 $&  0.00096 \\
2454437.63466 &$ 0.00991 $&  0.00096 \\
2454437.63499 &$ 0.01004 $&  0.00097 \\
2454437.63531 &$ 0.01138 $&  0.00097 \\
2454437.63565 &$ 0.01297 $&  0.00098 \\
2454437.63597 &$ 0.01209 $&  0.00097 \\
2454437.63631 &$ 0.01144 $&  0.00098 \\
2454437.63665 &$ 0.01296 $&  0.00097 \\
2454437.63699 &$ 0.01170 $&  0.00098 \\
2454437.63732 &$ 0.01192 $&  0.00098 \\
2454437.63767 &$ 0.01168 $&  0.00097 \\
2454437.63802 &$ 0.01094 $&  0.00098 \\
2454437.63834 &$ 0.01022 $&  0.00097 \\
2454437.63868 &$ 0.01193 $&  0.00098 \\
2454437.63900 &$ 0.01286 $&  0.00100 \\
2454437.63933 &$ 0.01126 $&  0.00098 \\
2454437.63967 &$ 0.01087 $&  0.00098 \\
2454437.64001 &$ 0.01003 $&  0.00098 \\
2454437.64032 &$ 0.00924 $&  0.00098 \\
2454437.64066 &$ 0.01057 $&  0.00099 \\
2454437.64096 &$ 0.01123 $&  0.00097 \\
2454437.64128 &$ 0.01209 $&  0.00098 \\
2454437.64163 &$ 0.01126 $&  0.00098 \\
2454437.64195 &$ 0.01264 $&  0.00097 \\
2454437.64230 &$ 0.01167 $&  0.00097 \\
2454437.64264 &$ 0.00897 $&  0.00099 \\
2454437.64294 &$ 0.01266 $&  0.00099 \\
2454437.64328 &$ 0.01129 $&  0.00098 \\
2454437.64360 &$ 0.00934 $&  0.00098 \\
2454437.64396 &$ 0.01032 $&  0.00098 \\
2454437.64428 &$ 0.01250 $&  0.00097 \\
2454437.64460 &$ 0.00913 $&  0.00098 \\
2454437.64493 &$ 0.01030 $&  0.00097 \\
2454437.64526 &$ 0.01225 $&  0.00098 \\
2454437.64560 &$ 0.01239 $&  0.00097 \\
2454437.64591 &$ 0.01097 $&  0.00097 \\
2454437.64627 &$ 0.01141 $&  0.00097 \\
2454437.64659 &$ 0.01501 $&  0.00098 \\
2454437.64694 &$ 0.01255 $&  0.00099 \\
2454437.64725 &$ 0.01037 $&  0.00098 \\
2454437.64759 &$ 0.01228 $&  0.00097 \\
2454437.64792 &$ 0.00838 $&  0.00097 \\
2454437.64825 &$ 0.01123 $&  0.00099 \\
2454437.64858 &$ 0.01153 $&  0.00099 \\
2454437.64891 &$ 0.00930 $&  0.00098 \\
2454437.64924 &$ 0.01241 $&  0.00099 \\
2454437.64956 &$ 0.01192 $&  0.00097 \\
2454437.64989 &$ 0.00863 $&  0.00098 \\
2454437.65024 &$ 0.00718 $&  0.00098 \\
2454437.65055 &$ 0.01146 $&  0.00098 \\
2454437.65090 &$ 0.00714 $&  0.00100 \\
2454437.65122 &$ 0.01202 $&  0.00098 \\
2454437.65156 &$ 0.00949 $&  0.00098 \\
2454437.65191 &$ 0.00971 $&  0.00097 \\
2454437.65224 &$ 0.01025 $&  0.00097 \\
2454437.65258 &$ 0.01172 $&  0.00097 \\
2454437.65289 &$ 0.01056 $&  0.00098 \\
2454437.65323 &$ 0.00859 $&  0.00097 \\
2454437.65356 &$ 0.00955 $&  0.00098 \\
2454437.65387 &$ 0.01266 $&  0.00098 \\
2454437.65421 &$ 0.00801 $&  0.00098 \\
2454437.65455 &$ 0.00800 $&  0.00097 \\
2454437.65488 &$ 0.00825 $&  0.00098 \\
2454437.65523 &$ 0.01230 $&  0.00097 \\
2454437.65556 &$ 0.00894 $&  0.00097 \\
2454437.65590 &$ 0.00994 $&  0.00098 \\
2454437.65621 &$ 0.01199 $&  0.00098 \\
2454437.65656 &$ 0.01003 $&  0.00099 \\
2454437.65688 &$ 0.00873 $&  0.00098 \\
2454437.65719 &$ 0.01051 $&  0.00099 \\
2454437.65752 &$ 0.01290 $&  0.00099 \\
2454437.65787 &$ 0.01182 $&  0.00098 \\
2454437.65819 &$ 0.00961 $&  0.00098 \\
2454437.65851 &$ 0.01238 $&  0.00100 \\
2454437.65886 &$ 0.01030 $&  0.00101 \\
2454437.65921 &$ 0.01274 $&  0.00098 \\
2454437.65953 &$ 0.01109 $&  0.00098 \\
2454437.65988 &$ 0.01270 $&  0.00098 \\
2454437.66022 &$ 0.00882 $&  0.00098 \\
2454437.66056 &$ 0.01288 $&  0.00100 \\
2454437.66089 &$ 0.00996 $&  0.00099 \\
2454437.66122 &$ 0.01132 $&  0.00098 \\
2454437.66155 &$ 0.01068 $&  0.00098 \\
2454437.66188 &$ 0.01204 $&  0.00098 \\
2454437.66222 &$ 0.01037 $&  0.00097 \\
2454437.66254 &$ 0.01244 $&  0.00097 \\
2454437.66288 &$ 0.01097 $&  0.00097 \\
2454437.66320 &$ 0.01030 $&  0.00098 \\
2454437.66354 &$ 0.01149 $&  0.00098 \\
2454437.66386 &$ 0.01189 $&  0.00099 \\
2454437.66421 &$ 0.01029 $&  0.00099 \\
2454437.66454 &$ 0.00895 $&  0.00098 \\
2454437.66488 &$ 0.01146 $&  0.00097 \\
2454437.66522 &$ 0.01105 $&  0.00098 \\
2454437.66555 &$ 0.00990 $&  0.00097 \\
2454437.66589 &$ 0.01173 $&  0.00098 \\
2454437.66623 &$ 0.01003 $&  0.00099 \\
2454437.66657 &$ 0.01132 $&  0.00100 \\
2454437.66689 &$ 0.01002 $&  0.00099 \\
2454437.66722 &$ 0.01115 $&  0.00098 \\
2454437.66757 &$ 0.01074 $&  0.00098 \\
2454437.66789 &$ 0.01270 $&  0.00099 \\
2454437.66824 &$ 0.01324 $&  0.00100 \\
2454437.66853 &$ 0.01356 $&  0.00099 \\
2454437.66887 &$ 0.01014 $&  0.00099 \\
2454437.66920 &$ 0.01059 $&  0.00097 \\
2454437.66952 &$ 0.01170 $&  0.00098 \\
2454437.66988 &$ 0.01144 $&  0.00099 \\
2454437.67020 &$ 0.01278 $&  0.00099 \\
2454437.67053 &$ 0.00970 $&  0.00100 \\
2454437.67084 &$ 0.01041 $&  0.00100 \\
2454437.67119 &$ 0.01314 $&  0.00099 \\
2454437.67153 &$ 0.01316 $&  0.00101 \\
2454437.67186 &$ 0.01454 $&  0.00100 \\
2454437.67221 &$ 0.01358 $&  0.00099 \\
2454437.67252 &$ 0.01255 $&  0.00100 \\
2454437.67284 &$ 0.01127 $&  0.00101 \\
2454437.67318 &$ 0.01254 $&  0.00102 \\
2454437.67354 &$ 0.01080 $&  0.00103 \\
2454437.67386 &$ 0.01304 $&  0.00101 \\
2454437.67420 &$ 0.01310 $&  0.00102 \\
2454437.67452 &$ 0.01368 $&  0.00100 \\
2454437.67486 &$ 0.00969 $&  0.00098 \\
2454437.67520 &$ 0.01020 $&  0.00098 \\
2454437.67556 &$ 0.01500 $&  0.00099 \\
2454437.67591 &$ 0.01204 $&  0.00099 \\
2454437.67623 &$ 0.00998 $&  0.00097 \\
2454437.67657 &$ 0.00996 $&  0.00097 \\
2454437.67690 &$ 0.01276 $&  0.00098 \\
2454437.67724 &$ 0.01099 $&  0.00097 \\
2454437.67756 &$ 0.01467 $&  0.00099 \\
2454437.67790 &$ 0.01147 $&  0.00097 \\
2454437.67822 &$ 0.00964 $&  0.00099 \\
2454437.67855 &$ 0.01072 $&  0.00098 \\
2454437.67887 &$ 0.01405 $&  0.00098 \\
2454437.67924 &$ 0.01038 $&  0.00098 \\
2454437.67957 &$ 0.01234 $&  0.00099 \\
2454437.67990 &$ 0.01293 $&  0.00097 \\
2454437.68023 &$ 0.00742 $&  0.00097 \\
2454437.68057 &$ 0.00845 $&  0.00099 \\
2454437.68090 &$ 0.00790 $&  0.00098 \\
2454437.68122 &$ 0.01054 $&  0.00099 \\
2454437.68155 &$ 0.01064 $&  0.00098 \\
2454437.68189 &$ 0.01272 $&  0.00098 \\
2454437.68223 &$ 0.01240 $&  0.00098 \\
2454437.68256 &$ 0.01047 $&  0.00099 \\
2454437.68289 &$ 0.00891 $&  0.00099 \\
2454437.68322 &$ 0.01514 $&  0.00098 \\
2454437.68355 &$ 0.00877 $&  0.00098 \\
2454437.68386 &$ 0.01037 $&  0.00099 \\
2454437.68421 &$ 0.01120 $&  0.00097 \\
2454437.68452 &$ 0.01328 $&  0.00097 \\
2454437.68486 &$ 0.01304 $&  0.00097 \\
2454437.68519 &$ 0.01258 $&  0.00098 \\
2454437.68554 &$ 0.00884 $&  0.00097 \\
2454437.68587 &$ 0.01249 $&  0.00098 \\
2454437.68623 &$ 0.01237 $&  0.00100 \\
2454437.68654 &$ 0.01107 $&  0.00100 \\
2454437.68689 &$ 0.01347 $&  0.00099 \\
2454437.68720 &$ 0.01312 $&  0.00105 \\
2454437.68756 &$ 0.01429 $&  0.00105 \\
2454437.68789 &$ 0.01040 $&  0.00100 \\
2454437.68823 &$ 0.01080 $&  0.00102 \\
2454437.68856 &$ 0.01181 $&  0.00100 \\
2454437.68888 &$ 0.01079 $&  0.00101 \\
2454437.68923 &$ 0.01041 $&  0.00101 \\
2454437.68958 &$ 0.01194 $&  0.00101 \\
2454437.68992 &$ 0.00868 $&  0.00099 \\
2454437.69025 &$ 0.01229 $&  0.00107 \\
2454437.69058 &$ 0.01137 $&  0.00100 \\
2454437.69090 &$ 0.01037 $&  0.00100 \\
2454437.69124 &$ 0.01148 $&  0.00100 \\
2454437.69159 &$ 0.01410 $&  0.00104 \\
2454437.69191 &$ 0.00817 $&  0.00101 \\
2454437.69226 &$ 0.01196 $&  0.00098 \\
2454437.69260 &$ 0.01428 $&  0.00104 \\
2454437.69296 &$ 0.01192 $&  0.00102 \\
2454437.69327 &$ 0.00965 $&  0.00101 \\
2454437.69362 &$ 0.01103 $&  0.00099 \\
2454437.69394 &$ 0.00935 $&  0.00100 \\
2454437.69429 &$ 0.01097 $&  0.00101 \\
2454437.69461 &$ 0.01011 $&  0.00098 \\
2454437.69496 &$ 0.01004 $&  0.00099 \\
2454437.69528 &$ 0.01209 $&  0.00098 \\
2454437.69562 &$ 0.01057 $&  0.00099 \\
2454437.69594 &$ 0.01168 $&  0.00099 \\
2454437.69630 &$ 0.01153 $&  0.00104 \\
2454437.69663 &$ 0.00936 $&  0.00101 \\
2454437.69695 &$ 0.01048 $&  0.00100 \\
2454437.69730 &$ 0.00962 $&  0.00101 \\
2454437.69762 &$ 0.01125 $&  0.00103 \\
2454437.69794 &$ 0.01222 $&  0.00099 \\
2454437.69827 &$ 0.01288 $&  0.00101 \\
2454437.69862 &$ 0.01119 $&  0.00104 \\
2454437.69893 &$ 0.01060 $&  0.00106 \\
2454437.69926 &$ 0.01204 $&  0.00102 \\
2454437.69961 &$ 0.01211 $&  0.00104 \\
2454437.69995 &$ 0.01047 $&  0.00102 \\
2454437.70028 &$ 0.01031 $&  0.00101 \\
2454437.70062 &$ 0.01262 $&  0.00101 \\
2454437.70095 &$ 0.01009 $&  0.00102 \\
2454437.70128 &$ 0.01185 $&  0.00099 \\
2454437.70160 &$ 0.01070 $&  0.00099 \\
2454437.70193 &$ 0.00936 $&  0.00101 \\
2454437.70228 &$ 0.01224 $&  0.00102 \\
2454437.70260 &$ 0.00892 $&  0.00100 \\
2454437.70293 &$ 0.01274 $&  0.00101 \\
2454437.70326 &$ 0.01192 $&  0.00100 \\
2454437.70360 &$ 0.01108 $&  0.00100 \\
2454437.70394 &$ 0.01276 $&  0.00100 \\
2454437.70426 &$ 0.01055 $&  0.00100 \\
2454437.70460 &$ 0.01205 $&  0.00105 \\
2454437.70495 &$ 0.00750 $&  0.00100 \\
2454437.70527 &$ 0.01329 $&  0.00101 \\
2454437.70562 &$ 0.00898 $&  0.00104 \\
2454437.70594 &$ 0.01231 $&  0.00107 \\
2454437.70629 &$ 0.00940 $&  0.00101 \\
2454437.70662 &$ 0.01134 $&  0.00100 \\
2454437.70695 &$ 0.01110 $&  0.00100 \\
2454437.70730 &$ 0.00555 $&  0.00102 \\
2454437.70763 &$ 0.01116 $&  0.00100 \\
2454437.70794 &$ 0.00673 $&  0.00100 \\
2454437.70829 &$ 0.00650 $&  0.00103 \\
2454437.70862 &$ 0.00598 $&  0.00106 \\
2454437.70896 &$ 0.00732 $&  0.00104 \\
2454437.70930 &$ 0.01358 $&  0.00103 \\
2454437.70962 &$ 0.01059 $&  0.00101 \\
2454437.70997 &$ 0.01212 $&  0.00100 \\
2454437.71029 &$ 0.01076 $&  0.00102 \\
2454437.71064 &$ 0.00879 $&  0.00101 \\
2454437.71099 &$ 0.01361 $&  0.00100 \\
2454437.71131 &$ 0.01302 $&  0.00102 \\
2454437.71165 &$ 0.00699 $&  0.00101 \\
2454437.71199 &$ 0.01297 $&  0.00103 \\
2454437.71235 &$ 0.01035 $&  0.00101 \\
2454437.71269 &$ 0.01078 $&  0.00099 \\
2454437.71302 &$ 0.01027 $&  0.00102 \\
2454437.71335 &$ 0.00925 $&  0.00104 \\
2454437.71370 &$ 0.01295 $&  0.00101 \\
2454437.71404 &$ 0.00940 $&  0.00104 \\
2454437.71437 &$ 0.01154 $&  0.00102 \\
2454437.71470 &$ 0.01268 $&  0.00104 \\
2454437.71505 &$ 0.00947 $&  0.00103 \\
2454437.71539 &$ 0.00970 $&  0.00103 \\
2454437.71572 &$ 0.00902 $&  0.00102 \\
2454437.71606 &$ 0.01183 $&  0.00101 \\
2454437.71638 &$ 0.00457 $&  0.00101 \\
2454437.71668 &$ 0.01253 $&  0.00103 \\
2454437.71702 &$ 0.00611 $&  0.00103 \\
2454437.71734 &$ 0.00831 $&  0.00104 \\
2454437.71767 &$ 0.00993 $&  0.00106 \\
2454437.71800 &$ 0.00375 $&  0.00104 \\
2454437.71831 &$ 0.00662 $&  0.00106 \\
2454437.71864 &$ 0.01375 $&  0.00108 \\
2454437.71897 &$ 0.01479 $&  0.00102 \\
2454437.71931 &$ 0.00759 $&  0.00102 \\
2454437.71963 &$ 0.00604 $&  0.00105 \\
2454437.71997 &$ 0.01072 $&  0.00099 \\
2454437.72029 &$ 0.00940 $&  0.00102 \\
2454437.72062 &$ 0.01156 $&  0.00101 \\
2454437.72094 &$ 0.00899 $&  0.00103 \\
2454437.72126 &$ 0.00822 $&  0.00103 \\
2454437.72159 &$ 0.01240 $&  0.00099 \\
2454437.72194 &$ 0.01249 $&  0.00102 \\
2454437.72227 &$ 0.00723 $&  0.00101 \\
2454437.72262 &$ 0.01300 $&  0.00120 \\
2454437.72295 &$ 0.00792 $&  0.00106 \\
2454437.72328 &$ 0.00827 $&  0.00101 \\
2454437.72360 &$ 0.01242 $&  0.00100 \\
2454437.72394 &$ 0.00819 $&  0.00102 \\
2454437.72429 &$ 0.00907 $&  0.00101 \\
2454437.72461 &$ 0.01124 $&  0.00101 \\
2454437.72494 &$ 0.01275 $&  0.00102 \\
2454437.72528 &$ 0.01406 $&  0.00109 \\
2454437.72563 &$ 0.01125 $&  0.00101 \\
2454437.72596 &$ 0.00588 $&  0.00102 \\
2454437.72629 &$ 0.00717 $&  0.00107 \\
2454437.72661 &$ 0.00882 $&  0.00101 \\
2454437.72693 &$ 0.00647 $&  0.00105 \\
2454437.72728 &$ 0.00595 $&  0.00100 \\
2454437.72759 &$ 0.01016 $&  0.00100 \\
2454437.72795 &$ 0.00983 $&  0.00103 \\
2454437.72828 &$ 0.00806 $&  0.00100 \\
2454437.72860 &$ 0.01130 $&  0.00104 \\
2454437.72895 &$ 0.00579 $&  0.00102 \\
2454437.72927 &$ 0.00596 $&  0.00099 \\
2454437.72961 &$ 0.01246 $&  0.00101 \\
2454437.72993 &$ 0.00801 $&  0.00103 \\
2454437.73028 &$ 0.01331 $&  0.00103 \\
2454437.73063 &$ 0.01313 $&  0.00103 \\
2454437.73095 &$ 0.01258 $&  0.00107 \\
2454437.73129 &$ 0.00952 $&  0.00101 \\
2454437.73162 &$ 0.01418 $&  0.00104 \\
2454437.73195 &$ 0.00927 $&  0.00098 \\
2454437.73227 &$ 0.01267 $&  0.00100 \\
2454437.73261 &$ 0.01089 $&  0.00101 \\
2454437.73294 &$ 0.01060 $&  0.00100 \\
2454437.73329 &$ 0.00809 $&  0.00110 \\
2454437.73360 &$ 0.00825 $&  0.00110 \\
2454437.73395 &$ 0.00652 $&  0.00102 \\
2454437.73427 &$ 0.00939 $&  0.00098 \\
2454437.73460 &$ 0.01364 $&  0.00099 \\
2454437.73494 &$ 0.00691 $&  0.00099 \\
2454437.73530 &$ 0.00577 $&  0.00101 \\
2454437.73563 &$ 0.00667 $&  0.00101 \\
2454437.73597 &$ 0.01121 $&  0.00101 \\
2454437.73629 &$ 0.00767 $&  0.00097 \\
2454437.73662 &$ 0.01562 $&  0.00099 \\
2454437.73695 &$ 0.01222 $&  0.00099 \\
2454437.73729 &$ 0.00688 $&  0.00098 \\
2454437.73763 &$ 0.00831 $&  0.00102 \\
2454437.73795 &$ 0.00944 $&  0.00108 \\
2454437.73829 &$ 0.00921 $&  0.00105 \\
2454437.73864 &$ 0.00632 $&  0.00098 \\
2454437.73895 &$ 0.00917 $&  0.00098 \\
2454437.73928 &$ 0.01181 $&  0.00100 \\
2454437.73961 &$ 0.00303 $&  0.00098 \\
2454437.73995 &$ 0.00146 $&  0.00099 \\
2454437.74029 &$ 0.00783 $&  0.00099 \\
2454437.74064 &$ 0.01021 $&  0.00100 \\
2454437.74100 &$ 0.01091 $&  0.00099 \\
2454437.74136 &$ 0.01140 $&  0.00103 \\
2454437.74170 &$ 0.00602 $&  0.00099 \\
2454437.74204 &$ 0.01105 $&  0.00101 \\
2454437.74242 &$ 0.00438 $&  0.00100 \\
2454437.74276 &$ 0.00649 $&  0.00101 \\
2454437.74308 &$ 0.01239 $&  0.00109 \\
2454437.74342 &$ 0.00364 $&  0.00100 \\
2454437.74374 &$ 0.00609 $&  0.00103 \\
2454437.74410 &$ 0.00898 $&  0.00103 \\
2454437.74442 &$ 0.00487 $&  0.00111 \\
2454437.74476 &$ 0.00847 $&  0.00101 \\
2454437.74511 &$ 0.00910 $&  0.00104 \\
2454437.74542 &$ 0.01015 $&  0.00115 \\
2454437.74574 &$ 0.00482 $&  0.00107 \\
2454437.74609 &$ 0.00125 $&  0.00117 \\
2454437.74642 &$ 0.00623 $&  0.00103 \\
2454437.74675 &$ 0.00459 $&  0.00104 \\
2454437.74706 &$ 0.00544 $&  0.00106 \\
2454437.74741 &$ 0.00845 $&  0.00107 \\
2454437.74772 &$ 0.00951 $&  0.00102 \\
2454437.74805 &$ 0.00484 $&  0.00105 \\
2454437.74837 &$ 0.00523 $&  0.00108 \\
2454437.74870 &$ 0.00655 $&  0.00103 \\
2454437.74904 &$ 0.00470 $&  0.00110 \\
2454437.74939 &$ 0.00707 $&  0.00106 \\
2454437.74971 &$ 0.00853 $&  0.00106 \\
2454437.75005 &$ 0.00151 $&  0.00105 \\
2454437.75037 &$ 0.00409 $&  0.00109 \\
2454437.75072 &$ 0.00400 $&  0.00102 \\
2454437.75105 &$-0.00410 $&  0.00115 \\
2454437.75138 &$ 0.00489 $&  0.00105 \\
2454437.75171 &$ 0.00136 $&  0.00103 \\
2454437.75203 &$ 0.00551 $&  0.00105 \\
2454437.75237 &$ 0.00256 $&  0.00102 \\
2454437.75269 &$ 0.00288 $&  0.00106 \\
2454437.75303 &$ 0.00184 $&  0.00102 \\
2454437.75337 &$-0.00314 $&  0.00109 \\
2454437.75369 &$ 0.00231 $&  0.00117 \\
2454437.75403 &$-0.00000 $&  0.00109 \\
2454437.75435 &$ 0.00490 $&  0.00103 \\
2454437.75470 &$ 0.00203 $&  0.00105 \\
2454437.75502 &$ 0.00137 $&  0.00105 \\
2454437.75537 &$-0.00082 $&  0.00103 \\
2454437.75571 &$-0.00071 $&  0.00102 \\
2454437.75603 &$ 0.00200 $&  0.00105 \\
2454437.75635 &$-0.00403 $&  0.00105 \\
2454437.75669 &$-0.00325 $&  0.00110 \\
2454437.75704 &$-0.00330 $&  0.00115 \\
2454437.75736 &$-0.00181 $&  0.00110 \\
2454437.75771 &$-0.00044 $&  0.00107 \\
2454437.75803 &$ 0.00091 $&  0.00104 \\
2454437.75838 &$-0.00790 $&  0.00105 \\
2454437.75868 &$ 0.00030 $&  0.00104 \\
2454437.75904 &$-0.00078 $&  0.00106 \\
2454437.75938 &$-0.00229 $&  0.00105 \\
2454437.75971 &$-0.00003 $&  0.00103 \\
2454437.76003 &$-0.00285 $&  0.00102 \\
2454437.76039 &$-0.00012 $&  0.00107 \\
2454437.76071 &$-0.00029 $&  0.00105 \\
2454437.76104 &$ 0.00048 $&  0.00105 \\
2454437.76137 &$-0.00285 $&  0.00109 \\
2454437.76170 &$ 0.00156 $&  0.00112 \\
2454437.76204 &$-0.00184 $&  0.00106 \\
2454437.76237 &$ 0.00051 $&  0.00105 \\
2454437.76270 &$ 0.00224 $&  0.00104 \\
2454437.76302 &$ 0.00526 $&  0.00106 \\
2454437.76337 &$ 0.00458 $&  0.00105 \\
2454437.76372 &$-0.00008 $&  0.00105 \\
2454437.76403 &$ 0.00523 $&  0.00106 \\
2454437.76438 &$-0.00057 $&  0.00111 \\
2454437.76473 &$ 0.00700 $&  0.00108 \\
2454437.76508 &$ 0.00086 $&  0.00102 \\
2454437.76539 &$-0.00284 $&  0.00103 \\
2454437.76574 &$-0.00537 $&  0.00108 \\
2454437.76605 &$-0.00571 $&  0.00106 \\
2454437.76636 &$-0.00117 $&  0.00109 \\
2454437.76670 &$ 0.00206 $&  0.00126 \\
2454437.76705 &$-0.00255 $&  0.00126 \\
2454437.76737 &$ 0.00336 $&  0.00110 \\
2454437.76771 &$ 0.01020 $&  0.00113 \\
2454437.76804 &$ 0.00176 $&  0.00108 \\
2454437.76834 &$ 0.00166 $&  0.00108 \\
2454437.76868 &$ 0.00406 $&  0.00106 \\
2454437.76902 &$ 0.00475 $&  0.00103 \\
2454437.76934 &$-0.00111 $&  0.00105 \\
2454437.76970 &$ 0.00023 $&  0.00109 \\
2454437.77002 &$ 0.00861 $&  0.00114 \\
2454437.77037 &$ 0.00547 $&  0.00115 \\
2454437.77071 &$-0.00603 $&  0.00116 \\
2454437.77102 &$-0.00172 $&  0.00109 \\
\enddata
\label{tab:keplercam}
\tablecomments{
column (1): Barycentric Julian Day, \\
column (2): Best detrended KeplerCam $z$ magnitude, normalized to 0.0 out of transit, \\
column (3): Estimated error in the best magnitude.}
\tablecomments{
Table 10 is presented in its entirety in the electronic edition
of the Astrophysical Journal. A portion is shown here for guidance
regarding its form and content.} \\
\end{deluxetable}


==> tab2.tex <==
\begin{deluxetable}{llllrr}
\tabletypesize{\scriptsize}
\tablewidth{0pc}
\tablenum{2}\tablecaption{Single-Lined Radial Velocities \label{tab2}}
\tablehead{
\colhead{~~~~~Star~~~~~~~~~~} &
\colhead{Tel} &
\colhead{Template} &
\colhead{HJD} &
\colhead{$V_{\rm A}$} &
\colhead{$\sigma(V_{\rm A})$}}
\startdata
HTR205-001 & T & t10000g45p00v008 & 2453158.90513 &   -2.58 &  0.65 \\
HTR205-001 & T & t10000g45p00v008 & 2453161.96505 &   -2.75 &  0.58 \\
HTR205-001 & W & t10000g45p00v008 & 2453183.82621 &   -2.19 &  1.17 \\
HTR205-002 & W & t05000g30p00v000 & 2453137.83494 &  -27.03 &  0.27 \\
HTR205-002 & W & t05000g30p00v000 & 2453154.80255 &  -27.06 &  0.28 \\
HTR205-002 & W & t05000g30p00v000 & 2453180.82534 &  -26.76 &  0.26 \\
HTR205-003 & T & t06500g45p00v030 & 2453162.91121 &  -23.55 &  1.27 \\
HTR205-003 & T & t06500g45p00v030 & 2453183.95068 &  -67.55 &  1.48 \\
HTR205-003 & T & t06500g45p00v030 & 2453511.95989 &   -1.53 &  2.43 \\
HTR205-003 & T & t06500g45p00v030 & 2453513.96752 &   -3.18 &  1.94 \\
HTR205-003 & T & t06500g45p00v030 & 2453514.94885 &  -55.09 &  2.27 \\
HTR205-003 & T & t06500g45p00v030 & 2453515.97011 &  -17.78 &  1.75 \\
HTR205-003 & T & t06500g45p00v030 & 2453541.91282 &  -42.91 &  1.79 \\
HTR205-003 & T & t06500g45p00v030 & 2453576.91339 &  -26.83 &  1.64 \\
HTR205-003 & T & t06500g45p00v030 & 2453626.78164 &  -53.09 &  1.34 \\
HTR205-003 & T & t06500g45p00v030 & 2453631.71182 &   -2.72 &  1.05 \\
HTR205-003 & T & t06500g45p00v030 & 2453663.74912 &  -57.87 &  1.48 \\
HTR205-003 & T & t06500g45p00v030 & 2453665.76621 &  -67.58 &  1.56 \\
HTR205-003 & T & t06500g45p00v030 & 2453666.75540 &   -1.75 &  1.82 \\
HTR205-003 & T & t06500g45p00v030 & 2453688.66899 &   -2.68 &  1.52 \\
HTR205-003 & T & t06500g45p00v030 & 2453692.70727 &   -7.06 &  1.46 \\
HTR205-003 & T & t06500g45p00v030 & 2453989.84385 &  -39.55 &  1.76 \\
HTR205-003 & T & t06500g45p00v030 & 2454042.67398 &  -70.63 &  3.33 \\
HTR205-005 & T & t06750g35p00v060 & 2453162.95313 &   10.68 &  4.14 \\
HTR205-005 & T & t06750g35p00v060 & 2453187.92272 &  -42.97 &  8.20 \\
HTR205-006 & T & t04500g25p00v000 & 2453187.93435 &  -51.02 &  0.30 \\
HTR205-006 & T & t04500g25p00v000 & 2453692.72147 &  -51.77 &  0.26 \\
HTR205-007W & T & t06250g40p00v050 & 2453187.90941 &  -0.72 &  1.75 \\
HTR205-007W & T & t06250g40p00v050 & 2453189.89866 &  -3.78 &  3.46 \\
HTR205-007W & T & t06250g40p00v050 & 2453684.74920 &  -1.52 &  3.04 \\
HTR205-007W & T & t06250g40p00v050 & 2453926.90323 & -63.86 &  2.37 \\
HTR205-007E & T & t06000g40p00v008 & 2453187.90941 & -35.49 &  0.79 \\
HTR205-007E & T & t06000g40p00v008 & 2453189.90974 & -36.98 &  0.75 \\
HTR205-008 & T & t04750g25p00v002 & 2453161.95728 &   31.86 &  0.21 \\
HTR205-008 & T & t04750g25p00v002 & 2453163.97192 &   31.63 &  0.23 \\
HTR205-008 & W & t04750g25p00v002 & 2453184.82076 &   31.43 &  0.40 \\
HTR205-009 & T & t05750g35p00v120 & 2453686.69865 &    2.56 &  5.14 \\
HTR205-013 & W & t06250g40p00v030 & 2453034.45642 &   -2.02 &  1.38 \\
HTR205-013 & W & t06250g40p00v030 & 2453035.47574 &  -10.11 &  1.61 \\
HTR205-013 & T & t06250g40p00v030 & 2453035.58018 &  -18.52 &  1.01 \\
HTR205-013 & W & t06250g40p00v030 & 2453036.48778 &  -12.93 &  1.53 \\
HTR205-013 & W & t06250g40p00v030 & 2453037.46565 &   -0.47 &  1.43 \\
HTR205-013 & T & t06250g40p00v030 & 2453037.61215 &   -6.83 &  0.91 \\
HTR205-013 & W & t06250g40p00v030 & 2453038.46413 &  -25.72 &  1.48 \\
HTR205-013 & T & t06250g40p00v030 & 2453038.57874 &  -19.76 &  1.15 \\
HTR205-013 & W & t06250g40p00v030 & 2453040.47360 &  -28.58 &  1.24 \\
HTR205-013 & T & t06250g40p00v030 & 2453042.58686 &  -27.79 &  0.91 \\
HTR205-013 & T & t06250g40p00v030 & 2453043.58338 &    4.84 &  1.23 \\
HTR205-013 & T & t06250g40p00v030 & 2453044.58422 &  -19.73 &  1.14 \\
HTR205-013 & T & t06250g40p00v030 & 2453045.57911 &   -6.42 &  0.73 \\
HTR205-013 & W & t06250g40p00v030 & 2453046.46373 &   -2.11 &  0.80 \\
HTR205-013 & T & t06250g40p00v030 & 2453046.60000 &  -10.47 &  0.77 \\
HTR205-013 & W & t06250g40p00v030 & 2453047.50881 &  -20.45 &  1.49 \\
HTR205-013 & T & t06250g40p00v030 & 2453047.58731 &  -14.83 &  0.95 \\
HTR205-013 & T & t06250g40p00v030 & 2453543.94910 &   -4.01 &  1.10 \\
HTR205-013 & T & t06250g40p00v030 & 2453658.69572 &  -20.53 &  1.16 \\
HTR205-013 & T & t06250g40p00v030 & 2453659.75967 &    3.14 &  2.28 \\
HTR205-013 & T & t06250g40p00v030 & 2453659.78398 &    2.85 &  1.09 \\
HTR205-013 & T & t06250g40p00v030 & 2453660.70213 &  -25.98 &  1.57 \\
HTR205-013 & T & t06250g40p00v030 & 2453664.70202 &  -19.39 &  1.21 \\
HTR205-014 & W & t07500g35p00v000 & 2453155.79810 &  550.28 &  1.51 \\
HTR205-014 & T & t07500g35p00v000 & 2453186.98181 &   23.28 &  2.33 \\
HTR205-015 & T & t05250g30p00v002 & 2453689.77673 &  -42.47 &  0.40 \\
HTR205-015 & T & t05250g30p00v002 & 2454075.66325 &  -42.82 &  0.44 \\
HTR205-016 & T & t04500g25p00v000 & 2453187.96376 &  -29.86 &  0.38 \\
HTR205-016 & W & t04500g25p00v000 & 2453240.74690 &  -30.00 &  0.38 \\
HTR205-016 & T & t04500g25p00v000 & 2453692.75399 &  -30.29 &  0.31 \\
HTR205-018 & T & t06000g40p00v006 & 2453187.95843 &  -22.93 &  0.73 \\
HTR205-018 & T & t06000g40p00v006 & 2453214.93425 &  -23.13 &  0.39 \\
HTR205-018 & T & t06000g40p00v006 & 2453271.77454 &  -22.65 &  0.36 \\
HTR205-018 & T & t06000g40p00v006 & 2453279.71519 &  -23.39 &  0.38 \\
HTR205-018 & T & t06000g40p00v006 & 2453302.64311 &  -23.20 &  0.38 \\
HTR205-019 & T & t04750g30p00v000 & 2453186.94607 &  -13.49 &  0.38 \\
HTR205-019 & T & t04750g30p00v000 & 2453189.94645 &  -16.97 &  0.38 \\
HTR205-019 & T & t04750g30p00v000 & 2453213.95865 &  -39.59 &  0.37 \\
HTR205-019 & T & t04750g30p00v000 & 2453689.76737 &  -42.30 &  0.42 \\
HTR205-019 & T & t04750g30p00v000 & 2453989.87514 &  -54.48 &  0.40 \\
HTR205-019 & T & t04750g30p00v000 & 2454012.84775 &  -56.04 &  0.40 \\
HTR205-019 & T & t04750g30p00v000 & 2454019.81148 &  -34.50 &  0.33 \\
HTR205-019 & T & t04750g30p00v000 & 2454042.74672 &  -21.19 &  0.35 \\
HTR205-019 & T & t04750g30p00v000 & 2454047.65410 &  -25.92 &  0.28 \\
HTR205-019 & T & t04750g30p00v000 & 2454049.65043 &  -27.60 &  0.29 \\
HTR205-021 & T & t06000g45p00v000 & 2453184.96679 &  -28.41 &  0.36 \\
HTR205-021 & T & t06000g45p00v000 & 2453186.92432 &  -30.11 &  0.40 \\
HTR205-021 & T & t06000g45p00v000 & 2453187.90176 &  -30.70 &  0.42 \\
HTR205-021 & T & t06000g45p00v000 & 2453189.95167 &  -31.58 &  0.31 \\
HTR205-021 & T & t06000g45p00v000 & 2453684.68435 &    9.56 &  0.36 \\
HTR205-021 & T & t06000g45p00v000 & 2453685.55876 &    9.15 &  0.37 \\
HTR205-021 & T & t06000g45p00v000 & 2453689.65051 &    8.42 &  0.46 \\
HTR205-021 & T & t06000g45p00v000 & 2453694.63598 &    6.55 &  0.52 \\
HTR205-021 & T & t06000g45p00v000 & 2453898.93278 &    8.73 &  0.49 \\
HTR205-021 & T & t06000g45p00v000 & 2453989.82374 &  -28.24 &  0.43 \\
HTR205-021 & T & t06000g45p00v000 & 2454075.62738 &  -15.65 &  0.39 \\
HTR205-021 & T & t06000g45p00v000 & 2454104.59186 &  -26.39 &  0.40 \\
HTR205-022 & T & t06000g40p00v008 & 2453514.96503 &   -3.51 &  0.38 \\
HTR205-022 & T & t06000g40p00v008 & 2453515.98345 &   -3.27 &  0.37 \\
HTR205-022 & T & t06000g40p00v008 & 2453516.96912 &   -3.64 &  0.37 \\
HTR205-022 & T & t06000g40p00v008 & 2453543.93564 &   -3.76 &  0.36 \\
HTR205-022 & T & t06000g40p00v008 & 2453546.96213 &   -2.87 &  0.49 \\
HTR205-022 & T & t06000g40p00v008 & 2453748.59467 &   -3.53 &  0.44 \\
HTR205-023 & T & t05750g40p00v001 & 2453514.96793 &   -2.58 &  0.23 \\
HTR205-023 & T & t05750g40p00v001 & 2453515.98136 &   -3.20 &  0.52 \\
HTR205-023 & T & t05750g40p00v001 & 2453516.97219 &   -3.00 &  0.44 \\
HTR205-023 & T & t05750g40p00v001 & 2453543.94000 &   -2.81 &  0.31 \\
HTR205-023 & T & t05750g40p00v001 & 2453546.96743 &   -2.18 &  0.55 \\
HTR205-023 & T & t05750g40p00v001 & 2453748.59832 &   -3.83 &  0.39 \\
HTR205-024 & T & t06250g40p00v012 & 2453747.60878 &  -22.51 &  0.68 \\
HTR205-024 & T & t06250g40p00v012 & 2453752.60888 &  -22.90 &  0.53 \\
HTR205-024 & T & t06250g40p00v012 & 2453898.95199 &  -21.10 &  0.64 \\
HTR205-024 & T & t06250g40p00v012 & 2454016.62714 &  -23.67 &  0.55 \\
HTR205-024 & T & t06250g40p00v012 & 2454042.68540 &  -22.08 &  0.48 \\
HTR205-024 & T & t06250g40p00v012 & 2454075.65687 &  -22.39 &  0.49 \\
HTR205-024 & T & t06250g40p00v012 & 2454104.59826 &  -22.20 &  0.57 \\
HTR205-025 & T & t04750g25p00v001 & 2453748.58615 &  -42.82 &  0.30 \\
HTR205-025 & T & t04750g25p00v001 & 2453752.57411 &  -42.44 &  0.26 \\
HTR205-026 & T & t05750g40p00v000 & 2453752.59184 &  -17.38 &  0.30 \\
HTR205-026 & T & t05750g40p00v000 & 2453989.83028 &  -17.40 &  0.46 \\
HTR205-026 & T & t05750g40p00v000 & 2454042.65984 &  -17.19 &  0.45 \\
HTR205-026 & T & t05750g40p00v000 & 2454045.70499 &  -17.97 &  0.54 \\
HTR205-030 & T & t05500g40p00v004 & 2454423.68630 &  -23.91 &  0.47 \\
HTR205-030 & T & t05500g40p00v004 & 2454458.62883 &  -24.82 &  0.45 \\
HTR205-030 & T & t05500g40p00v004 & 2454486.60826 &  -22.80 &  0.68 \\
HTR205-030 & T & t05500g40p00v004 & 2454637.95048 &  -23.12 &  0.54 \\
\enddata
\tablecomments{
column (1): HATNet transiting-planet candidate designation, \\
column (2): telescope (W=Wyeth, T=Tillinghast), \\
column (3): template (see text for code), \\
column (4): heliocentric Julian date, \\
column (5): heliocentric radial velocity (\kms), \\
column (6): radial velocity error estimate (\kms), \\}
\tablecomments{
This table is presented in its entirety in the electronic edition of the Astrophysical Journal.
A portion is shown here for guidance regarding its form and content.}
\end{deluxetable}

==> tab3.tex <==
\begin{deluxetable}{llllrr}
\tabletypesize{\scriptsize}
\tablewidth{0pc}
\tablenum{3}\tablecaption{Double-Lined Radial Velocities \label{tab3}}
\tablehead{
\colhead{~~~~~Star~~~~~~~~~~} &
\colhead{Template A}     &
\colhead{Template B}     &
\colhead{HJD}            &
\colhead{$V_{\rm A}$}    &
\colhead{$V_{\rm B}$}}
\startdata
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453162.9343 &  -41.09 &  -16.87 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453183.9643 &   22.52 &  -83.60 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453188.9069 &   45.65 & -102.90 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453684.6943 &   37.57 & -102.34 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453689.6640 &    5.36 &  -72.24 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453694.6542 &  -23.91 &  -36.67 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453714.6282 &  -97.31 &   39.29 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453746.5850 &  -41.46 &  -19.67 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453984.8431 &   42.79 & -102.59 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453991.8608 &  -20.21 &  -39.25 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24453992.7920 &  -96.78 &   31.83 \\
HTR205-004 & t06250g40p00v016 & t06250g40p00v016 & 24454045.7312 &   24.21 &  -92.46 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24453686.7129 & -105.66 &  105.06 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24453714.6922 &  -60.29 &   54.99 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24453721.6837 &  -99.87 &   89.99 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24453748.6266 &   45.52 &  -85.33 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24453925.9756 &  -54.81 &   31.11 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24453927.9627 & -106.47 &   87.95 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24453984.9185 &   54.74 &  -87.81 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24454012.8186 &    5.02 &  -22.65 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24454018.7145 &  -98.03 &   90.68 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24454046.7097 &  -40.72 &    3.88 \\
HTR205-010 & t05750g35p00v040 & t06000g40p00v030 & 24454049.5973 &   45.01 &  -75.69 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453187.9696 &   81.21 &  -95.52 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453684.7869 &   26.29 &  -36.76 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453689.7528 &    8.49 &  -22.12 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453690.7202 &   74.12 &  -86.15 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453714.7076 &  -24.41 &    6.10 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453722.6981 &  -19.05 &    6.45 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453747.5911 &   21.08 &  -32.73 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453984.8282 &    5.61 &  -14.05 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453990.8696 &  -37.96 &   25.42 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453991.9186 &   83.54 & -100.21 \\
HTR205-011 & t05500g35p00v020 & t05500g35p00v020 & 24453992.8562 &  -47.60 &   38.41 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453186.9557 &   39.50 & -116.96 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453188.9631 &  -45.96 &  -14.90 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453191.9633 &  -71.06 &   12.77 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453686.6673 &  -41.67 &  -18.42 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453690.7429 & -111.16 &   67.61 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453694.7150 &   -0.58 &  -73.33 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453714.7231 &   21.61 &  -89.96 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453988.7650 &   29.55 &  -96.79 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453990.9198 & -109.03 &   66.24 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24453991.9339 &   32.58 & -105.97 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24454012.7635 & -111.03 &   69.78 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24454015.7369 &  -99.09 &   58.04 \\
HTR205-012 & t06250g40p00v035 & t05500g40p00v025 & 24454019.7036 &  -69.33 &   14.72 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453187.9439 &  -61.62 &   68.28 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453275.8629 &   51.61 &  -66.59 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453663.7601 &  -35.51 &   26.96 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453684.7254 &   53.45 & -106.85 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453689.6827 &   46.14 &  -87.43 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453694.6791 &   36.99 &  -73.78 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453714.6449 &  -20.80 &   11.43 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453746.5692 &   53.38 &  -99.39 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453984.9005 &  -73.46 &   95.52 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453987.8450 &   25.34 &  -59.07 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453990.8243 &    6.36 &  -37.35 \\
HTR205-017 & t06750g40p00v010 & t05000g45p00v006 & 24453991.8888 &   57.51 & -105.11 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453187.9529 &  -30.05 &   13.61 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453684.7370 &  -73.29 &   92.12 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453685.5762 &  -66.61 &   79.04 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453689.6960 &    2.51 &  -40.54 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453714.6574 &   49.46 & -112.66 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453748.6055 &   -9.08 &  -19.38 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453902.9482 &   40.62 &  -99.67 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453987.8524 &   41.11 & -108.30 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453990.7679 &  -57.02 &   64.15 \\
HTR205-020 & t11500g50p00v012 & t06500g45p00v006 & 24453991.9036 &  -72.57 &   94.91 \\
\enddata
\tablecomments{
column (1): HATNet transiting-planet candidate designation, \\
column (3): template for primary, \\
column (3): template for secondary, \\
column (4): heliocentric Julian date, \\
column (5): primary heliocentric radial velocity (\kms), \\
column (6): secondary heliocentric radial velocity (\kms), \\}
\tablecomments{
This table is presented in its entirety in the electronic edition of the Astrophysical Journal.
A portion is shown here for guidance regarding its form and content.}
\end{deluxetable}


==> tab9.tex <==
\begin{deluxetable}{ccc}
\tablewidth{0pc}
\tablenum{9}\tablecaption{HATNet Photometry for HTR205-024}
\tablehead{
\colhead{BJD} &
\colhead{Mag} &
\colhead{Error}}
\startdata
2453939.70260 & 9.57255 & 0.00461 \\
2453939.70642 & 9.56319 & 0.00372 \\
2453939.71020 & 9.56735 & 0.00358 \\
2453939.71398 & 9.57243 & 0.00354 \\
2453939.71777 & 9.56314 & 0.00364 \\
2453939.72155 & 9.56694 & 0.00357 \\
2453939.72535 & 9.56329 & 0.00362 \\
2453939.72914 & 9.57796 & 0.00351 \\
2453939.73294 & 9.56721 & 0.00372 \\
2453939.73675 & 9.56942 & 0.00359 \\
2453939.74054 & 9.57218 & 0.00383 \\
2453939.74435 & 9.56721 & 0.00349 \\
2453939.74815 & 9.57110 & 0.00315 \\
2453939.75195 & 9.56914 & 0.00332 \\
2453939.75587 & 9.58305 & 0.00328 \\
2453939.75967 & 9.57258 & 0.00344 \\
2453939.76346 & 9.56742 & 0.00340 \\
2453939.76726 & 9.57114 & 0.00344 \\
2453939.77106 & 9.56687 & 0.00319 \\
2453939.77485 & 9.56297 & 0.00339 \\
2453939.77865 & 9.56469 & 0.00320 \\
2453939.78244 & 9.56737 & 0.00330 \\
2453939.78625 & 9.56924 & 0.00332 \\
2453939.79002 & 9.56261 & 0.00353 \\
2453939.79382 & 9.56215 & 0.00325 \\
2453939.79762 & 9.56305 & 0.00319 \\
2453939.80519 & 9.57396 & 0.00337 \\
2453939.80899 & 9.57361 & 0.00320 \\
2453939.81276 & 9.57058 & 0.00313 \\
2453939.81656 & 9.57808 & 0.00334 \\
2453939.82035 & 9.57397 & 0.00319 \\
2453939.82415 & 9.56878 & 0.00317 \\
2453939.82795 & 9.56795 & 0.00317 \\
2453939.83187 & 9.56399 & 0.00340 \\
2453939.83566 & 9.57495 & 0.00362 \\
2453939.83948 & 9.55837 & 0.00317 \\
2453939.84327 & 9.56849 & 0.00380 \\
2453939.84707 & 9.58142 & 0.00358 \\
2453939.85087 & 9.56003 & 0.00365 \\
2453939.85466 & 9.58472 & 0.00364 \\
2453939.85846 & 9.57212 & 0.00341 \\
2453939.86226 & 9.56096 & 0.00366 \\
2453939.86606 & 9.57071 & 0.00355 \\
2453939.86985 & 9.56607 & 0.00317 \\
2453939.87364 & 9.56703 & 0.00354 \\
2453939.87744 & 9.57488 & 0.00350 \\
2453939.88124 & 9.57623 & 0.00357 \\
2453939.88504 & 9.57561 & 0.00364 \\
2453939.88883 & 9.56804 & 0.00331 \\
2453939.89263 & 9.56492 & 0.00362 \\
2453939.89642 & 9.56598 & 0.00329 \\
2453939.90023 & 9.57984 & 0.00359 \\
2453939.90402 & 9.57068 & 0.00352 \\
2453939.90794 & 9.56832 & 0.00694 \\
2453939.91928 & 9.55764 & 0.00609 \\
2453939.92308 & 9.57878 & 0.00589 \\
2453939.92686 & 9.58837 & 0.00985 \\
2453939.93063 & 9.56107 & 0.00849 \\
2453939.95331 & 9.56625 & 0.00686 \\
2453939.95710 & 9.56733 & 0.00676 \\
2452910.71316 & 9.57302 & 0.00250 \\
2452910.71716 & 9.56905 & 0.00248 \\
2452910.72089 & 9.56972 & 0.00253 \\
2452910.72503 & 9.57369 & 0.00248 \\
2452910.72877 & 9.57537 & 0.00240 \\
2452910.76399 & 9.58334 & 0.00244 \\
2452910.76772 & 9.57099 & 0.00249 \\
2452910.77186 & 9.56833 & 0.00242 \\
2452910.77559 & 9.57645 & 0.00245 \\
2452910.77960 & 9.57242 & 0.00239 \\
2452910.79120 & 9.58166 & 0.00261 \\
2452910.79520 & 9.56933 & 0.00254 \\
2452910.79894 & 9.56646 & 0.00248 \\
2452910.80384 & 9.56339 & 0.00246 \\
2452910.80759 & 9.57559 & 0.00247 \\
2452910.81158 & 9.56362 & 0.00255 \\
2452910.81944 & 9.56213 & 0.00259 \\
2452910.82317 & 9.56439 & 0.00269 \\
2452910.82718 & 9.57040 & 0.00258 \\
2452910.83091 & 9.56672 & 0.00248 \\
2452910.83505 & 9.57137 & 0.00276 \\
2452910.83878 & 9.56135 & 0.00252 \\
2452910.84278 & 9.56730 & 0.00271 \\
2452910.84651 & 9.57014 & 0.00265 \\
2452910.85064 & 9.56559 & 0.00258 \\
2452910.85438 & 9.57081 & 0.00282 \\
2452910.85838 & 9.57193 & 0.00274 \\
2452910.86211 & 9.56772 & 0.00262 \\
2452910.86624 & 9.56111 & 0.00265 \\
2452910.86997 & 9.57517 & 0.00276 \\
2452910.87397 & 9.57742 & 0.00250 \\
2452910.87770 & 9.56866 & 0.00249 \\
2452910.88183 & 9.57076 & 0.00263 \\
2452910.88556 & 9.56849 & 0.00272 \\
2452910.88955 & 9.56361 & 0.00267 \\
2452910.89329 & 9.57052 & 0.00250 \\
2452910.89852 & 9.57163 & 0.00261 \\
2452910.90225 & 9.56443 & 0.00252 \\
2452910.90628 & 9.55317 & 0.00257 \\
2452910.90999 & 9.57343 & 0.00266 \\
2452910.91415 & 9.56612 & 0.00266 \\
2452910.91788 & 9.57415 & 0.00254 \\
2452910.92187 & 9.57965 & 0.00255 \\
2452910.92560 & 9.57108 & 0.00254 \\
2452910.92974 & 9.56471 & 0.00269 \\
2452910.93347 & 9.56470 & 0.00271 \\
2452910.93749 & 9.57616 & 0.00251 \\
2452910.94122 & 9.57388 & 0.00252 \\
2452910.94535 & 9.57434 & 0.00265 \\
2452910.94909 & 9.56119 & 0.00254 \\
2452910.95309 & 9.56680 & 0.00269 \\
2452910.95683 & 9.57744 & 0.00248 \\
2452910.96097 & 9.56287 & 0.00266 \\
2452910.96470 & 9.57218 & 0.00262 \\
2452911.65283 & 9.55896 & 0.00246 \\
2452911.66537 & 9.56351 & 0.00265 \\
2452911.66911 & 9.56068 & 0.00246 \\
2452911.67284 & 9.57538 & 0.00262 \\
2452911.67669 & 9.56808 & 0.00245 \\
2452911.68064 & 9.56105 & 0.00248 \\
2452911.68446 & 9.56591 & 0.00252 \\
2452911.68829 & 9.57474 & 0.00251 \\
2452911.69605 & 9.57105 & 0.00260 \\
2452911.69989 & 9.56965 & 0.00251 \\
2452911.70375 & 9.57863 & 0.00251 \\
2452911.70757 & 9.56895 & 0.00238 \\
2452911.71153 & 9.56618 & 0.00244 \\
2452911.71921 & 9.57504 & 0.00243 \\
2452911.72303 & 9.56527 & 0.00260 \\
2452911.72699 & 9.57324 & 0.00247 \\
2452911.73081 & 9.56971 & 0.00257 \\
2452911.73463 & 9.57215 & 0.00246 \\
2452911.73846 & 9.57496 & 0.00253 \\
2452911.74242 & 9.58165 & 0.00251 \\
2452911.74626 & 9.57016 & 0.00237 \\
2452911.75011 & 9.57285 & 0.00264 \\
2452911.75396 & 9.57316 & 0.00255 \\
2452911.75852 & 9.58014 & 0.00274 \\
2452911.76235 & 9.56898 & 0.00258 \\
2452911.76621 & 9.57558 & 0.00263 \\
2452911.77003 & 9.57325 & 0.00252 \\
2452911.77401 & 9.58153 & 0.00256 \\
2452911.77787 & 9.57802 & 0.00261 \\
2452911.78165 & 9.58329 & 0.00254 \\
2452911.78548 & 9.58585 & 0.00247 \\
2452911.78944 & 9.57494 & 0.00264 \\
2452911.79326 & 9.57868 & 0.00245 \\
2452911.79709 & 9.57616 & 0.00241 \\
2452911.80092 & 9.57495 & 0.00247 \\
2452911.80487 & 9.57575 & 0.00257 \\
2452911.80869 & 9.57403 & 0.00248 \\
2452911.81251 & 9.57744 & 0.00259 \\
2452911.81634 & 9.57478 & 0.00250 \\
2452911.82029 & 9.57766 & 0.00272 \\
2452911.82411 & 9.57064 & 0.00246 \\
2452911.83572 & 9.57822 & 0.00239 \\
2452911.83953 & 9.58166 & 0.00249 \\
2452911.84335 & 9.57766 & 0.00255 \\
2452911.84717 & 9.56548 & 0.00264 \\
2452911.85205 & 9.56493 & 0.00244 \\
2452911.85588 & 9.57496 & 0.00248 \\
2452911.85975 & 9.58107 & 0.00255 \\
2452911.86357 & 9.58063 & 0.00262 \\
2452911.86752 & 9.57116 & 0.00247 \\
2452911.87134 & 9.57733 & 0.00255 \\
2452911.87516 & 9.58063 & 0.00260 \\
2452911.88677 & 9.56731 & 0.00251 \\
2452911.89058 & 9.56852 & 0.00253 \\
2452911.89441 & 9.57122 & 0.00271 \\
2452911.89837 & 9.57050 & 0.00262 \\
2452912.59425 & 9.55949 & 0.00300 \\
2452912.59806 & 9.56431 & 0.00261 \\
2452912.60188 & 9.57225 & 0.00268 \\
2452912.60583 & 9.58451 & 0.00263 \\
2452912.60964 & 9.57228 & 0.00284 \\
2452912.61346 & 9.57713 & 0.00272 \\
2452912.61727 & 9.56959 & 0.00244 \\
2452912.62123 & 9.56360 & 0.00270 \\
2452912.62506 & 9.57436 & 0.00253 \\
2452912.62888 & 9.56959 & 0.00258 \\
2452912.63269 & 9.56592 & 0.00243 \\
2452912.63666 & 9.57530 & 0.00263 \\
2452912.64047 & 9.56704 & 0.00251 \\
2452912.64431 & 9.57377 & 0.00244 \\
2452912.64814 & 9.57101 & 0.00261 \\
2452912.65209 & 9.56437 & 0.00255 \\
2452912.65591 & 9.57103 & 0.00256 \\
2452912.65973 & 9.56286 & 0.00241 \\
2452912.66355 & 9.58149 & 0.00258 \\
2452912.66750 & 9.58085 & 0.00265 \\
2452912.67132 & 9.57650 & 0.00241 \\
2452912.67890 & 9.57627 & 0.00248 \\
2452912.68426 & 9.57738 & 0.00257 \\
2452912.68810 & 9.57471 & 0.00261 \\
2452912.69192 & 9.57295 & 0.00254 \\
2452912.69578 & 9.57683 & 0.00236 \\
2452912.69973 & 9.58033 & 0.00238 \\
2452912.70358 & 9.56757 & 0.00252 \\
2452912.70740 & 9.57397 & 0.00257 \\
2452912.71123 & 9.57319 & 0.00238 \\
2452912.71519 & 9.56473 & 0.00264 \\
2452912.71903 & 9.57447 & 0.00260 \\
2452912.72289 & 9.56755 & 0.00245 \\
2452912.72672 & 9.56935 & 0.00248 \\
2452912.73068 & 9.57073 & 0.00240 \\
2452912.73450 & 9.56332 & 0.00241 \\
2452912.73834 & 9.58096 & 0.00247 \\
2452912.74607 & 9.57644 & 0.00234 \\
2452912.74990 & 9.57384 & 0.00247 \\
2452912.75371 & 9.57261 & 0.00235 \\
2452912.76146 & 9.56686 & 0.00245 \\
2452912.76527 & 9.56342 & 0.00249 \\
2452912.76912 & 9.56388 & 0.00237 \\
2452912.77295 & 9.56495 & 0.00245 \\
2452912.78517 & 9.57552 & 0.00288 \\
2452912.78900 & 9.57333 & 0.00231 \\
2452912.79296 & 9.56377 & 0.00255 \\
2452912.79679 & 9.56516 & 0.00247 \\
2452912.80062 & 9.56898 & 0.00243 \\
2452912.80444 & 9.56346 & 0.00235 \\
2452912.80839 & 9.57145 & 0.00252 \\
2452912.81223 & 9.57393 & 0.00277 \\
2452912.81607 & 9.57615 & 0.00237 \\
2452912.81990 & 9.56664 & 0.00245 \\
2452912.83151 & 9.56483 & 0.00250 \\
2452912.83534 & 9.56760 & 0.00238 \\
2452912.83929 & 9.56669 & 0.00247 \\
2452912.84313 & 9.57047 & 0.00252 \\
2452912.84695 & 9.57578 & 0.00242 \\
2452912.85858 & 9.56589 & 0.00252 \\
2452912.86241 & 9.56895 & 0.00256 \\
2452912.86623 & 9.57314 & 0.00250 \\
2452912.87128 & 9.57475 & 0.00264 \\
2452912.88675 & 9.56896 & 0.00247 \\
2452912.89057 & 9.56654 & 0.00243 \\
2452912.89440 & 9.55515 & 0.00244 \\
2452912.89823 & 9.57096 & 0.00238 \\
2452913.59781 & 9.54631 & 0.00258 \\
2452913.60163 & 9.58138 & 0.00292 \\
2452913.60544 & 9.56810 & 0.00265 \\
2452913.60938 & 9.56503 & 0.00259 \\
2452913.61321 & 9.56143 & 0.00251 \\
2452913.61703 & 9.56074 & 0.00264 \\
2452913.62085 & 9.57291 & 0.00276 \\
2452913.62480 & 9.57706 & 0.00264 \\
2452913.62862 & 9.56104 & 0.00265 \\
2452913.63245 & 9.56217 & 0.00250 \\
2452913.63628 & 9.56333 & 0.00267 \\
2452913.64028 & 9.57443 & 0.00264 \\
2452913.64411 & 9.55768 & 0.00265 \\
2452913.64794 & 9.57846 & 0.00250 \\
2452913.65177 & 9.56652 & 0.00258 \\
2452913.65572 & 9.57265 & 0.00282 \\
2452913.65959 & 9.56326 & 0.00246 \\
2452913.66337 & 9.56087 & 0.00255 \\
2452913.66723 & 9.56519 & 0.00267 \\
2452913.67121 & 9.57659 & 0.00265 \\
2452913.67505 & 9.57140 & 0.00261 \\
2452913.67888 & 9.56356 & 0.00261 \\
2452913.68271 & 9.56971 & 0.00256 \\
2452913.68810 & 9.57583 & 0.00284 \\
2452913.69193 & 9.56558 & 0.00250 \\
2452913.69579 & 9.57209 & 0.00255 \\
2452913.69961 & 9.57445 & 0.00260 \\
2452913.70356 & 9.58379 & 0.00259 \\
2452913.70739 & 9.56007 & 0.00274 \\
2452913.71123 & 9.56559 & 0.00300 \\
2452913.71895 & 9.57089 & 0.00254 \\
2452913.72281 & 9.57396 & 0.00247 \\
2452913.72663 & 9.57213 & 0.00262 \\
2452913.73052 & 9.56033 & 0.00301 \\
2452913.73448 & 9.56330 & 0.00263 \\
2452913.73830 & 9.56840 & 0.00241 \\
2452913.74212 & 9.57465 & 0.00245 \\
2452913.74598 & 9.57924 & 0.00283 \\
2452913.74994 & 9.57403 & 0.00247 \\
2452913.75378 & 9.56825 & 0.00261 \\
2452913.75762 & 9.57197 & 0.00261 \\
2452913.76144 & 9.57452 & 0.00240 \\
2452913.76541 & 9.56585 & 0.00262 \\
2452913.76925 & 9.57142 & 0.00243 \\
2452913.77314 & 9.57682 & 0.00250 \\
2452913.77698 & 9.57131 & 0.00236 \\
2452913.78544 & 9.57321 & 0.00248 \\
2452913.78927 & 9.56211 & 0.00242 \\
2452913.79311 & 9.56748 & 0.00254 \\
2452913.79706 & 9.56629 & 0.00249 \\
2452913.80090 & 9.56688 & 0.00249 \\
2452913.80473 & 9.56188 & 0.00251 \\
2452913.80856 & 9.57338 & 0.00257 \\
2452913.81247 & 9.57273 & 0.00249 \\
2452913.81630 & 9.57009 & 0.00245 \\
2452913.82011 & 9.56680 & 0.00250 \\
2452913.82789 & 9.56512 & 0.00246 \\
2452913.83175 & 9.56974 & 0.00247 \\
2452913.83938 & 9.57308 & 0.00244 \\
2452913.85483 & 9.56758 & 0.00270 \\
2452913.85879 & 9.56479 & 0.00250 \\
2452913.86262 & 9.57022 & 0.00259 \\
2452913.86646 & 9.56969 & 0.00248 \\
2452913.87029 & 9.57437 & 0.00249 \\
2452913.87529 & 9.56984 & 0.00248 \\
2452913.87907 & 9.57090 & 0.00258 \\
2452913.88291 & 9.56986 & 0.00253 \\
2452913.88676 & 9.56407 & 0.00253 \\
2452913.89072 & 9.56194 & 0.00260 \\
2452913.89457 & 9.57759 & 0.00247 \\
2452916.59468 & 9.56734 & 0.00286 \\
2452916.59851 & 9.57004 & 0.00263 \\
2452916.60233 & 9.57359 & 0.00264 \\
2452916.60629 & 9.57826 & 0.00248 \\
2452916.61011 & 9.57294 & 0.00277 \\
2452916.61395 & 9.56877 & 0.00257 \\
2452916.61780 & 9.57314 & 0.00272 \\
2452916.62175 & 9.57256 & 0.00257 \\
2452916.62557 & 9.57231 & 0.00273 \\
2452916.62940 & 9.57092 & 0.00278 \\
2452916.63336 & 9.57350 & 0.00262 \\
2452916.63731 & 9.56453 & 0.00283 \\
2452916.64518 & 9.56696 & 0.00249 \\
2452916.64916 & 9.56114 & 0.00262 \\
2452916.65335 & 9.56974 & 0.00260 \\
2452916.65739 & 9.56584 & 0.00276 \\
2452916.66143 & 9.56777 & 0.00298 \\
2452916.66540 & 9.57389 & 0.00310 \\
2452916.66957 & 9.56976 & 0.00347 \\
2452916.67355 & 9.56531 & 0.00311 \\
2452916.67755 & 9.56435 & 0.00267 \\
2452916.68156 & 9.56504 & 0.00271 \\
2452916.68573 & 9.55716 & 0.00271 \\
2452916.69363 & 9.57105 & 0.00287 \\
2452916.69765 & 9.55732 & 0.00397 \\
2452916.70179 & 9.57538 & 0.00316 \\
2452916.70576 & 9.57692 & 0.00296 \\
2452916.70958 & 9.56168 & 0.00390 \\
2452916.71747 & 9.57723 & 0.00427 \\
2452916.81023 & 9.56747 & 0.00341 \\
2452916.81405 & 9.56950 & 0.00687 \\
2452916.82564 & 9.58344 & 0.00301 \\
2452916.82946 & 9.57103 & 0.00282 \\
2452916.83328 & 9.56333 & 0.00265 \\
2452916.83710 & 9.57217 & 0.00311 \\
2452916.84105 & 9.56764 & 0.00257 \\
2452916.85648 & 9.56614 & 0.00260 \\
2452916.86034 & 9.56542 & 0.00258 \\
2452916.86416 & 9.57538 & 0.00258 \\
2452916.88345 & 9.57038 & 0.00264 \\
2452916.88742 & 9.55548 & 0.00268 \\
2452916.89126 & 9.58097 & 0.00258 \\
2452917.70178 & 9.57048 & 0.00266 \\
2452917.70588 & 9.56989 & 0.00274 \\
2452917.70970 & 9.57050 & 0.00252 \\
2452917.71393 & 9.57776 & 0.00305 \\
2452917.71773 & 9.56812 & 0.00262 \\
2452917.72183 & 9.57755 & 0.00252 \\
2452917.72564 & 9.57658 & 0.00275 \\
2452917.72986 & 9.57360 & 0.00269 \\
2452917.73370 & 9.56985 & 0.00286 \\
2452917.73782 & 9.56412 & 0.00266 \\
2452917.74165 & 9.57299 & 0.00261 \\
2452917.74587 & 9.57233 & 0.00257 \\
2452917.74970 & 9.57212 & 0.00267 \\
2452917.75379 & 9.56985 & 0.00270 \\
2452917.75761 & 9.57091 & 0.00287 \\
2452917.76185 & 9.56903 & 0.00259 \\
2452917.76573 & 9.56493 & 0.00267 \\
2452917.76986 & 9.56558 & 0.00260 \\
2452917.77370 & 9.56906 & 0.00270 \\
2452917.77792 & 9.57284 & 0.00268 \\
2452917.78176 & 9.57959 & 0.00253 \\
2452917.78586 & 9.56688 & 0.00268 \\
2452917.78971 & 9.57623 & 0.00269 \\
2452917.79393 & 9.57850 & 0.00252 \\
2452917.79775 & 9.56692 & 0.00269 \\
2452917.80184 & 9.56859 & 0.00269 \\
2452917.80567 & 9.57379 & 0.00274 \\
2452917.80983 & 9.57276 & 0.00277 \\
2452917.81365 & 9.57775 & 0.00275 \\
2452917.82569 & 9.56760 & 0.00267 \\
2452917.82952 & 9.57018 & 0.00275 \\
2452917.83360 & 9.57372 & 0.00258 \\
2452917.83742 & 9.56531 & 0.00280 \\
2452917.84166 & 9.58043 & 0.00260 \\
2452917.85339 & 9.56936 & 0.00275 \\
2452917.85761 & 9.56472 & 0.00247 \\
2452917.86142 & 9.56142 & 0.00287 \\
2452917.86552 & 9.56718 & 0.00264 \\
2452917.88148 & 9.56907 & 0.00260 \\
2452917.88530 & 9.57676 & 0.00282 \\
2452917.88954 & 9.57369 & 0.00273 \\
2452918.58907 & 9.58220 & 0.00291 \\
2452918.59315 & 9.57223 & 0.00272 \\
2452918.59721 & 9.56685 & 0.00279 \\
2452918.60129 & 9.57008 & 0.00269 \\
2452918.60556 & 9.57485 & 0.00273 \\
2452918.60964 & 9.57263 & 0.00278 \\
2452918.61765 & 9.57293 & 0.00309 \\
2452918.62193 & 9.56954 & 0.00278 \\
2452918.62599 & 9.57114 & 0.00277 \\
2452918.63008 & 9.56817 & 0.00271 \\
2452918.63416 & 9.57122 & 0.00274 \\
2452918.63845 & 9.57290 & 0.00287 \\
2452918.64253 & 9.56949 & 0.00256 \\
2452918.64661 & 9.57433 & 0.00272 \\
2452918.65069 & 9.57356 & 0.00283 \\
2452918.65496 & 9.57831 & 0.00469 \\
2452918.66301 & 9.57914 & 0.00366 \\
2452918.66707 & 9.57268 & 0.00300 \\
2452918.67126 & 9.57301 & 0.00273 \\
2452918.67535 & 9.57709 & 0.00271 \\
2452918.67942 & 9.56757 & 0.00275 \\
2452918.68350 & 9.56450 & 0.00262 \\
2452918.68778 & 9.56354 & 0.00297 \\
2452918.69185 & 9.57150 & 0.00269 \\
2452918.69586 & 9.57141 & 0.00299 \\
2452918.69991 & 9.56801 & 0.00337 \\
2452918.70418 & 9.57291 & 0.00297 \\
2452918.70828 & 9.57293 & 0.00292 \\
2452918.71239 & 9.56857 & 0.00268 \\
2452918.71636 & 9.57673 & 0.00295 \\
2452918.72053 & 9.57851 & 0.00268 \\
2452918.72840 & 9.56515 & 0.00275 \\
2452918.73238 & 9.57048 & 0.00263 \\
2452918.73645 & 9.56593 & 0.00267 \\
2452918.74048 & 9.55904 & 0.00276 \\
2452918.74446 & 9.56144 & 0.00266 \\
2452918.74849 & 9.56970 & 0.00284 \\
2452918.75265 & 9.57049 & 0.00264 \\
2452918.75659 & 9.56424 & 0.00268 \\
2452918.76057 & 9.56660 & 0.00290 \\
2452918.76462 & 9.56901 & 0.00277 \\
2452918.76873 & 9.57056 & 0.00280 \\
2452918.77279 & 9.57020 & 0.00271 \\
2452918.77683 & 9.57338 & 0.00297 \\
2452918.78083 & 9.57045 & 0.00266 \\
2452918.78500 & 9.57522 & 0.00299 \\
2452918.78900 & 9.57396 & 0.00263 \\
2452918.79298 & 9.57066 & 0.00289 \\
2452918.79695 & 9.57105 & 0.00287 \\
2452918.80111 & 9.57311 & 0.00276 \\
2452918.80507 & 9.57732 & 0.00272 \\
2452918.80906 & 9.57835 & 0.00267 \\
2452918.81305 & 9.57161 & 0.00266 \\
2452918.81721 & 9.57884 & 0.00266 \\
2452918.82124 & 9.57032 & 0.00263 \\
2452918.82522 & 9.56085 & 0.00287 \\
2452918.82920 & 9.57355 & 0.00301 \\
2452918.83330 & 9.57441 & 0.00269 \\
2452918.83728 & 9.57427 & 0.00283 \\
2452918.84124 & 9.56285 & 0.00270 \\
2452918.84943 & 9.57194 & 0.00295 \\
2452918.85340 & 9.57077 & 0.00275 \\
2452918.85743 & 9.57003 & 0.00280 \\
2452918.86140 & 9.58153 & 0.00263 \\
2452918.86557 & 9.56719 & 0.00290 \\
2452918.86954 & 9.58100 & 0.00268 \\
2452918.87358 & 9.56664 & 0.00275 \\
2452918.87761 & 9.57713 & 0.00265 \\
2452918.88171 & 9.56797 & 0.00257 \\
2452918.88567 & 9.56583 & 0.00283 \\
2452918.88964 & 9.56428 & 0.00278 \\
2452925.65161 & 9.56958 & 0.00265 \\
2452925.65559 & 9.56486 & 0.00271 \\
2452925.65965 & 9.57154 & 0.00282 \\
2452925.66382 & 9.56691 & 0.00260 \\
2452925.66786 & 9.56495 & 0.00280 \\
2452925.67187 & 9.56711 & 0.00304 \\
2452925.67590 & 9.57673 & 0.00279 \\
2452925.68006 & 9.56763 & 0.00275 \\
2452925.68800 & 9.57036 & 0.00270 \\
2452925.69203 & 9.56575 & 0.00294 \\
2452925.69614 & 9.56733 & 0.00298 \\
2452925.70017 & 9.56748 & 0.00277 \\
2452925.70416 & 9.56607 & 0.00287 \\
2452925.70819 & 9.56991 & 0.00289 \\
2452925.71230 & 9.56680 & 0.00272 \\
2452925.71627 & 9.57257 & 0.00291 \\
2452925.72026 & 9.57480 & 0.00299 \\
2452925.72425 & 9.57432 & 0.00266 \\
2452925.72835 & 9.57734 & 0.00292 \\
2452925.73233 & 9.56784 & 0.00269 \\
2452925.73634 & 9.56984 & 0.00297 \\
2452925.74032 & 9.57509 & 0.00257 \\
2452925.74445 & 9.57161 & 0.00247 \\
2452925.75236 & 9.56848 & 0.00277 \\
2452925.75636 & 9.56788 & 0.00266 \\
2452925.76054 & 9.56992 & 0.00277 \\
2452925.76447 & 9.56151 & 0.00259 \\
2452925.76844 & 9.57735 & 0.00261 \\
2452925.77242 & 9.57040 & 0.00272 \\
2452925.77653 & 9.56751 & 0.00289 \\
2452925.78057 & 9.56970 & 0.00287 \\
2452925.78462 & 9.56835 & 0.00270 \\
2452925.78865 & 9.56287 & 0.00265 \\
2452925.79277 & 9.56574 & 0.00269 \\
2452925.80085 & 9.58176 & 0.00280 \\
2452925.80489 & 9.56406 & 0.00293 \\
2452925.80900 & 9.56911 & 0.00298 \\
2452925.81298 & 9.56999 & 0.00281 \\
2452925.81701 & 9.56999 & 0.00295 \\
2452925.82101 & 9.57998 & 0.00290 \\
2452925.83320 & 9.56420 & 0.00282 \\
2452925.83726 & 9.57414 & 0.00284 \\
2452925.84139 & 9.56911 & 0.00258 \\
2452925.84538 & 9.57629 & 0.00294 \\
2452925.85742 & 9.57660 & 0.00304 \\
2452925.86143 & 9.57591 & 0.00311 \\
2452925.86546 & 9.57626 & 0.00280 \\
2452925.86951 & 9.58361 & 0.00292 \\
2452926.65125 & 9.56500 & 0.00254 \\
2452926.65532 & 9.56600 & 0.00257 \\
2452926.65930 & 9.56832 & 0.00284 \\
2452926.66350 & 9.57007 & 0.00309 \\
2452926.66748 & 9.56940 & 0.00269 \\
2452926.67146 & 9.57834 & 0.00259 \\
2452926.67544 & 9.56589 & 0.00259 \\
2452926.67956 & 9.57232 & 0.00272 \\
2452926.68353 & 9.56850 & 0.00268 \\
2452926.68755 & 9.57016 & 0.00254 \\
2452926.69159 & 9.57640 & 0.00320 \\
2452926.69576 & 9.56713 & 0.00261 \\
2452926.69972 & 9.57390 & 0.00262 \\
2452926.70377 & 9.56453 & 0.00271 \\
2452926.70782 & 9.57190 & 0.00273 \\
2452926.71194 & 9.56841 & 0.00288 \\
2452926.71591 & 9.56991 & 0.00247 \\
2452926.71998 & 9.56895 & 0.00266 \\
2452926.72403 & 9.56817 & 0.00288 \\
2452926.72819 & 9.56508 & 0.00270 \\
2452926.73219 & 9.56591 & 0.00274 \\
2452926.73613 & 9.56940 & 0.00250 \\
2452926.74007 & 9.56430 & 0.00235 \\
2452926.74423 & 9.56770 & 0.00257 \\
2452926.74820 & 9.57072 & 0.00274 \\
2452926.75214 & 9.56954 & 0.00268 \\
2452926.75621 & 9.57051 & 0.00270 \\
2452926.76030 & 9.56722 & 0.00272 \\
2452926.76436 & 9.56934 & 0.00259 \\
2452926.76839 & 9.57100 & 0.00281 \\
2452926.77235 & 9.57223 & 0.00271 \\
2452926.77652 & 9.56116 & 0.00272 \\
2452926.78052 & 9.56888 & 0.00267 \\
2452926.78448 & 9.56934 & 0.00281 \\
2452926.78848 & 9.56624 & 0.00274 \\
2452926.80057 & 9.57509 & 0.00256 \\
2452926.80455 & 9.56276 & 0.00290 \\
2452926.80866 & 9.57092 & 0.00300 \\
2452926.81268 & 9.57849 & 0.00271 \\
2452926.81665 & 9.57725 & 0.00270 \\
2452926.82891 & 9.57545 & 0.00276 \\
2452926.83291 & 9.57043 & 0.00275 \\
2452926.83697 & 9.56573 & 0.00264 \\
2452926.84109 & 9.56413 & 0.00268 \\
2452926.84506 & 9.57289 & 0.00284 \\
2452926.85314 & 9.57453 & 0.00275 \\
2452926.85730 & 9.57394 & 0.00278 \\
2452926.86133 & 9.57550 & 0.00313 \\
2452926.86535 & 9.57327 & 0.00320 \\
2452927.64601 & 9.56642 & 0.00248 \\
2452927.65003 & 9.57276 & 0.00268 \\
2452927.65402 & 9.57452 & 0.00254 \\
2452927.66213 & 9.56747 & 0.00262 \\
2452927.66612 & 9.56613 & 0.00252 \\
2452927.67011 & 9.57104 & 0.00283 \\
2452927.67410 & 9.57829 & 0.00279 \\
2452927.67822 & 9.56919 & 0.00285 \\
2452927.68221 & 9.57139 & 0.00292 \\
2452927.68619 & 9.57385 & 0.00259 \\
2452927.69024 & 9.57173 & 0.00258 \\
2452927.69842 & 9.57391 & 0.00280 \\
2452927.70241 & 9.57074 & 0.00270 \\
2452927.70647 & 9.57037 & 0.00271 \\
2452927.71058 & 9.57074 & 0.00266 \\
2452927.71457 & 9.56915 & 0.00266 \\
2452927.71856 & 9.57396 & 0.00286 \\
2452927.72260 & 9.56571 & 0.00272 \\
2452927.72672 & 9.56996 & 0.00275 \\
2452927.73071 & 9.56993 & 0.00259 \\
2452927.73863 & 9.57224 & 0.00270 \\
2452927.74279 & 9.57787 & 0.00277 \\
2452927.74683 & 9.57457 & 0.00264 \\
2452927.75086 & 9.56188 & 0.00276 \\
2452927.75486 & 9.57353 & 0.00264 \\
2452927.75903 & 9.56757 & 0.00261 \\
2452927.76306 & 9.56666 & 0.00283 \\
2452927.76712 & 9.56405 & 0.00266 \\
2452927.77111 & 9.57586 & 0.00255 \\
2452927.77527 & 9.56499 & 0.00289 \\
2452927.77926 & 9.56871 & 0.00298 \\
2452927.78324 & 9.56984 & 0.00266 \\
2452927.78724 & 9.56428 & 0.00273 \\
2452927.79136 & 9.56385 & 0.00273 \\
2452927.79534 & 9.56843 & 0.00289 \\
2452927.79937 & 9.57275 & 0.00272 \\
2452927.80343 & 9.57114 & 0.00298 \\
2452927.80753 & 9.56885 & 0.00268 \\
2452927.81153 & 9.57247 & 0.00289 \\
2452927.81553 & 9.56480 & 0.00272 \\
2452927.82761 & 9.56879 & 0.00281 \\
2452927.83165 & 9.57036 & 0.00303 \\
2452927.83563 & 9.58312 & 0.00304 \\
2452927.83974 & 9.57032 & 0.00250 \\
2452927.85592 & 9.57353 & 0.00301 \\
2452927.85989 & 9.56891 & 0.00279 \\
2452927.86388 & 9.56538 & 0.00311 \\
2452928.64543 & 9.57613 & 0.00280 \\
2452928.64941 & 9.56984 & 0.00282 \\
2452928.65344 & 9.57352 & 0.00253 \\
2452928.65741 & 9.57063 & 0.00260 \\
2452928.66157 & 9.56676 & 0.00292 \\
2452928.66555 & 9.57422 & 0.00277 \\
2452928.66958 & 9.57223 & 0.00305 \\
2452928.67357 & 9.56541 & 0.00257 \\
2452928.67770 & 9.56363 & 0.00251 \\
2452928.68169 & 9.56842 & 0.00265 \\
2452928.68572 & 9.57465 & 0.00318 \\
2452928.68976 & 9.57192 & 0.00296 \\
2452928.69385 & 9.56549 & 0.00277 \\
2452928.69783 & 9.56613 & 0.00270 \\
2452928.70575 & 9.57561 & 0.00287 \\
2452928.70987 & 9.56724 & 0.00267 \\
2452928.71385 & 9.57020 & 0.00257 \\
2452928.71785 & 9.57000 & 0.00266 \\
2452928.72183 & 9.56774 & 0.00266 \\
2452928.72599 & 9.56991 & 0.00297 \\
2452928.73000 & 9.56681 & 0.00263 \\
2452928.73403 & 9.56594 & 0.00272 \\
2452928.73806 & 9.57533 & 0.00253 \\
2452928.74224 & 9.57255 & 0.00306 \\
2452928.74620 & 9.57163 & 0.00276 \\
2452928.75024 & 9.57023 & 0.00262 \\
2452928.75419 & 9.57582 & 0.00307 \\
2452928.75828 & 9.56373 & 0.00284 \\
2452928.76229 & 9.56745 & 0.00281 \\
2452928.76629 & 9.57612 & 0.00315 \\
2452928.77032 & 9.56876 & 0.00300 \\
2452928.77443 & 9.56606 & 0.00295 \\
2452928.77846 & 9.56665 & 0.00291 \\
2452928.78245 & 9.57158 & 0.00295 \\
2452928.78643 & 9.56197 & 0.00293 \\
2452928.79054 & 9.56522 & 0.00265 \\
2452928.79459 & 9.57494 & 0.00275 \\
2452928.79856 & 9.57289 & 0.00274 \\
2452928.80254 & 9.56789 & 0.00274 \\
2452928.80664 & 9.57819 & 0.00282 \\
2452928.81065 & 9.57182 & 0.00275 \\
2452928.81467 & 9.57500 & 0.00278 \\
2452928.81873 & 9.56665 & 0.00291 \\
2452928.82687 & 9.57072 & 0.00277 \\
2452928.83090 & 9.57393 & 0.00283 \\
2452928.83493 & 9.57837 & 0.00286 \\
2452928.83905 & 9.57540 & 0.00280 \\
2452928.85122 & 9.56065 & 0.00266 \\
2452928.85539 & 9.56339 & 0.00276 \\
2452928.85942 & 9.56832 & 0.00289 \\
2452929.64066 & 9.57285 & 0.00256 \\
2452929.64476 & 9.57138 & 0.00252 \\
2452929.64874 & 9.56604 & 0.00257 \\
2452929.65274 & 9.57253 & 0.00242 \\
2452929.65673 & 9.57286 & 0.00261 \\
2452929.66084 & 9.57110 & 0.00278 \\
2452929.66483 & 9.56796 & 0.00255 \\
2452929.66881 & 9.56445 & 0.00270 \\
2452929.67279 & 9.57379 & 0.00269 \\
2452929.67690 & 9.57036 & 0.00250 \\
2452929.68089 & 9.56443 & 0.00261 \\
2452929.68493 & 9.57085 & 0.00262 \\
2452929.68892 & 9.57404 & 0.00279 \\
2452929.69307 & 9.56614 & 0.00251 \\
2452929.69705 & 9.56274 & 0.00256 \\
2452929.70104 & 9.57079 & 0.00258 \\
2452929.70503 & 9.57018 & 0.00289 \\
2452929.70919 & 9.57376 & 0.00274 \\
2452929.71318 & 9.56736 & 0.00261 \\
2452929.71721 & 9.57008 & 0.00267 \\
2452929.72119 & 9.57104 & 0.00295 \\
2452929.72931 & 9.56885 & 0.00263 \\
2452929.73335 & 9.57353 & 0.00281 \\
2452929.73734 & 9.57561 & 0.00278 \\
2452929.74148 & 9.57118 & 0.00269 \\
2452929.74552 & 9.57231 & 0.00270 \\
2452929.74951 & 9.56144 & 0.00260 \\
2452929.75347 & 9.57199 & 0.00271 \\
2452929.75761 & 9.56655 & 0.00283 \\
2452929.76161 & 9.57425 & 0.00263 \\
2452929.76561 & 9.57686 & 0.00269 \\
2452929.76958 & 9.57210 & 0.00287 \\
2452929.77371 & 9.57365 & 0.00292 \\
2452929.77769 & 9.57280 & 0.00257 \\
2452929.78167 & 9.56969 & 0.00276 \\
2452929.78565 & 9.57018 & 0.00265 \\
2452929.78982 & 9.57151 & 0.00272 \\
2452929.79380 & 9.56716 & 0.00278 \\
2452929.79784 & 9.57651 & 0.00301 \\
2452929.80182 & 9.56423 & 0.00292 \\
2452929.80599 & 9.56746 & 0.00271 \\
2452929.80997 & 9.57564 & 0.00274 \\
2452929.82210 & 9.57526 & 0.00307 \\
2452929.82613 & 9.56997 & 0.00272 \\
2452929.83018 & 9.56939 & 0.00285 \\
2452929.83416 & 9.57671 & 0.00282 \\
2452929.84641 & 9.56636 & 0.00276 \\
2452929.85039 & 9.57233 & 0.00289 \\
2452929.85449 & 9.57864 & 0.00330 \\
2452929.85848 & 9.56317 & 0.00259 \\
2452930.65865 & 9.56333 & 0.00275 \\
2452930.66264 & 9.56201 & 0.00262 \\
2452930.66664 & 9.56551 & 0.00259 \\
2452930.67076 & 9.57536 & 0.00244 \\
2452930.67474 & 9.56833 & 0.00267 \\
2452930.67874 & 9.56578 & 0.00248 \\
2452930.68273 & 9.56848 & 0.00267 \\
2452930.68691 & 9.56719 & 0.00263 \\
2452930.69097 & 9.57880 & 0.00267 \\
2452930.69495 & 9.57151 & 0.00245 \\
2452930.69893 & 9.56683 & 0.00256 \\
2452930.70311 & 9.57798 & 0.00257 \\
2452930.70714 & 9.56422 & 0.00274 \\
2452930.71503 & 9.56668 & 0.00254 \\
2452930.71913 & 9.57297 & 0.00255 \\
2452930.72317 & 9.57175 & 0.00260 \\
2452930.72715 & 9.57059 & 0.00265 \\
2452930.73119 & 9.57207 & 0.00262 \\
2452930.73530 & 9.57675 & 0.00263 \\
2452930.73928 & 9.56677 & 0.00260 \\
2452930.74327 & 9.57283 & 0.00290 \\
2452930.74725 & 9.57512 & 0.00284 \\
2452930.75138 & 9.56892 & 0.00252 \\
2452930.75542 & 9.56881 & 0.00262 \\
2452930.75941 & 9.57229 & 0.00260 \\
2452930.76347 & 9.57106 & 0.00259 \\
2452930.76764 & 9.56719 & 0.00260 \\
2452930.77167 & 9.57373 & 0.00253 \\
2452930.77565 & 9.56889 & 0.00250 \\
2452930.77971 & 9.57061 & 0.00256 \\
2452930.79186 & 9.57128 & 0.00293 \\
2452930.79990 & 9.57035 & 0.00286 \\
2452930.80392 & 9.57482 & 0.00265 \\
2452930.81606 & 9.57479 & 0.00267 \\
2452930.82004 & 9.56794 & 0.00272 \\
2452930.82402 & 9.57069 & 0.00272 \\
2452930.82806 & 9.57908 & 0.00276 \\
2452930.83217 & 9.56766 & 0.00281 \\
2452930.85223 & 9.57588 & 0.00295 \\
2452930.85621 & 9.55938 & 0.00261 \\
2452931.63461 & 9.57213 & 0.00248 \\
2452931.64274 & 9.56609 & 0.00265 \\
2452931.64675 & 9.56900 & 0.00257 \\
2452931.65073 & 9.56903 & 0.00267 \\
2452931.65471 & 9.57408 & 0.00255 \\
2452931.65888 & 9.56033 & 0.00261 \\
2452931.66674 & 9.56966 & 0.00264 \\
2452931.67072 & 9.57136 & 0.00264 \\
2452931.67482 & 9.57333 & 0.00287 \\
2452931.67887 & 9.57529 & 0.00266 \\
2452931.68285 & 9.57175 & 0.00265 \\
2452931.68684 & 9.57064 & 0.00286 \\
2452931.69094 & 9.56380 & 0.00292 \\
2452931.69497 & 9.56680 & 0.00264 \\
2452931.69900 & 9.56685 & 0.00267 \\
2452931.70299 & 9.56699 & 0.00257 \\
2452931.70716 & 9.56850 & 0.00253 \\
2452931.71114 & 9.57538 & 0.00281 \\
2452931.71519 & 9.56381 & 0.00258 \\
2452931.71923 & 9.56754 & 0.00249 \\
2452931.72335 & 9.56755 & 0.00250 \\
2452931.73132 & 9.57745 & 0.00253 \\
2452931.73942 & 9.56799 & 0.00271 \\
2452931.74345 & 9.56938 & 0.00255 \\
2452931.74743 & 9.56516 & 0.00268 \\
2452931.75144 & 9.56956 & 0.00256 \\
2452931.75556 & 9.56617 & 0.00271 \\
2452931.76353 & 9.57973 & 0.00288 \\
2452931.76756 & 9.57463 & 0.00258 \\
2452931.77166 & 9.57189 & 0.00273 \\
2452931.77564 & 9.56996 & 0.00255 \\
2452931.77970 & 9.56916 & 0.00254 \\
2452931.78780 & 9.56653 & 0.00272 \\
2452931.79181 & 9.56807 & 0.00286 \\
2452931.79578 & 9.57272 & 0.00278 \\
2452931.79976 & 9.56959 & 0.00266 \\
2452931.80390 & 9.57071 & 0.00275 \\
2452931.81200 & 9.57574 & 0.00248 \\
2452931.81598 & 9.56988 & 0.00263 \\
2452931.82009 & 9.56832 & 0.00254 \\
2452931.82408 & 9.57682 & 0.00308 \\
2452931.82810 & 9.57182 & 0.00287 \\
2452931.84433 & 9.56915 & 0.00260 \\
2452931.84831 & 9.57441 & 0.00279 \\
2452931.85241 & 9.57064 & 0.00302 \\
2452932.81146 & 9.57362 & 0.00259 \\
2452932.81546 & 9.58013 & 0.00281 \\
2452932.81950 & 9.57429 & 0.00271 \\
2452932.82359 & 9.57260 & 0.00274 \\
2452932.83973 & 9.57026 & 0.00267 \\
2452932.84383 & 9.57180 & 0.00277 \\
2452932.84783 & 9.57328 & 0.00286 \\
2452932.85188 & 9.57313 & 0.00254 \\
2452933.81197 & 9.57271 & 0.00293 \\
2452933.81597 & 9.56804 & 0.00279 \\
2452933.82001 & 9.57123 & 0.00275 \\
2452933.83617 & 9.57017 & 0.00274 \\
2452933.84011 & 9.57811 & 0.00285 \\
2452933.84421 & 9.57097 & 0.00276 \\
2452933.84820 & 9.56667 & 0.00279 \\
2452934.62878 & 9.55870 & 0.00256 \\
2452934.63282 & 9.57008 & 0.00262 \\
2452934.63680 & 9.57676 & 0.00254 \\
2452934.64097 & 9.56437 & 0.00262 \\
2452934.64495 & 9.56280 & 0.00271 \\
2452934.64893 & 9.56216 & 0.00248 \\
2452934.65297 & 9.56385 & 0.00251 \\
2452934.65709 & 9.57196 & 0.00247 \\
2452934.66113 & 9.57672 & 0.00267 \\
2452934.66517 & 9.56689 & 0.00254 \\
2452934.66913 & 9.56769 & 0.00263 \\
2452934.67324 & 9.57247 & 0.00261 \\
2452934.67731 & 9.56690 & 0.00257 \\
2452934.68130 & 9.56929 & 0.00250 \\
2452934.68527 & 9.57144 & 0.00270 \\
2452934.68945 & 9.56688 & 0.00258 \\
2452934.69350 & 9.57270 & 0.00277 \\
2452934.69754 & 9.57388 & 0.00244 \\
2452934.70151 & 9.56935 & 0.00249 \\
2452934.70569 & 9.56710 & 0.00251 \\
2452934.70967 & 9.56967 & 0.00260 \\
2452934.71366 & 9.56840 & 0.00239 \\
2452934.71773 & 9.56666 & 0.00261 \\
2452934.72184 & 9.56563 & 0.00268 \\
2452934.72583 & 9.57122 & 0.00267 \\
2452934.72980 & 9.57398 & 0.00265 \\
2452934.73783 & 9.57342 & 0.00257 \\
2452934.74188 & 9.57497 & 0.00267 \\
2452934.74587 & 9.56513 & 0.00270 \\
2452934.74983 & 9.57132 & 0.00266 \\
2452934.75798 & 9.58069 & 0.00291 \\
2452934.76197 & 9.56998 & 0.00276 \\
2452934.76593 & 9.56649 & 0.00267 \\
2452934.77012 & 9.57388 & 0.00253 \\
2452934.77415 & 9.56551 & 0.00281 \\
2452934.77820 & 9.57903 & 0.00266 \\
2452934.78217 & 9.57079 & 0.00276 \\
2452934.78628 & 9.56670 & 0.00290 \\
2452934.79025 & 9.56160 & 0.00277 \\
2452934.79428 & 9.57676 & 0.00276 \\
2452934.79827 & 9.58147 & 0.00269 \\
2452934.81040 & 9.57314 & 0.00269 \\
2452934.81436 & 9.57512 & 0.00274 \\
2452934.81853 & 9.56590 & 0.00279 \\
2452934.83471 & 9.55768 & 0.00290 \\
2452934.83869 & 9.57360 & 0.00278 \\
2452934.84273 & 9.57458 & 0.00302 \\
2452935.62392 & 9.56675 & 0.00256 \\
2452935.62789 & 9.57386 & 0.00273 \\
2452935.63193 & 9.57108 & 0.00257 \\
2452935.63590 & 9.56495 & 0.00264 \\
2452935.64007 & 9.55827 & 0.00265 \\
2452935.64411 & 9.57064 & 0.00282 \\
2452935.64816 & 9.56412 & 0.00268 \\
2452935.65220 & 9.57056 & 0.00262 \\
2452935.65637 & 9.56812 & 0.00285 \\
2452935.66040 & 9.57193 & 0.00276 \\
2452935.66445 & 9.56591 & 0.00255 \\
2452935.66851 & 9.57733 & 0.00271 \\
2452935.67269 & 9.57729 & 0.00252 \\
2452935.67668 & 9.57194 & 0.00269 \\
2452935.68065 & 9.57088 & 0.00271 \\
2452935.68471 & 9.57627 & 0.00263 \\
2452935.68889 & 9.57307 & 0.00257 \\
2452935.69294 & 9.57030 & 0.00281 \\
2452935.69698 & 9.57645 & 0.00285 \\
2452935.70102 & 9.56854 & 0.00277 \\
2452935.70514 & 9.57240 & 0.00267 \\
2452935.70913 & 9.57407 & 0.00280 \\
2452935.71317 & 9.57763 & 0.00269 \\
2452935.71721 & 9.56991 & 0.00267 \\
2452935.72137 & 9.56852 & 0.00274 \\
2452935.72536 & 9.56931 & 0.00256 \\
2452935.72941 & 9.57173 & 0.00277 \\
2452935.73339 & 9.56741 & 0.00269 \\
2452935.73749 & 9.56573 & 0.00263 \\
2452935.74156 & 9.57349 & 0.00274 \\
2452935.74554 & 9.56565 & 0.00241 \\
2452935.74953 & 9.56436 & 0.00259 \\
2452935.75364 & 9.57610 & 0.00300 \\
2452935.75760 & 9.57021 & 0.00273 \\
2452935.76157 & 9.57237 & 0.00267 \\
2452935.76563 & 9.57289 & 0.00288 \\
2452935.76976 & 9.56331 & 0.00256 \\
2452935.77770 & 9.57164 & 0.00262 \\
2452935.78172 & 9.57160 & 0.00273 \\
2452935.78588 & 9.56699 & 0.00276 \\
2452935.78986 & 9.57053 & 0.00279 \\
2452935.79384 & 9.57475 & 0.00256 \\
2452935.79786 & 9.57763 & 0.00254 \\
2452935.80600 & 9.56987 & 0.00275 \\
2452935.80998 & 9.57151 & 0.00255 \\
2452935.81398 & 9.55949 & 0.00267 \\
2452935.81815 & 9.56217 & 0.00266 \\
2452935.82208 & 9.57433 & 0.00275 \\
2452935.83421 & 9.56575 & 0.00273 \\
2452935.83816 & 9.56983 & 0.00278 \\
2452935.84220 & 9.56598 & 0.00272 \\
2452936.62327 & 9.56361 & 0.00273 \\
2452936.62732 & 9.56893 & 0.00268 \\
2452936.63131 & 9.56669 & 0.00253 \\
2452936.63538 & 9.56537 & 0.00273 \\
2452936.63955 & 9.57675 & 0.00262 \\
2452936.64361 & 9.56776 & 0.00271 \\
2452936.64762 & 9.56429 & 0.00267 \\
2452936.65160 & 9.56992 & 0.00275 \\
2452936.65572 & 9.57040 & 0.00255 \\
2452936.65975 & 9.57429 & 0.00262 \\
2452936.66379 & 9.56368 & 0.00265 \\
2452936.66783 & 9.56650 & 0.00268 \\
2452936.67202 & 9.57103 & 0.00269 \\
2452936.67605 & 9.57384 & 0.00264 \\
2452936.68008 & 9.56937 & 0.00263 \\
2452936.68408 & 9.57215 & 0.00245 \\
2452936.68819 & 9.57121 & 0.00268 \\
2452936.69224 & 9.57052 & 0.00268 \\
2452936.69628 & 9.57347 & 0.00283 \\
2452936.70435 & 9.57310 & 0.00261 \\
2452936.70838 & 9.57228 & 0.00250 \\
2452936.71242 & 9.56878 & 0.00255 \\
2452936.71641 & 9.57035 & 0.00244 \\
2452936.72052 & 9.57867 & 0.00274 \\
2452936.72449 & 9.56706 & 0.00262 \\
2452936.72847 & 9.57700 & 0.00261 \\
2452936.73243 & 9.57427 & 0.00263 \\
2452936.73656 & 9.56518 & 0.00248 \\
2452936.74055 & 9.57622 & 0.00273 \\
2452936.74455 & 9.56662 & 0.00248 \\
2452936.74854 & 9.57124 & 0.00272 \\
2452936.75265 & 9.57317 & 0.00271 \\
2452936.75670 & 9.57368 & 0.00274 \\
2452936.76071 & 9.57470 & 0.00261 \\
2452936.76475 & 9.57054 & 0.00240 \\
2452936.76894 & 9.57230 & 0.00258 \\
2452936.77292 & 9.56914 & 0.00253 \\
2452936.77688 & 9.58504 & 0.00242 \\
2452936.78086 & 9.56920 & 0.00267 \\
2452936.78497 & 9.57474 & 0.00257 \\
2452936.78902 & 9.57211 & 0.00256 \\
2452936.79300 & 9.56773 & 0.00277 \\
2452936.80112 & 9.58092 & 0.00275 \\
2452936.80515 & 9.56869 & 0.00282 \\
2452936.80913 & 9.57005 & 0.00270 \\
2452936.81307 & 9.57443 & 0.00287 \\
2452936.82924 & 9.57936 & 0.00273 \\
2452936.83336 & 9.57592 & 0.00266 \\
2452936.83733 & 9.56884 & 0.00286 \\
2452937.61828 & 9.56666 & 0.00292 \\
2452937.62238 & 9.56989 & 0.00260 \\
2452937.63031 & 9.56339 & 0.00261 \\
2452937.63433 & 9.57158 & 0.00283 \\
2452937.63840 & 9.57204 & 0.00294 \\
2452937.64239 & 9.57282 & 0.00283 \\
2452937.64645 & 9.56968 & 0.00260 \\
2452937.65049 & 9.56629 & 0.00286 \\
2452937.65461 & 9.56383 & 0.00304 \\
2452937.65858 & 9.57214 & 0.00270 \\
2452937.66262 & 9.56924 & 0.00282 \\
2452937.66665 & 9.57513 & 0.00338 \\
2452937.67077 & 9.56508 & 0.00276 \\
2452937.67479 & 9.56812 & 0.00271 \\
2452937.67884 & 9.57017 & 0.00273 \\
2452937.68281 & 9.56910 & 0.00259 \\
2452937.68693 & 9.56812 & 0.00274 \\
2452937.69091 & 9.56846 & 0.00254 \\
2452937.69495 & 9.56975 & 0.00287 \\
2452937.69894 & 9.56763 & 0.00312 \\
2452937.70303 & 9.56785 & 0.00293 \\
2452937.70703 & 9.56459 & 0.00274 \\
2452937.71100 & 9.56826 & 0.00265 \\
2452937.71498 & 9.56887 & 0.00252 \\
2452937.71916 & 9.57140 & 0.00264 \\
2452937.72323 & 9.56818 & 0.00263 \\
2452937.73121 & 9.56759 & 0.00289 \\
2452937.73538 & 9.56650 & 0.00267 \\
2452937.73937 & 9.56888 & 0.00261 \\
2452937.74333 & 9.57840 & 0.00283 \\
2452937.74731 & 9.57017 & 0.00262 \\
2452937.75148 & 9.57298 & 0.00283 \\
2452937.75552 & 9.57540 & 0.00298 \\
2452937.75951 & 9.57391 & 0.00296 \\
2452937.76348 & 9.57467 & 0.00277 \\
2452937.77169 & 9.57304 & 0.00263 \\
2452937.77574 & 9.57373 & 0.00263 \\
2452937.77973 & 9.57329 & 0.00254 \\
2452937.78387 & 9.56586 & 0.00281 \\
2452937.78788 & 9.57734 & 0.00268 \\
2452937.79187 & 9.56714 & 0.00265 \\
2452937.80003 & 9.57250 & 0.00256 \\
2452937.80405 & 9.57861 & 0.00276 \\
2452937.80804 & 9.56758 & 0.00264 \\
2452937.81198 & 9.56669 & 0.00275 \\
2452937.82809 & 9.57384 & 0.00279 \\
2452937.83214 & 9.56993 & 0.00273 \\
2452937.83614 & 9.56852 & 0.00255 \\
2452938.61760 & 9.55794 & 0.00267 \\
2452938.62174 & 9.57339 & 0.00296 \\
2452938.62572 & 9.57090 & 0.00296 \\
2452938.62975 & 9.57025 & 0.00270 \\
2452938.63373 & 9.57480 & 0.00292 \\
2452938.63787 & 9.56428 & 0.00272 \\
2452938.64186 & 9.57622 & 0.00291 \\
2452938.64589 & 9.57109 & 0.00270 \\
2452938.64988 & 9.57226 & 0.00286 \\
2452938.65400 & 9.57397 & 0.00254 \\
2452938.65804 & 9.55723 & 0.00304 \\
2452938.66211 & 9.56243 & 0.00283 \\
2452938.66608 & 9.56819 & 0.00266 \\
2452938.67423 & 9.57882 & 0.00296 \\
2452938.67820 & 9.57239 & 0.00260 \\
2452938.68224 & 9.57091 & 0.00264 \\
2452938.68636 & 9.56967 & 0.00272 \\
2452938.69034 & 9.56951 & 0.00291 \\
2452938.69432 & 9.57498 & 0.00276 \\
2452938.69836 & 9.56706 & 0.00270 \\
2452938.70247 & 9.56747 & 0.00256 \\
2452938.70646 & 9.56168 & 0.00270 \\
2452938.71044 & 9.57058 & 0.00293 \\
2452938.71447 & 9.58015 & 0.00307 \\
2452938.72251 & 9.57281 & 0.00258 \\
2452938.72647 & 9.57330 & 0.00303 \\
2452938.73045 & 9.56914 & 0.00277 \\
2452938.73457 & 9.57177 & 0.00257 \\
2452938.73853 & 9.57538 & 0.00268 \\
2452938.74252 & 9.56659 & 0.00276 \\
2452938.74649 & 9.56803 & 0.00275 \\
2452938.75060 & 9.57033 & 0.00282 \\
2452938.75463 & 9.57100 & 0.00299 \\
2452938.76269 & 9.56676 & 0.00289 \\
2452938.76685 & 9.55972 & 0.00282 \\
2452938.77476 & 9.58030 & 0.00284 \\
2452938.77874 & 9.57768 & 0.00314 \\
2452938.78283 & 9.56673 & 0.00282 \\
2452938.79086 & 9.57127 & 0.00273 \\
2452938.79487 & 9.56942 & 0.00274 \\
2452938.79901 & 9.57785 & 0.00289 \\
2452938.80306 & 9.56337 & 0.00312 \\
2452938.80711 & 9.56869 & 0.00294 \\
2452938.81108 & 9.57651 & 0.00279 \\
2452938.82719 & 9.56647 & 0.00266 \\
2452938.83135 & 9.57539 & 0.00288 \\
2452940.61207 & 9.56012 & 0.00484 \\
2452940.61609 & 9.56714 & 0.00377 \\
2452940.62021 & 9.56574 & 0.00391 \\
2452940.62423 & 9.57415 & 0.00399 \\
2452940.62820 & 9.58077 & 0.00513 \\
2452940.63223 & 9.57600 & 0.00680 \\
2452940.63632 & 9.56714 & 0.00860 \\
2452940.64426 & 9.57875 & 0.00567 \\
2452940.64823 & 9.56319 & 0.00880 \\
2452940.65623 & 9.58454 & 0.00621 \\
2452940.66025 & 9.56884 & 0.00667 \\
2452940.66835 & 9.57127 & 0.00566 \\
2452940.67638 & 9.56063 & 0.00919 \\
2452940.72043 & 9.59091 & 0.00976 \\
2452940.72444 & 9.56501 & 0.00441 \\
2452940.72847 & 9.56970 & 0.00381 \\
2452940.73259 & 9.56579 & 0.00499 \\
2452940.73661 & 9.56037 & 0.00323 \\
2452940.74463 & 9.58249 & 0.00777 \\
2452940.77671 & 9.55263 & 0.01086 \\
2452940.78079 & 9.58107 & 0.00680 \\
2452940.78475 & 9.56941 & 0.00554 \\
2452940.78877 & 9.58020 & 0.00521 \\
2452940.79279 & 9.56909 & 0.00473 \\
2452940.79694 & 9.55982 & 0.00435 \\
2452940.80097 & 9.58070 & 0.00815 \\
2452940.80903 & 9.56890 & 0.00327 \\
2452940.81720 & 9.57480 & 0.00328 \\
2452940.82117 & 9.57367 & 0.00323 \\
2452940.82522 & 9.57012 & 0.00398 \\
2452940.82934 & 9.57392 & 0.00340 \\
2452941.60789 & 9.56485 & 0.00312 \\
2452941.61186 & 9.57085 & 0.00287 \\
2452941.61584 & 9.57327 & 0.00285 \\
2452941.61995 & 9.56988 & 0.00274 \\
2452941.62394 & 9.57048 & 0.00274 \\
2452941.62797 & 9.57226 & 0.00286 \\
2452941.63195 & 9.56974 & 0.00263 \\
2452941.63614 & 9.56492 & 0.00253 \\
2452941.64018 & 9.57200 & 0.00276 \\
2452941.64422 & 9.57359 & 0.00263 \\
2452941.64825 & 9.57049 & 0.00257 \\
2452941.65238 & 9.56936 & 0.00257 \\
2452941.65636 & 9.57317 & 0.00269 \\
2452941.66036 & 9.56820 & 0.00258 \\
2452941.66440 & 9.57320 & 0.00264 \\
2452941.66852 & 9.56659 & 0.00263 \\
2452941.67251 & 9.57066 & 0.00285 \\
2452941.67648 & 9.56941 & 0.00267 \\
2452941.68046 & 9.56593 & 0.00278 \\
2452941.68463 & 9.56390 & 0.00259 \\
2452941.68869 & 9.57069 & 0.00270 \\
2452941.69272 & 9.57064 & 0.00288 \\
2452941.70077 & 9.57048 & 0.00258 \\
2452941.70476 & 9.57182 & 0.00256 \\
2452941.70881 & 9.57331 & 0.00263 \\
2452941.71285 & 9.57053 & 0.00260 \\
2452941.71696 & 9.57237 & 0.00254 \\
2452941.72100 & 9.57532 & 0.00251 \\
2452941.72498 & 9.57087 & 0.00261 \\
2452941.72902 & 9.56895 & 0.00254 \\
2452941.73312 & 9.57082 & 0.00255 \\
2452941.73711 & 9.56240 & 0.00246 \\
2452941.74109 & 9.56730 & 0.00272 \\
2452941.74512 & 9.57871 & 0.00255 \\
2452941.74923 & 9.57042 & 0.00281 \\
2452941.75321 & 9.57268 & 0.00267 \\
2452941.75719 & 9.57234 & 0.00286 \\
2452941.76122 & 9.56578 & 0.00267 \\
2452941.76534 & 9.57097 & 0.00263 \\
2452941.76931 & 9.56735 & 0.00271 \\
2452941.77327 & 9.56931 & 0.00261 \\
2452941.77732 & 9.56930 & 0.00258 \\
2452941.78143 & 9.58278 & 0.00262 \\
2452941.79351 & 9.57338 & 0.00289 \\
2452941.79768 & 9.57546 & 0.00271 \\
2452941.80166 & 9.57156 & 0.00289 \\
2452941.80565 & 9.56740 & 0.00266 \\
2452941.81778 & 9.57481 & 0.00260 \\
2452941.82175 & 9.57075 & 0.00295 \\
2452941.82576 & 9.57820 & 0.00274 \\
2452942.60337 & 9.58413 & 0.00286 \\
2452942.60741 & 9.58392 & 0.00318 \\
2452942.61142 & 9.57623 & 0.00293 \\
2452942.61544 & 9.57663 & 0.00300 \\
2452942.61956 & 9.57179 & 0.00281 \\
2452942.62358 & 9.58234 & 0.00298 \\
2452942.62755 & 9.57919 & 0.00294 \\
2452942.63159 & 9.57678 & 0.00296 \\
2452942.63573 & 9.58918 & 0.00304 \\
2452942.63972 & 9.57630 & 0.00306 \\
2452942.64369 & 9.58039 & 0.00301 \\
2452942.64768 & 9.57948 & 0.00430 \\
2452942.65969 & 9.56802 & 0.00417 \\
2452942.66372 & 9.56916 & 0.00609 \\
2452942.66787 & 9.56815 & 0.00296 \\
2452942.67192 & 9.57093 & 0.00278 \\
2452942.67595 & 9.56959 & 0.00267 \\
2452942.67998 & 9.57092 & 0.00261 \\
2452942.68415 & 9.57108 & 0.00287 \\
2452942.68812 & 9.56930 & 0.00277 \\
2452942.69217 & 9.57083 & 0.00280 \\
2452942.69620 & 9.56873 & 0.00296 \\
2452942.70032 & 9.55900 & 0.00335 \\
2452942.70438 & 9.57351 & 0.00349 \\
2452942.70836 & 9.57031 & 0.00275 \\
2452942.71239 & 9.57984 & 0.00334 \\
2452942.71649 & 9.57110 & 0.00383 \\
2452942.72052 & 9.56546 & 0.00371 \\
2452942.72452 & 9.57607 & 0.00447 \\
2452942.72847 & 9.57582 & 0.00529 \\
2452942.73256 & 9.57563 & 0.00355 \\
2452942.73659 & 9.57201 & 0.00321 \\
2452942.74056 & 9.57531 & 0.00346 \\
2452942.74460 & 9.56463 & 0.00459 \\
2452942.74869 & 9.57725 & 0.00511 \\
2452942.76072 & 9.57442 & 0.00398 \\
2452942.76487 & 9.56389 & 0.00448 \\
2452942.76884 & 9.57988 & 0.00439 \\
2452942.77281 & 9.56933 & 0.00343 \\
2452942.81679 & 9.56760 & 0.00426 \\
2452942.82075 & 9.59240 & 0.01111 \\
2452943.60256 & 9.57154 & 0.00276 \\
2452943.60659 & 9.57854 & 0.00297 \\
2452943.61063 & 9.57170 & 0.00292 \\
2452943.61468 & 9.56964 & 0.00292 \\
2452943.61878 & 9.56206 & 0.00276 \\
2452943.62277 & 9.57014 & 0.00292 \\
2452943.62681 & 9.57460 & 0.00294 \\
2452943.63085 & 9.56849 & 0.00292 \\
2452943.63498 & 9.56899 & 0.00283 \\
2452943.63896 & 9.57348 & 0.00287 \\
2452943.64301 & 9.56535 & 0.00277 \\
2452943.64700 & 9.56668 & 0.00268 \\
2452943.65109 & 9.56643 & 0.00312 \\
2452943.65514 & 9.57029 & 0.00289 \\
2452943.65912 & 9.57197 & 0.00303 \\
2452943.66312 & 9.57541 & 0.00267 \\
2452943.67122 & 9.57118 & 0.00297 \\
2452943.67520 & 9.57718 & 0.00293 \\
2452943.67919 & 9.56661 & 0.00288 \\
2452943.68725 & 9.57141 & 0.00331 \\
2452943.69123 & 9.56939 & 0.00296 \\
2452943.69520 & 9.57272 & 0.00266 \\
2452943.69937 & 9.56539 & 0.00291 \\
2452943.70342 & 9.56703 & 0.00301 \\
2452943.70748 & 9.57068 & 0.00310 \\
2452943.71144 & 9.57517 & 0.00331 \\
2452943.71560 & 9.57892 & 0.00355 \\
2452943.71958 & 9.57095 & 0.00323 \\
2452943.72353 & 9.57233 & 0.00338 \\
2452943.72759 & 9.57497 & 0.00313 \\
2452943.73170 & 9.56688 & 0.00311 \\
2452943.73966 & 9.56992 & 0.00337 \\
2452943.74769 & 9.57878 & 0.00337 \\
2452943.75173 & 9.55877 & 0.00352 \\
2452943.75974 & 9.56423 & 0.00282 \\
2452943.76390 & 9.56504 & 0.00307 \\
2452943.76787 & 9.56483 & 0.00287 \\
2452943.77185 & 9.56433 & 0.00309 \\
2452943.77584 & 9.58208 & 0.00301 \\
2452943.78803 & 9.57412 & 0.00320 \\
2452943.79202 & 9.56677 & 0.00320 \\
2452943.79611 & 9.57333 & 0.00453 \\
2452943.81625 & 9.56889 & 0.00448 \\
2452943.82017 & 9.56253 & 0.00364 \\
2452944.60957 & 9.57292 & 0.00534 \\
2452944.61355 & 9.57795 & 0.00340 \\
2452944.61766 & 9.57472 & 0.00298 \\
2452944.62170 & 9.57520 & 0.00370 \\
2452944.62574 & 9.57274 & 0.00348 \\
2452944.62978 & 9.57199 & 0.00294 \\
2452944.63391 & 9.56479 & 0.00267 \\
2452944.63796 & 9.56993 & 0.00258 \\
2452944.64193 & 9.56926 & 0.00281 \\
2452944.64593 & 9.58213 & 0.00299 \\
2452944.65007 & 9.54756 & 0.00421 \\
2452944.65410 & 9.55078 & 0.00422 \\
2452944.66626 & 9.57633 & 0.00335 \\
2452944.67031 & 9.56375 & 0.00261 \\
2452944.67433 & 9.57306 & 0.00308 \\
2452944.67835 & 9.57521 & 0.00281 \\
2452944.68250 & 9.57216 & 0.00282 \\
2452944.68648 & 9.56068 & 0.00263 \\
2452944.69049 & 9.56872 & 0.00290 \\
2452944.69451 & 9.56761 & 0.00280 \\
2452944.69861 & 9.56474 & 0.00287 \\
2452944.70267 & 9.55694 & 0.00322 \\
2452944.70667 & 9.57663 & 0.00280 \\
2452944.71061 & 9.57096 & 0.00291 \\
2452944.71472 & 9.57399 & 0.00292 \\
2452944.71879 & 9.56866 & 0.00299 \\
2452944.72278 & 9.56148 & 0.00372 \\
2452944.72675 & 9.55611 & 0.00358 \\
2452944.73091 & 9.56788 & 0.00526 \\
2452944.73488 & 9.56905 & 0.00495 \\
2452944.74284 & 9.54669 & 0.00636 \\
2452944.74700 & 9.57997 & 0.00482 \\
2452944.75494 & 9.56857 & 0.00345 \\
2452944.75892 & 9.56678 & 0.00278 \\
2452944.76303 & 9.57185 & 0.00370 \\
2452944.77101 & 9.56534 & 0.00571 \\
2452944.78319 & 9.58124 & 0.00842 \\
2452944.79117 & 9.57856 & 0.00790 \\
2452944.79525 & 9.56764 & 0.00636 \\
2452944.81144 & 9.56096 & 0.00312 \\
2452944.81542 & 9.57115 & 0.00311 \\
2452945.59741 & 9.57162 & 0.00283 \\
2452945.60149 & 9.58700 & 0.00277 \\
2452945.60547 & 9.58029 & 0.00294 \\
2452945.60944 & 9.57357 & 0.00298 \\
2452945.61756 & 9.57674 & 0.00667 \\
2452945.62152 & 9.57749 & 0.00328 \\
2452945.62557 & 9.58368 & 0.00500 \\
2452945.62955 & 9.57862 & 0.00575 \\
2452945.63363 & 9.57050 & 0.00565 \\
2452945.64151 & 9.58139 & 0.00515 \\
2452945.64546 & 9.56995 & 0.00520 \\
2452945.64955 & 9.58105 & 0.00347 \\
2452945.65353 & 9.57795 & 0.00420 \\
2452945.65758 & 9.57942 & 0.00336 \\
2452945.66157 & 9.57632 & 0.00323 \\
2452945.66568 & 9.57186 & 0.00289 \\
2452945.66963 & 9.57694 & 0.00294 \\
2452945.67362 & 9.57980 & 0.00319 \\
2452945.71713 & 9.58495 & 0.00580 \\
2452945.81280 & 9.57009 & 0.00344 \\
2452948.67106 & 9.57170 & 0.00281 \\
2452948.67514 & 9.57688 & 0.00298 \\
2452948.67912 & 9.57471 & 0.00244 \\
2452948.68312 & 9.58482 & 0.00257 \\
2452948.68725 & 9.57770 & 0.00257 \\
2452948.69126 & 9.57874 & 0.00275 \\
2452948.69922 & 9.57703 & 0.00282 \\
2452948.70335 & 9.57697 & 0.00276 \\
2452948.70738 & 9.57793 & 0.00288 \\
2452948.71143 & 9.57049 & 0.00301 \\
2452948.71541 & 9.57481 & 0.00279 \\
2452948.71952 & 9.57602 & 0.00311 \\
2452948.72355 & 9.57706 & 0.00284 \\
2452948.72753 & 9.58105 & 0.00275 \\
2452948.73151 & 9.57933 & 0.00307 \\
2452948.73569 & 9.57839 & 0.00285 \\
2452948.74367 & 9.57812 & 0.00270 \\
2452948.74764 & 9.58050 & 0.00291 \\
2452948.75175 & 9.57883 & 0.00277 \\
2452948.75579 & 9.57120 & 0.00283 \\
2452948.75975 & 9.56585 & 0.00258 \\
2452948.76376 & 9.57128 & 0.00267 \\
2452948.77191 & 9.57512 & 0.00282 \\
2452948.77595 & 9.57441 & 0.00270 \\
2452948.77998 & 9.57278 & 0.00284 \\
2452948.78412 & 9.56700 & 0.00289 \\
2452948.78811 & 9.57839 & 0.00297 \\
2452948.80020 & 9.56179 & 0.00309 \\
2452948.80418 & 9.56980 & 0.00277 \\
2452949.58707 & 9.56978 & 0.00289 \\
2452949.59109 & 9.56828 & 0.00290 \\
2452949.59509 & 9.57663 & 0.00299 \\
2452949.59920 & 9.56745 & 0.00262 \\
2452949.60318 & 9.55901 & 0.00285 \\
2452949.60716 & 9.55919 & 0.00276 \\
2452949.61120 & 9.56824 & 0.00291 \\
2452949.61535 & 9.56713 & 0.00295 \\
2452949.61935 & 9.56919 & 0.00255 \\
2452949.62330 & 9.57336 & 0.00275 \\
2452949.62730 & 9.56760 & 0.00295 \\
2452949.63146 & 9.55846 & 0.00282 \\
2452949.63545 & 9.55934 & 0.00272 \\
2452949.63949 & 9.56771 & 0.00287 \\
2452949.64352 & 9.57055 & 0.00277 \\
2452949.64769 & 9.56570 & 0.00269 \\
2452949.65169 & 9.56664 & 0.00283 \\
2452949.65563 & 9.56588 & 0.00278 \\
2452949.65970 & 9.57387 & 0.00257 \\
2452949.66380 & 9.57335 & 0.00273 \\
2452949.66782 & 9.57046 & 0.00274 \\
2452949.67181 & 9.56611 & 0.00289 \\
2452949.67579 & 9.56774 & 0.00308 \\
2452949.67990 & 9.57195 & 0.00256 \\
2452949.68393 & 9.57117 & 0.00269 \\
2452949.69184 & 9.57489 & 0.00277 \\
2452949.69595 & 9.57017 & 0.00294 \\
2452949.69995 & 9.56960 & 0.00275 \\
2452949.70395 & 9.56356 & 0.00276 \\
2452949.70793 & 9.57647 & 0.00311 \\
2452949.71205 & 9.56030 & 0.00254 \\
2452949.71605 & 9.56252 & 0.00247 \\
2452949.72007 & 9.56924 & 0.00280 \\
2452949.72406 & 9.56944 & 0.00304 \\
2452949.72817 & 9.56429 & 0.00281 \\
2452949.73219 & 9.56236 & 0.00290 \\
2452949.74014 & 9.57083 & 0.00289 \\
2452949.74425 & 9.56746 & 0.00280 \\
2452949.74829 & 9.56530 & 0.00304 \\
2452949.75226 & 9.56964 & 0.00270 \\
2452949.75624 & 9.55427 & 0.00281 \\
2452949.76041 & 9.56020 & 0.00282 \\
2452949.76849 & 9.57191 & 0.00310 \\
2452949.77254 & 9.56416 & 0.00277 \\
2452949.77670 & 9.56728 & 0.00315 \\
2452949.78075 & 9.57620 & 0.00287 \\
2452949.79287 & 9.57160 & 0.00301 \\
2452949.80087 & 9.56869 & 0.00286 \\
2452950.64285 & 9.57469 & 0.00276 \\
2452950.64688 & 9.56891 & 0.00302 \\
2452950.65085 & 9.57430 & 0.00284 \\
2452950.65485 & 9.57215 & 0.00326 \\
2452950.65895 & 9.56789 & 0.00273 \\
2452950.66299 & 9.57176 & 0.00308 \\
2452950.66704 & 9.56286 & 0.00291 \\
2452950.67107 & 9.56364 & 0.00303 \\
2452950.67519 & 9.56221 & 0.00294 \\
2452950.67923 & 9.57330 & 0.00309 \\
2452950.68325 & 9.57056 & 0.00295 \\
2452950.68723 & 9.56797 & 0.00341 \\
2452950.69134 & 9.57031 & 0.00303 \\
2452950.69529 & 9.57296 & 0.00285 \\
2452950.69932 & 9.56746 & 0.00282 \\
2452950.70331 & 9.56906 & 0.00283 \\
2452950.70747 & 9.56781 & 0.00274 \\
2452950.71147 & 9.56731 & 0.00276 \\
2452950.71545 & 9.57599 & 0.00309 \\
2452950.71941 & 9.56807 & 0.00258 \\
2452950.72352 & 9.56905 & 0.00318 \\
2452950.73144 & 9.57213 & 0.00296 \\
2452950.73961 & 9.57085 & 0.00291 \\
2452950.74359 & 9.57072 & 0.00316 \\
2452950.74755 & 9.56422 & 0.00306 \\
2452950.75159 & 9.56364 & 0.00287 \\
2452950.75576 & 9.56409 & 0.00271 \\
2452950.76781 & 9.56951 & 0.00308 \\
2452950.77198 & 9.56937 & 0.00315 \\
2452950.77596 & 9.57782 & 0.00321 \\
2452950.77994 & 9.56098 & 0.00319 \\
2452950.79206 & 9.56882 & 0.00291 \\
2452950.79609 & 9.57032 & 0.00279 \\
2452950.80006 & 9.56709 & 0.00340 \\
2452951.69141 & 9.56500 & 0.00301 \\
2452951.69548 & 9.56114 & 0.00300 \\
2452951.69951 & 9.56591 & 0.00307 \\
2452951.70353 & 9.57440 & 0.00298 \\
2452951.70765 & 9.57160 & 0.00291 \\
2452951.71167 & 9.57506 & 0.00299 \\
2452951.71566 & 9.56141 & 0.00298 \\
2452951.71963 & 9.56528 & 0.00281 \\
2452951.72373 & 9.57195 & 0.00324 \\
2452951.72777 & 9.57449 & 0.00334 \\
2452951.73174 & 9.57758 & 0.00297 \\
2452951.73988 & 9.57724 & 0.00257 \\
2452951.74385 & 9.56852 & 0.00271 \\
2452951.74788 & 9.57830 & 0.00294 \\
2452951.75185 & 9.57700 & 0.00271 \\
2452951.76399 & 9.57485 & 0.00293 \\
2452951.76796 & 9.57735 & 0.00316 \\
2452951.77208 & 9.58075 & 0.00301 \\
2452951.77609 & 9.57898 & 0.00279 \\
2452951.78829 & 9.57742 & 0.00267 \\
2452951.79227 & 9.56855 & 0.00314 \\
2452951.79632 & 9.58055 & 0.00266 \\
2452952.57751 & 9.56068 & 0.00279 \\
2452952.58168 & 9.56757 & 0.00287 \\
2452952.58567 & 9.56560 & 0.00286 \\
2452952.58974 & 9.56226 & 0.00271 \\
2452952.59373 & 9.56066 & 0.00267 \\
2452952.59789 & 9.56943 & 0.00256 \\
2452952.60192 & 9.56573 & 0.00267 \\
2452952.60588 & 9.56406 & 0.00276 \\
2452952.60987 & 9.56539 & 0.00269 \\
2452952.61397 & 9.57067 & 0.00276 \\
2452952.61795 & 9.56927 & 0.00277 \\
2452952.62191 & 9.57308 & 0.00295 \\
2452952.62587 & 9.57036 & 0.00309 \\
2452952.63392 & 9.57779 & 0.00293 \\
2452952.63789 & 9.57220 & 0.00288 \\
2452952.64188 & 9.56994 & 0.00309 \\
2452952.64601 & 9.57385 & 0.00310 \\
2452952.64999 & 9.57257 & 0.00283 \\
2452952.65404 & 9.57126 & 0.00277 \\
2452952.65807 & 9.56725 & 0.00297 \\
2452952.66219 & 9.57444 & 0.00297 \\
2452952.66615 & 9.56187 & 0.00332 \\
2452952.67012 & 9.57793 & 0.00293 \\
2452952.67416 & 9.56343 & 0.00292 \\
2452952.67832 & 9.56965 & 0.00322 \\
2452952.68235 & 9.56520 & 0.00297 \\
2452952.68639 & 9.56683 & 0.00310 \\
2452952.69037 & 9.56729 & 0.00314 \\
2452952.69448 & 9.58108 & 0.00310 \\
2452952.69852 & 9.56752 & 0.00311 \\
2452952.70250 & 9.55895 & 0.00290 \\
2452952.70655 & 9.56385 & 0.00320 \\
2452952.71071 & 9.56882 & 0.00283 \\
2452952.71469 & 9.56505 & 0.00296 \\
2452952.71868 & 9.56266 & 0.00302 \\
2452952.72271 & 9.56871 & 0.00285 \\
2452952.73486 & 9.57434 & 0.00312 \\
2452952.73884 & 9.56833 & 0.00305 \\
2452952.74294 & 9.57153 & 0.00283 \\
2452952.74691 & 9.56617 & 0.00268 \\
2452952.76304 & 9.57400 & 0.00311 \\
2452952.76702 & 9.57154 & 0.00291 \\
2452952.77100 & 9.57086 & 0.00319 \\
2452952.77509 & 9.56352 & 0.00311 \\
2452952.78712 & 9.56634 & 0.00308 \\
2452952.79128 & 9.57860 & 0.00351 \\
2452952.79524 & 9.56475 & 0.00280 \\
2452953.57300 & 9.57710 & 0.00288 \\
2452953.57697 & 9.57486 & 0.00270 \\
2452953.58113 & 9.56425 & 0.00293 \\
2452953.58511 & 9.57027 & 0.00283 \\
2452953.58916 & 9.55944 & 0.00320 \\
2452953.59314 & 9.57546 & 0.00296 \\
2452953.59729 & 9.57431 & 0.00312 \\
2452953.60127 & 9.57743 & 0.00301 \\
2452953.60523 & 9.57654 & 0.00284 \\
2452953.60923 & 9.57941 & 0.00290 \\
2452953.61333 & 9.56594 & 0.00301 \\
2452953.61731 & 9.56476 & 0.00266 \\
2452953.62130 & 9.56651 & 0.00285 \\
2452953.62938 & 9.57225 & 0.00288 \\
2452953.63344 & 9.57633 & 0.00303 \\
2452953.63740 & 9.56430 & 0.00285 \\
2452953.64145 & 9.56602 & 0.00301 \\
2452953.64561 & 9.57507 & 0.00282 \\
2452953.64958 & 9.56005 & 0.00274 \\
2452953.65357 & 9.57486 & 0.00292 \\
2452953.65761 & 9.57224 & 0.00290 \\
2452953.66172 & 9.57728 & 0.00305 \\
2452953.66576 & 9.56894 & 0.00307 \\
2452953.66981 & 9.56975 & 0.00270 \\
2452953.67380 & 9.57155 & 0.00305 \\
2452953.67790 & 9.57195 & 0.00309 \\
2452953.68187 & 9.56794 & 0.00266 \\
2452953.68584 & 9.57494 & 0.00274 \\
2452953.68987 & 9.56883 & 0.00272 \\
2452953.69406 & 9.56774 & 0.00324 \\
2452953.69810 & 9.57023 & 0.00271 \\
2452953.70215 & 9.56415 & 0.00289 \\
2452953.70614 & 9.56353 & 0.00299 \\
2452953.71025 & 9.56990 & 0.00296 \\
2452953.71430 & 9.57124 & 0.00282 \\
2452953.71827 & 9.57302 & 0.00297 \\
2452953.72231 & 9.56956 & 0.00322 \\
2452953.73045 & 9.57324 & 0.00282 \\
2452953.73443 & 9.56759 & 0.00282 \\
2452953.73842 & 9.57016 & 0.00300 \\
2452953.74259 & 9.57482 & 0.00268 \\
2452953.74656 & 9.56206 & 0.00301 \\
2452953.75053 & 9.56863 & 0.00282 \\
2452953.75861 & 9.56456 & 0.00293 \\
2452953.76265 & 9.57833 & 0.00295 \\
2452953.76661 & 9.57088 & 0.00296 \\
2452953.77064 & 9.57740 & 0.00317 \\
2452953.78672 & 9.56962 & 0.00301 \\
2452953.79083 & 9.55722 & 0.00336 \\
2452958.68041 & 9.56237 & 0.00254 \\
2452958.68447 & 9.57172 & 0.00256 \\
2452958.68852 & 9.56775 & 0.00281 \\
2452958.69249 & 9.57021 & 0.00251 \\
2452958.69662 & 9.56888 & 0.00254 \\
2452958.70066 & 9.57173 & 0.00258 \\
2452958.70466 & 9.57019 & 0.00282 \\
2452958.70870 & 9.56617 & 0.00282 \\
2452958.71287 & 9.57719 & 0.00257 \\
2452958.71691 & 9.56304 & 0.00263 \\
2452958.72095 & 9.56532 & 0.00272 \\
2452958.72493 & 9.57815 & 0.00288 \\
2452958.72900 & 9.57376 & 0.00322 \\
2452959.61342 & 9.57617 & 0.00269 \\
2452959.61746 & 9.57523 & 0.00249 \\
2452959.62145 & 9.56997 & 0.00254 \\
2452959.62556 & 9.56971 & 0.00263 \\
2452959.62960 & 9.57392 & 0.00254 \\
2452959.63364 & 9.57432 & 0.00256 \\
2452959.63768 & 9.56416 & 0.00265 \\
2452959.64178 & 9.56939 & 0.00265 \\
2452959.64582 & 9.57547 & 0.00260 \\
2452959.64981 & 9.58056 & 0.00261 \\
2452959.65379 & 9.56416 & 0.00260 \\
2452959.65801 & 9.56490 & 0.00244 \\
2452959.66199 & 9.57557 & 0.00247 \\
2452959.66603 & 9.57032 & 0.00257 \\
2452959.67009 & 9.57501 & 0.00263 \\
2452959.67421 & 9.56787 & 0.00250 \\
2452959.67818 & 9.56714 & 0.00254 \\
2452959.68221 & 9.56728 & 0.00254 \\
2452959.68620 & 9.56749 & 0.00250 \\
2452959.69038 & 9.56582 & 0.00262 \\
2452959.69834 & 9.57062 & 0.00239 \\
2452959.70240 & 9.56795 & 0.00262 \\
2452959.70657 & 9.56565 & 0.00268 \\
2452959.71061 & 9.57093 & 0.00253 \\
2452959.71467 & 9.56230 & 0.00259 \\
2452959.71863 & 9.57214 & 0.00286 \\
2452959.72273 & 9.56998 & 0.00261 \\
2452959.72674 & 9.57458 & 0.00273 \\
2452959.73071 & 9.56517 & 0.00246 \\
2452959.73476 & 9.57931 & 0.00283 \\
2452959.74286 & 9.56737 & 0.00269 \\
2452959.74690 & 9.57219 & 0.00269 \\
2452959.75088 & 9.56521 & 0.00266 \\
2452959.75501 & 9.56968 & 0.00280 \\
2452959.77109 & 9.56870 & 0.00274 \\
2452959.77511 & 9.57751 & 0.00288 \\
2452959.77914 & 9.56907 & 0.00260 \\
2452961.57034 & 9.58046 & 0.00255 \\
2452961.57847 & 9.57443 & 0.00262 \\
2452961.58251 & 9.57118 & 0.00260 \\
2452961.58649 & 9.56687 & 0.00250 \\
2452961.59046 & 9.56338 & 0.00272 \\
2452961.59855 & 9.57413 & 0.00247 \\
2452961.60252 & 9.57064 & 0.00251 \\
2452961.60657 & 9.56466 & 0.00266 \\
2452961.61068 & 9.56768 & 0.00254 \\
2452961.61468 & 9.56593 & 0.00241 \\
2452961.61872 & 9.56502 & 0.00257 \\
2452961.62271 & 9.56997 & 0.00260 \\
2452961.62682 & 9.57361 & 0.00262 \\
2452961.63080 & 9.57451 & 0.00250 \\
2452961.63485 & 9.56992 & 0.00259 \\
2452961.63887 & 9.57882 & 0.00274 \\
2452961.64303 & 9.56349 & 0.00260 \\
2452961.64701 & 9.55944 & 0.00255 \\
2452961.65105 & 9.56488 & 0.00250 \\
2452961.65504 & 9.57524 & 0.00741 \\
2452961.65913 & 9.57526 & 0.00248 \\
2452961.66314 & 9.57701 & 0.00263 \\
2452961.66714 & 9.56742 & 0.00252 \\
2452961.67117 & 9.57091 & 0.00250 \\
2452961.67528 & 9.56793 & 0.00258 \\
2452961.67932 & 9.56988 & 0.00258 \\
2452961.68330 & 9.56836 & 0.00279 \\
2452961.68728 & 9.57870 & 0.00252 \\
2452961.69139 & 9.57600 & 0.00258 \\
2452961.69532 & 9.56998 & 0.00251 \\
2452961.70326 & 9.58138 & 0.00275 \\
2452961.70743 & 9.56852 & 0.00249 \\
2452961.71141 & 9.57119 & 0.00243 \\
2452961.71542 & 9.57072 & 0.00257 \\
2452961.71939 & 9.57186 & 0.00258 \\
2452961.72354 & 9.57345 & 0.00253 \\
2452961.72752 & 9.57578 & 0.00254 \\
2452961.73550 & 9.57099 & 0.00268 \\
2452961.73963 & 9.57341 & 0.00253 \\
2452961.74361 & 9.56928 & 0.00269 \\
2452961.74759 & 9.56295 & 0.00250 \\
2452961.75153 & 9.56391 & 0.00270 \\
2452961.76371 & 9.57423 & 0.00253 \\
2452961.76775 & 9.56619 & 0.00261 \\
2452961.77192 & 9.56693 & 0.00266 \\
2452961.77595 & 9.56669 & 0.00265 \\
2452961.77996 & 9.57746 & 0.00257 \\
2452962.57379 & 9.56338 & 0.00261 \\
2452962.57776 & 9.57352 & 0.00275 \\
2452962.58187 & 9.56614 & 0.00279 \\
2452962.58589 & 9.57074 & 0.00254 \\
2452962.58986 & 9.56390 & 0.00248 \\
2452962.59388 & 9.56777 & 0.00258 \\
2452962.59801 & 9.56281 & 0.00259 \\
2452962.60205 & 9.56824 & 0.00257 \\
2452962.60603 & 9.56714 & 0.00249 \\
2452962.60999 & 9.57186 & 0.00270 \\
2452962.66893 & 9.57635 & 0.00253 \\
2452962.67300 & 9.57045 & 0.00270 \\
2452962.67702 & 9.57302 & 0.00257 \\
2452962.68101 & 9.56031 & 0.00258 \\
2452962.68512 & 9.56697 & 0.00261 \\
2452962.68916 & 9.56436 & 0.00283 \\
2452962.69322 & 9.56470 & 0.00272 \\
2452962.70138 & 9.56634 & 0.00263 \\
2452962.70538 & 9.57306 & 0.00265 \\
2452962.70936 & 9.57116 & 0.00269 \\
2452962.71334 & 9.55997 & 0.00266 \\
2452962.71744 & 9.56843 & 0.00275 \\
2452962.72144 & 9.56222 & 0.00264 \\
2452962.72546 & 9.57285 & 0.00267 \\
2452962.73364 & 9.56777 & 0.00285 \\
2452962.73761 & 9.56593 & 0.00272 \\
2452962.74158 & 9.57582 & 0.00281 \\
2452962.74562 & 9.56824 & 0.00275 \\
2452962.74972 & 9.57217 & 0.00263 \\
2452962.76164 & 9.56256 & 0.00276 \\
2452962.76581 & 9.57216 & 0.00290 \\
2452962.76977 & 9.56487 & 0.00263 \\
2452962.77376 & 9.56729 & 0.00295 \\
2452962.78590 & 9.57540 & 0.00305 \\
2452963.56568 & 9.57232 & 0.00272 \\
2452963.56967 & 9.57369 & 0.00273 \\
2452963.57368 & 9.56466 & 0.00279 \\
2452963.57778 & 9.57725 & 0.00268 \\
2452963.58177 & 9.56647 & 0.00259 \\
2452963.58577 & 9.57346 & 0.00294 \\
2452963.58975 & 9.56859 & 0.00275 \\
2452963.59389 & 9.56663 & 0.00271 \\
2452963.59789 & 9.56633 & 0.00251 \\
2452963.60190 & 9.57464 & 0.00272 \\
2452963.60592 & 9.56837 & 0.00271 \\
2452963.61004 & 9.57384 & 0.00273 \\
2452963.61405 & 9.57305 & 0.00271 \\
2452963.61805 & 9.57210 & 0.00264 \\
2452963.62202 & 9.56927 & 0.00271 \\
2452963.62620 & 9.57054 & 0.00266 \\
2452963.63018 & 9.57177 & 0.00286 \\
2452963.63419 & 9.56684 & 0.00260 \\
2452963.63816 & 9.56952 & 0.00265 \\
2452963.64228 & 9.56795 & 0.00259 \\
2452963.64633 & 9.57113 & 0.00279 \\
2452963.65032 & 9.56213 & 0.00276 \\
2452963.65430 & 9.56485 & 0.00249 \\
2452963.65843 & 9.57738 & 0.00262 \\
2452963.66240 & 9.57537 & 0.00255 \\
2452963.66639 & 9.57317 & 0.00263 \\
2452963.67044 & 9.56596 & 0.00278 \\
2452963.67457 & 9.56975 & 0.00287 \\
2452963.67854 & 9.56975 & 0.00264 \\
2452963.68254 & 9.57213 & 0.00262 \\
2452963.69190 & 9.56677 & 0.00266 \\
2452963.69978 & 9.57436 & 0.00284 \\
2452963.70369 & 9.57029 & 0.00259 \\
2452963.70783 & 9.56271 & 0.00258 \\
2452963.71175 & 9.56978 & 0.00262 \\
2452963.71567 & 9.57344 & 0.00297 \\
2452963.71959 & 9.56760 & 0.00256 \\
2452963.72364 & 9.57127 & 0.00282 \\
2452963.73148 & 9.57262 & 0.00300 \\
2452963.73943 & 9.57606 & 0.00301 \\
2452963.74338 & 9.58129 & 0.00274 \\
2452963.74734 & 9.57721 & 0.00281 \\
2452963.75925 & 9.57042 & 0.00254 \\
2452963.76316 & 9.57498 & 0.00289 \\
2452963.76711 & 9.55855 & 0.00289 \\
2452963.78301 & 9.56434 & 0.00255 \\
2452964.56068 & 9.56521 & 0.00271 \\
2452964.56466 & 9.57334 & 0.00298 \\
2452964.56858 & 9.57784 & 0.00263 \\
2452964.57246 & 9.57375 & 0.00270 \\
2452964.57650 & 9.56759 & 0.00253 \\
2452964.58050 & 9.56854 & 0.00258 \\
2452964.58448 & 9.56629 & 0.00245 \\
2452964.58842 & 9.57070 & 0.00258 \\
2452964.59255 & 9.56960 & 0.00269 \\
2452964.59647 & 9.56515 & 0.00247 \\
2452964.60045 & 9.56132 & 0.00267 \\
2452964.60438 & 9.57863 & 0.00281 \\
2452964.60844 & 9.56785 & 0.00279 \\
2452964.61235 & 9.57498 & 0.00251 \\
2452964.61630 & 9.57158 & 0.00246 \\
2452964.62022 & 9.56694 & 0.00280 \\
2452964.62428 & 9.54921 & 0.00261 \\
2452964.62821 & 9.57427 & 0.00265 \\
2452964.63213 & 9.57585 & 0.00271 \\
2452964.63604 & 9.57471 & 0.00250 \\
2452964.64010 & 9.56805 & 0.00258 \\
2452964.64408 & 9.57485 & 0.00251 \\
2452964.64808 & 9.56490 & 0.00263 \\
2452964.65199 & 9.56625 & 0.00279 \\
2452964.65604 & 9.57400 & 0.00253 \\
2452964.66002 & 9.58172 & 0.00265 \\
2452964.66393 & 9.57851 & 0.00273 \\
2452964.66788 & 9.57224 & 0.00258 \\
2452964.67194 & 9.56626 & 0.00266 \\
2452964.67586 & 9.56886 & 0.00282 \\
2452964.67977 & 9.57265 & 0.00268 \\
2452964.68369 & 9.56662 & 0.00265 \\
2452964.68777 & 9.57942 & 0.00259 \\
2452964.69559 & 9.58185 & 0.00272 \\
2452964.69952 & 9.57725 & 0.00295 \\
2452964.70357 & 9.56810 & 0.00266 \\
2452964.70747 & 9.56403 & 0.00266 \\
2452964.71142 & 9.57318 & 0.00253 \\
2452964.71535 & 9.56716 & 0.00265 \\
2452964.71941 & 9.56368 & 0.00248 \\
2452964.72333 & 9.57058 & 0.00278 \\
2452964.73120 & 9.57000 & 0.00246 \\
2452964.73525 & 9.57087 & 0.00266 \\
2452964.73925 & 9.57315 & 0.00264 \\
2452964.75507 & 9.57106 & 0.00283 \\
2452964.75907 & 9.57529 & 0.00282 \\
2452964.76299 & 9.57696 & 0.00300 \\
2452964.76706 & 9.56284 & 0.00269 \\
2452964.77104 & 9.56197 & 0.00264 \\
2452965.56184 & 9.57541 & 0.00270 \\
2452965.56578 & 9.57469 & 0.00259 \\
2452965.56972 & 9.56634 & 0.00260 \\
2452965.57364 & 9.57001 & 0.00256 \\
2452965.57770 & 9.56562 & 0.00250 \\
2452965.58164 & 9.56227 & 0.00260 \\
2452965.58556 & 9.58132 & 0.00262 \\
2452965.58949 & 9.56207 & 0.00257 \\
2452965.59354 & 9.56798 & 0.00260 \\
2452965.59746 & 9.56920 & 0.00261 \\
2452965.60141 & 9.57215 & 0.00254 \\
2452965.60539 & 9.56352 & 0.00261 \\
2452965.60945 & 9.57083 & 0.00258 \\
2452965.61340 & 9.57226 & 0.00274 \\
2452965.61739 & 9.56432 & 0.00247 \\
2452965.62134 & 9.57285 & 0.00264 \\
2452965.62542 & 9.57261 & 0.00268 \\
2452965.62933 & 9.57230 & 0.00272 \\
2452965.63329 & 9.57658 & 0.00250 \\
2452965.63720 & 9.56963 & 0.00248 \\
2452965.64124 & 9.57344 & 0.00250 \\
2452965.64519 & 9.56742 & 0.00257 \\
2452965.65300 & 9.56650 & 0.00261 \\
2452965.65712 & 9.57236 & 0.00258 \\
2452965.66107 & 9.57515 & 0.00262 \\
2452965.66505 & 9.56530 & 0.00254 \\
2452965.66905 & 9.56829 & 0.00260 \\
2452965.67310 & 9.57230 & 0.00250 \\
2452965.67704 & 9.56444 & 0.00276 \\
2452965.68104 & 9.56507 & 0.00252 \\
2452965.68495 & 9.56785 & 0.00248 \\
2452965.68901 & 9.56581 & 0.00271 \\
2452965.69691 & 9.57610 & 0.00267 \\
2452965.70084 & 9.57084 & 0.00262 \\
2452965.70488 & 9.56493 & 0.00260 \\
2452965.70881 & 9.57667 & 0.00269 \\
2452965.71276 & 9.56266 & 0.00260 \\
2452965.71668 & 9.57854 & 0.00310 \\
2452965.72470 & 9.57629 & 0.00296 \\
2452965.72861 & 9.57650 & 0.00275 \\
2452965.73256 & 9.56666 & 0.00262 \\
2452965.73663 & 9.57228 & 0.00257 \\
2452965.74055 & 9.56952 & 0.00255 \\
2452965.74453 & 9.57161 & 0.00294 \\
2452965.74846 & 9.57598 & 0.00290 \\
2452965.75643 & 9.56366 & 0.00297 \\
2452965.76035 & 9.57192 & 0.00303 \\
2452965.76428 & 9.56125 & 0.00275 \\
2452966.56023 & 9.57656 & 0.00269 \\
2452966.56417 & 9.56324 & 0.00278 \\
2452966.56810 & 9.57524 & 0.00270 \\
2452966.57207 & 9.56849 & 0.00249 \\
2452966.57613 & 9.56933 & 0.00252 \\
2452966.58009 & 9.57289 & 0.00264 \\
2452966.58402 & 9.56950 & 0.00251 \\
2452966.58794 & 9.57047 & 0.00255 \\
2452966.59199 & 9.57579 & 0.00266 \\
2452966.59592 & 9.56368 & 0.00247 \\
2452966.59987 & 9.56925 & 0.00257 \\
2452966.60379 & 9.56976 & 0.00255 \\
2452966.60782 & 9.57326 & 0.00257 \\
2452966.61175 & 9.56625 & 0.00258 \\
2452966.61568 & 9.56667 & 0.00267 \\
2452966.61961 & 9.56854 & 0.00258 \\
2452966.62375 & 9.56908 & 0.00261 \\
2452966.62768 & 9.57503 & 0.00253 \\
2452966.63159 & 9.56933 & 0.00249 \\
2452966.63548 & 9.55861 & 0.00244 \\
2452966.64346 & 9.56857 & 0.00238 \\
2452966.64734 & 9.56622 & 0.00246 \\
2452966.65127 & 9.57149 & 0.00267 \\
2452966.65538 & 9.57044 & 0.00256 \\
2452966.65931 & 9.57160 & 0.00254 \\
2452966.66325 & 9.56470 & 0.00249 \\
2452966.66717 & 9.57314 & 0.00260 \\
2452966.67133 & 9.57083 & 0.00255 \\
2452966.67912 & 9.56883 & 0.00250 \\
2452966.68305 & 9.56537 & 0.00254 \\
2452966.69101 & 9.57674 & 0.00265 \\
2452966.69494 & 9.57225 & 0.00261 \\
2452966.69887 & 9.57261 & 0.00252 \\
2452966.70291 & 9.56724 & 0.00258 \\
2452966.70683 & 9.56983 & 0.00249 \\
2452966.71079 & 9.56443 & 0.00254 \\
2452966.71472 & 9.56421 & 0.00252 \\
2452966.71878 & 9.57041 & 0.00276 \\
2452966.72271 & 9.57059 & 0.00255 \\
2452966.72663 & 9.57048 & 0.00251 \\
2452966.73055 & 9.56678 & 0.00258 \\
2452966.73461 & 9.57071 & 0.00270 \\
2452966.73852 & 9.57456 & 0.00245 \\
2452966.74244 & 9.57502 & 0.00246 \\
2452966.74632 & 9.57283 & 0.00260 \\
2452966.75038 & 9.56503 & 0.00284 \\
2452966.75430 & 9.57727 & 0.00275 \\
2452966.75822 & 9.56809 & 0.00264 \\
2452966.76222 & 9.56679 & 0.00258 \\
2452966.77407 & 9.56731 & 0.00284 \\
2452967.56003 & 9.56150 & 0.00273 \\
2452967.56398 & 9.56622 & 0.00297 \\
2452967.56795 & 9.56497 & 0.00278 \\
2452967.57193 & 9.57471 & 0.00256 \\
2452967.57599 & 9.57456 & 0.00262 \\
2452967.57990 & 9.57693 & 0.00274 \\
2452967.58383 & 9.57398 & 0.00276 \\
2452967.58775 & 9.56985 & 0.00260 \\
2452967.59186 & 9.56781 & 0.00265 \\
2452967.59578 & 9.56985 & 0.00259 \\
2452967.59973 & 9.57042 & 0.00262 \\
2452967.60366 & 9.56440 & 0.00258 \\
2452967.60771 & 9.57650 & 0.00265 \\
2452967.61160 & 9.56596 & 0.00260 \\
2452967.61559 & 9.57224 & 0.00269 \\
2452967.61951 & 9.56325 & 0.00258 \\
2452967.62356 & 9.56737 & 0.00246 \\
2452967.62757 & 9.57083 & 0.00259 \\
2452967.63149 & 9.56481 & 0.00245 \\
2452967.63545 & 9.56536 & 0.00257 \\
2452967.63957 & 9.57077 & 0.00270 \\
2452967.64350 & 9.56302 & 0.00255 \\
2452967.64744 & 9.56355 & 0.00273 \\
2452967.65137 & 9.57218 & 0.00247 \\
2452967.65931 & 9.56903 & 0.00255 \\
2452967.66329 & 9.57051 & 0.00266 \\
2452967.66728 & 9.57300 & 0.00267 \\
2452967.67140 & 9.57014 & 0.00279 \\
2452967.67540 & 9.56975 & 0.00250 \\
2452967.67935 & 9.57101 & 0.00234 \\
2452967.68326 & 9.57621 & 0.00274 \\
2452967.68733 & 9.56394 & 0.00257 \\
2452967.69124 & 9.56919 & 0.00252 \\
2452967.69517 & 9.56892 & 0.00263 \\
2452967.69910 & 9.56799 & 0.00256 \\
2452967.70321 & 9.57217 & 0.00272 \\
2452967.70720 & 9.56955 & 0.00259 \\
2452967.71118 & 9.57543 & 0.00242 \\
2452967.71513 & 9.58006 & 0.00252 \\
2452967.72310 & 9.57526 & 0.00273 \\
2452967.72702 & 9.56761 & 0.00256 \\
2452967.73096 & 9.57059 & 0.00261 \\
2452967.73502 & 9.57141 & 0.00265 \\
2452967.73903 & 9.56982 & 0.00271 \\
2452967.74700 & 9.56763 & 0.00290 \\
2452967.75103 & 9.57121 & 0.00272 \\
2452967.75501 & 9.56270 & 0.00271 \\
2452967.75895 & 9.57275 & 0.00276 \\
2452970.56341 & 9.57195 & 0.00254 \\
2452970.56732 & 9.57540 & 0.00262 \\
2452970.57131 & 9.57210 & 0.00270 \\
2452970.57542 & 9.57113 & 0.00265 \\
2452970.57941 & 9.57428 & 0.00261 \\
2452970.58338 & 9.56973 & 0.00252 \\
2452970.58736 & 9.56812 & 0.00258 \\
2452970.59147 & 9.56530 & 0.00260 \\
2452970.59540 & 9.57421 & 0.00287 \\
2452970.59935 & 9.57317 & 0.00253 \\
2452970.60333 & 9.56930 & 0.00256 \\
2452970.61527 & 9.56782 & 0.00272 \\
2452970.61922 & 9.56938 & 0.00262 \\
2452970.62329 & 9.57144 & 0.00250 \\
2452970.62727 & 9.56429 & 0.00259 \\
2452970.63120 & 9.56631 & 0.00279 \\
2452970.63514 & 9.56879 & 0.00269 \\
2452970.63922 & 9.56934 & 0.00268 \\
2452970.64320 & 9.57589 & 0.00258 \\
2452970.64716 & 9.56819 & 0.00252 \\
2452970.65107 & 9.57317 & 0.00261 \\
2452970.65514 & 9.56773 & 0.00290 \\
2452970.65905 & 9.56800 & 0.00263 \\
2452970.66298 & 9.56992 & 0.00269 \\
2452970.66691 & 9.56231 & 0.00255 \\
2452970.67097 & 9.57154 & 0.00258 \\
2452970.67488 & 9.57679 & 0.00263 \\
2452970.68282 & 9.57301 & 0.00255 \\
2452970.68696 & 9.56442 & 0.00264 \\
2452970.69088 & 9.57447 & 0.00264 \\
2452970.69477 & 9.56689 & 0.00268 \\
2452970.69874 & 9.57582 & 0.00262 \\
2452970.70679 & 9.57009 & 0.00265 \\
2452970.71467 & 9.57061 & 0.00281 \\
2452970.71879 & 9.56939 & 0.00247 \\
2452970.72277 & 9.56878 & 0.00260 \\
2452970.72676 & 9.57134 & 0.00282 \\
2452970.73070 & 9.57207 & 0.00254 \\
2452970.73873 & 9.56846 & 0.00268 \\
2452970.74271 & 9.57745 & 0.00257 \\
2452970.74669 & 9.57043 & 0.00279 \\
2452970.75075 & 9.56814 & 0.00270 \\
2452971.58538 & 9.56907 & 0.00249 \\
2452971.58931 & 9.57766 & 0.00266 \\
2452971.59330 & 9.56603 & 0.00253 \\
2452971.59740 & 9.57449 & 0.00257 \\
2452971.60132 & 9.57276 & 0.00257 \\
2452971.60523 & 9.56760 & 0.00252 \\
2452971.60914 & 9.57067 & 0.00261 \\
2452971.61321 & 9.56791 & 0.00898 \\
2452971.61712 & 9.56892 & 0.00254 \\
2452971.62110 & 9.56970 & 0.00254 \\
2452971.62511 & 9.56959 & 0.00250 \\
2452971.62923 & 9.56451 & 0.00242 \\
2452971.63315 & 9.57427 & 0.00269 \\
2452971.63708 & 9.57472 & 0.00254 \\
2452971.64100 & 9.57092 & 0.00258 \\
2452971.64506 & 9.56491 & 0.00241 \\
2452971.64899 & 9.57163 & 0.00241 \\
2452971.65291 & 9.56635 & 0.00257 \\
2452971.65685 & 9.56933 & 0.00268 \\
2452971.66095 & 9.57437 & 0.00262 \\
2452971.66487 & 9.56938 & 0.00242 \\
2452971.66880 & 9.57398 & 0.00252 \\
2452971.67274 & 9.56732 & 0.00242 \\
2452971.67681 & 9.56551 & 0.00258 \\
2452971.68080 & 9.57574 & 0.00267 \\
2452971.68479 & 9.57052 & 0.00265 \\
2452971.68878 & 9.57022 & 0.00261 \\
2452971.69285 & 9.57001 & 0.00251 \\
2452971.69677 & 9.56617 & 0.00242 \\
2452971.70075 & 9.57637 & 0.00236 \\
2452971.70467 & 9.57658 & 0.00241 \\
2452971.70879 & 9.57586 & 0.00248 \\
2452971.71270 & 9.57896 & 0.00256 \\
2452971.71668 & 9.57435 & 0.00258 \\
2452971.72060 & 9.57394 & 0.00683 \\
2452971.72464 & 9.57677 & 0.00662 \\
2452971.73262 & 9.57792 & 0.00256 \\
2452971.73654 & 9.56941 & 0.00258 \\
2452971.74054 & 9.56465 & 0.00251 \\
2452971.74447 & 9.57144 & 0.00270 \\
2452971.74839 & 9.56415 & 0.00268 \\
2452971.75231 & 9.57632 & 0.00251 \\
2452972.65783 & 9.56032 & 0.00291 \\
2452972.66176 & 9.57175 & 0.00294 \\
2452972.66570 & 9.57328 & 0.00326 \\
2452972.66967 & 9.57296 & 0.00298 \\
2452972.67768 & 9.57157 & 0.00318 \\
2452972.68165 & 9.58045 & 0.00411 \\
2452972.68562 & 9.57544 & 0.00302 \\
2452972.68964 & 9.57445 & 0.00302 \\
2452972.69362 & 9.55719 & 0.00283 \\
2452972.70560 & 9.56708 & 0.00357 \\
2452972.70952 & 9.56943 & 0.00328 \\
2452972.71345 & 9.57937 & 0.00358 \\
2452972.71736 & 9.56354 & 0.00370 \\
2452972.72139 & 9.56286 & 0.00314 \\
2452972.72927 & 9.56847 & 0.00445 \\
2452972.73324 & 9.56885 & 0.00379 \\
2452972.73730 & 9.57306 & 0.00697 \\
2452972.74126 & 9.57163 & 0.01249 \\
2452972.74521 & 9.58551 & 0.00669 \\
2452974.56287 & 9.57095 & 0.00285 \\
2452974.56680 & 9.56605 & 0.00289 \\
2452974.57076 & 9.57366 & 0.00329 \\
2452974.57481 & 9.57462 & 0.00284 \\
2452974.57872 & 9.57336 & 0.00294 \\
2452974.58270 & 9.57596 & 0.00272 \\
2452974.58669 & 9.57570 & 0.00321 \\
2452974.59080 & 9.55728 & 0.00270 \\
2452974.59478 & 9.56787 & 0.00274 \\
2452974.59869 & 9.57318 & 0.00303 \\
2452974.60261 & 9.57671 & 0.00295 \\
2452974.60667 & 9.56129 & 0.00314 \\
2452974.61066 & 9.57497 & 0.00291 \\
2452974.61458 & 9.57025 & 0.00287 \\
2452974.61851 & 9.57215 & 0.00257 \\
2452974.62263 & 9.57182 & 0.00292 \\
2452974.62656 & 9.57807 & 0.00262 \\
2452974.63055 & 9.57066 & 0.00280 \\
2452974.63445 & 9.57918 & 0.00297 \\
2452974.63848 & 9.58210 & 0.00283 \\
2452974.64240 & 9.57713 & 0.00284 \\
2452974.65030 & 9.56477 & 0.00272 \\
2452974.65441 & 9.57151 & 0.00334 \\
2452974.65832 & 9.57097 & 0.00299 \\
2452974.66226 & 9.56790 & 0.00290 \\
2452974.67031 & 9.57578 & 0.00281 \\
2452974.67422 & 9.56923 & 0.00295 \\
2452974.67813 & 9.56646 & 0.00301 \\
2452974.68612 & 9.57085 & 0.00269 \\
2452974.69010 & 9.56863 & 0.00304 \\
2452974.69398 & 9.56888 & 0.00272 \\
2452974.70200 & 9.57198 & 0.00298 \\
2452974.70598 & 9.56736 & 0.00307 \\
2452974.70991 & 9.57691 & 0.00306 \\
2452974.71389 & 9.57603 & 0.00310 \\
2452974.71798 & 9.57464 & 0.00301 \\
2452974.72192 & 9.57433 & 0.00290 \\
2452974.72979 & 9.57188 & 0.00282 \\
2452974.73773 & 9.57008 & 0.00289 \\
2452975.56281 & 9.56356 & 0.00437 \\
2452975.56678 & 9.58088 & 0.00353 \\
2452975.57071 & 9.56804 & 0.00316 \\
2452975.57480 & 9.56932 & 0.00435 \\
2452975.57876 & 9.56783 & 0.00486 \\
2452975.58266 & 9.57449 & 0.00404 \\
2452975.58661 & 9.56943 & 0.00438 \\
2452975.59453 & 9.56615 & 0.00533 \\
2452975.59842 & 9.56393 & 0.00489 \\
2452975.60237 & 9.56758 & 0.00457 \\
2452975.60640 & 9.57162 & 0.00772 \\
2452975.61035 & 9.55389 & 0.00561 \\
2452975.61424 & 9.57526 & 0.00590 \\
2452975.61813 & 9.57853 & 0.00557 \\
2452975.62216 & 9.58145 & 0.00469 \\
2452975.62606 & 9.56602 & 0.00510 \\
2452975.63002 & 9.58097 & 0.00692 \\
2452975.63396 & 9.57133 & 0.00495 \\
2452975.63800 & 9.57268 & 0.00406 \\
2452975.64189 & 9.57503 & 0.00444 \\
2452975.64580 & 9.56844 & 0.00387 \\
2452975.64970 & 9.57724 & 0.00443 \\
2452975.65379 & 9.56956 & 0.00542 \\
2452975.65769 & 9.57676 & 0.00579 \\
2452975.72832 & 9.56370 & 0.00886 \\
2452975.73237 & 9.57439 & 0.01056 \\
2452977.55870 & 9.56085 & 0.00748 \\
2452977.56261 & 9.57702 & 0.00518 \\
2452977.57827 & 9.57826 & 0.00429 \\
2452977.58223 & 9.57624 & 0.00306 \\
2452977.58620 & 9.57448 & 0.00311 \\
2452977.59032 & 9.56842 & 0.00268 \\
2452977.59429 & 9.56556 & 0.00293 \\
2452977.59821 & 9.57413 & 0.00310 \\
2452977.60218 & 9.57730 & 0.00292 \\
2452977.60623 & 9.56403 & 0.00291 \\
2452977.61015 & 9.56983 & 0.00309 \\
2452977.61413 & 9.56910 & 0.00319 \\
2452977.61806 & 9.57611 & 0.00299 \\
2452977.62219 & 9.57626 & 0.00298 \\
2452977.62618 & 9.56999 & 0.00277 \\
2452977.63009 & 9.57459 & 0.00292 \\
2452977.63401 & 9.57073 & 0.00290 \\
2452977.63804 & 9.56362 & 0.00520 \\
2452977.64192 & 9.57980 & 0.00609 \\
2452977.64581 & 9.54929 & 0.00645 \\
2452977.64970 & 9.57236 & 0.00419 \\
2452977.65763 & 9.56404 & 0.00399 \\
2452977.66549 & 9.57064 & 0.00576 \\
2452977.66950 & 9.56975 & 0.00363 \\
2452977.67349 & 9.57242 & 0.00318 \\
2452977.67742 & 9.56727 & 0.00311 \\
2452977.68134 & 9.56941 & 0.00317 \\
2452977.68546 & 9.57305 & 0.00304 \\
2452977.69341 & 9.57252 & 0.00276 \\
2452977.69733 & 9.58134 & 0.00287 \\
2452977.70139 & 9.57069 & 0.00317 \\
2452977.70531 & 9.57220 & 0.00266 \\
2452977.70923 & 9.56811 & 0.00308 \\
2452977.71320 & 9.57245 & 0.00314 \\
2452977.72124 & 9.56561 & 0.00293 \\
2452977.72517 & 9.57509 & 0.00307 \\
2452977.72908 & 9.56632 & 0.00327 \\
2452977.73312 & 9.56378 & 0.00338 \\
2452978.55862 & 9.57428 & 0.00323 \\
2452978.56259 & 9.58077 & 0.00277 \\
2452978.56650 & 9.56693 & 0.00267 \\
2452978.57031 & 9.57626 & 0.00297 \\
2452978.57422 & 9.56924 & 0.00315 \\
2452978.57814 & 9.57578 & 0.00259 \\
2452978.58195 & 9.56953 & 0.00278 \\
2452978.58587 & 9.57139 & 0.00299 \\
2452978.58977 & 9.56200 & 0.00266 \\
2452978.59358 & 9.56535 & 0.00267 \\
2452978.59755 & 9.56851 & 0.00267 \\
2452978.60148 & 9.57122 & 0.00286 \\
2452978.60529 & 9.58035 & 0.00300 \\
2452978.60925 & 9.56340 & 0.00281 \\
2452978.61322 & 9.58237 & 0.00309 \\
2452978.61705 & 9.56993 & 0.00276 \\
2452978.62094 & 9.55995 & 0.00274 \\
2452978.62870 & 9.57227 & 0.00295 \\
2452978.63261 & 9.57385 & 0.00283 \\
2452978.63652 & 9.55642 & 0.00294 \\
2452978.64033 & 9.57004 & 0.00279 \\
2452978.64423 & 9.57516 & 0.00284 \\
2452978.64821 & 9.56248 & 0.00286 \\
2452978.65202 & 9.57610 & 0.00319 \\
2452978.65593 & 9.56821 & 0.00291 \\
2452978.65984 & 9.57083 & 0.00276 \\
2452978.66757 & 9.56859 & 0.00292 \\
2452978.67148 & 9.57131 & 0.00283 \\
2452978.67529 & 9.57050 & 0.00325 \\
2452978.69091 & 9.57180 & 0.00294 \\
2452978.69871 & 9.56621 & 0.00312 \\
2452978.70262 & 9.57533 & 0.00296 \\
2452978.71832 & 9.58955 & 0.00280 \\
2452978.72211 & 9.57080 & 0.00332 \\
2452978.72600 & 9.57146 & 0.00309 \\
2452978.72991 & 9.57186 & 0.00323 \\
2452979.56262 & 9.56677 & 0.00361 \\
2452979.56651 & 9.56145 & 0.00302 \\
2452979.57042 & 9.56882 & 0.00341 \\
2452979.57452 & 9.57201 & 0.00350 \\
2452979.57843 & 9.57450 & 0.00309 \\
2452979.58234 & 9.56933 & 0.00342 \\
2452979.58626 & 9.57014 & 0.00401 \\
2452979.59035 & 9.57441 & 0.00352 \\
2452979.59432 & 9.56392 & 0.00333 \\
2452979.59824 & 9.56535 & 0.00379 \\
2452979.60216 & 9.57223 & 0.00329 \\
2452979.60620 & 9.56500 & 0.00362 \\
2452979.61015 & 9.55398 & 0.00654 \\
2452979.62203 & 9.54488 & 0.01124 \\
2452979.62591 & 9.56078 & 0.00578 \\
2452979.62985 & 9.57690 & 0.00458 \\
2452979.64160 & 9.56760 & 0.00852 \\
2452979.64548 & 9.56946 & 0.00448 \\
2452979.64945 & 9.57520 & 0.00443 \\
2452979.66133 & 9.56011 & 0.00409 \\
2452979.66528 & 9.55929 & 0.00443 \\
2452979.66932 & 9.56490 & 0.00382 \\
2452979.67330 & 9.57164 & 0.00354 \\
2452979.68919 & 9.57001 & 0.00406 \\
2452979.69310 & 9.58454 & 0.00328 \\
2452979.69707 & 9.56151 & 0.00316 \\
2452979.70110 & 9.56475 & 0.00321 \\
2452979.71693 & 9.57302 & 0.00310 \\
2452979.72089 & 9.57339 & 0.00295 \\
2452979.72481 & 9.56779 & 0.00309 \\
2452979.72871 & 9.57210 & 0.00291 \\
2452979.73272 & 9.56933 & 0.00347 \\
2452980.56269 & 9.56929 & 0.00339 \\
2452980.56660 & 9.57130 & 0.00293 \\
2452980.57051 & 9.56666 & 0.00301 \\
2452980.57461 & 9.57396 & 0.00286 \\
2452980.57857 & 9.56943 & 0.00282 \\
2452980.58249 & 9.57737 & 0.00300 \\
2452980.58641 & 9.56727 & 0.00306 \\
2452980.59046 & 9.57963 & 0.00299 \\
2452980.59433 & 9.56978 & 0.00288 \\
2452980.59829 & 9.56885 & 0.00273 \\
2452980.60220 & 9.57345 & 0.00326 \\
2452980.60632 & 9.57066 & 0.00282 \\
2452980.61023 & 9.57073 & 0.00270 \\
2452980.61411 & 9.57289 & 0.00308 \\
2452980.61801 & 9.57611 & 0.00293 \\
2452980.62205 & 9.57940 & 0.00288 \\
2452980.62597 & 9.56981 & 0.00304 \\
2452980.62987 & 9.56521 & 0.00283 \\
2452980.63380 & 9.56655 & 0.00318 \\
2452980.63790 & 9.57082 & 0.00304 \\
2452980.64181 & 9.57058 & 0.00275 \\
2452980.64572 & 9.56690 & 0.00305 \\
2452980.64963 & 9.56749 & 0.00309 \\
2452980.65374 & 9.57106 & 0.00306 \\
2452980.65765 & 9.57418 & 0.00302 \\
2452980.66164 & 9.57365 & 0.00323 \\
2452980.66955 & 9.57259 & 0.00324 \\
2452980.67345 & 9.57612 & 0.00274 \\
2452980.67742 & 9.56956 & 0.00278 \\
2452980.68543 & 9.56979 & 0.00332 \\
2452980.68936 & 9.57264 & 0.00338 \\
2452980.69332 & 9.56796 & 0.00328 \\
2452980.69724 & 9.57196 & 0.00273 \\
2452980.70920 & 9.56766 & 0.00320 \\
2452980.71312 & 9.57141 & 0.00302 \\
2452980.71723 & 9.56545 & 0.00313 \\
2452980.72119 & 9.56755 & 0.00285 \\
2452981.55870 & 9.55602 & 0.00490 \\
2452981.56262 & 9.56734 & 0.00342 \\
2452981.56652 & 9.56825 & 0.00325 \\
2452981.57043 & 9.57700 & 0.00459 \\
2452981.57445 & 9.57802 & 0.00492 \\
2452981.59795 & 9.57083 & 0.00524 \\
2452981.60186 & 9.56077 & 0.00533 \\
2452981.60593 & 9.58324 & 0.00514 \\
2452981.60986 & 9.57415 & 0.00705 \\
2452981.61762 & 9.57380 & 0.00408 \\
2452981.62165 & 9.56953 & 0.00342 \\
2452981.62557 & 9.56961 & 0.00354 \\
2452981.62954 & 9.57390 & 0.00350 \\
2452981.63347 & 9.57347 & 0.00329 \\
2452981.63752 & 9.56748 & 0.00295 \\
2452981.64150 & 9.57456 & 0.00292 \\
2452981.64545 & 9.57130 & 0.00283 \\
2452981.64943 & 9.57440 & 0.00298 \\
2452981.65746 & 9.56378 & 0.00318 \\
2452981.66144 & 9.56813 & 0.00278 \\
2452981.66546 & 9.57435 & 0.00307 \\
2452981.66954 & 9.57827 & 0.00275 \\
2452981.67344 & 9.57350 & 0.00289 \\
2452981.68128 & 9.57284 & 0.00300 \\
2452981.68531 & 9.57500 & 0.00538 \\
2452981.68921 & 9.58263 & 0.00693 \\
2452981.69703 & 9.56349 & 0.00479 \\
2452981.70896 & 9.57401 & 0.00896 \\
2452983.58430 & 9.57464 & 0.00272 \\
2452983.62041 & 9.56562 & 0.00259 \\
2452983.62441 & 9.56777 & 0.00258 \\
2452983.62833 & 9.56334 & 0.00251 \\
2452983.63232 & 9.56662 & 0.00261 \\
2452983.63638 & 9.57074 & 0.00262 \\
2452983.64027 & 9.57020 & 0.00254 \\
2452983.64421 & 9.56249 & 0.00267 \\
2452983.64820 & 9.57289 & 0.00267 \\
2452983.65227 & 9.57183 & 0.00260 \\
2452983.65620 & 9.57037 & 0.00279 \\
2452983.66018 & 9.56923 & 0.00249 \\
2452983.66414 & 9.56692 & 0.00272 \\
2452983.66825 & 9.57210 & 0.00260 \\
2452983.67621 & 9.56518 & 0.00269 \\
2452983.68019 & 9.56788 & 0.00268 \\
2452983.68422 & 9.56635 & 0.00262 \\
2452983.68814 & 9.56972 & 0.00268 \\
2452983.69206 & 9.56323 & 0.00250 \\
2452983.70400 & 9.57455 & 0.00279 \\
2452983.70797 & 9.57115 & 0.00268 \\
2452983.71188 & 9.56618 & 0.00277 \\
2452983.71593 & 9.56540 & 0.00295 \\
2452983.71985 & 9.56219 & 0.00274 \\
2452984.59328 & 9.57330 & 0.00248 \\
2452984.59729 & 9.56896 & 0.00275 \\
2452984.60120 & 9.57445 & 0.00291 \\
2452984.60530 & 9.56717 & 0.00261 \\
2452984.60929 & 9.56488 & 0.00272 \\
2452984.61321 & 9.57513 & 0.00276 \\
2452984.61719 & 9.57507 & 0.00266 \\
2452984.62125 & 9.56959 & 0.00261 \\
2452984.62522 & 9.57376 & 0.00267 \\
2452984.62920 & 9.57101 & 0.00248 \\
2452984.63311 & 9.56824 & 0.00272 \\
2452984.63720 & 9.56889 & 0.00249 \\
2452984.64119 & 9.56166 & 0.00269 \\
2452984.64512 & 9.57090 & 0.00284 \\
2452984.64910 & 9.56813 & 0.00280 \\
2452984.65319 & 9.57477 & 0.00271 \\
2452984.65711 & 9.57157 & 0.00272 \\
2452984.66103 & 9.56690 & 0.00275 \\
2452984.66501 & 9.57736 & 0.00286 \\
2452984.67304 & 9.56895 & 0.00260 \\
2452984.67702 & 9.57237 & 0.00264 \\
2452984.68099 & 9.56650 & 0.00274 \\
2452984.68505 & 9.56821 & 0.00281 \\
2452984.68900 & 9.57253 & 0.00259 \\
2452984.70100 & 9.56893 & 0.00291 \\
2452984.70491 & 9.57084 & 0.00282 \\
2452984.70883 & 9.57621 & 0.00278 \\
2452984.71280 & 9.57001 & 0.00265 \\
2452986.55801 & 9.57206 & 0.00250 \\
2452986.56196 & 9.56957 & 0.00240 \\
2452986.56589 & 9.57001 & 0.00245 \\
2452986.56980 & 9.57755 & 0.00248 \\
2452986.57385 & 9.57553 & 0.00244 \\
2452986.57779 & 9.57294 & 0.00243 \\
2452986.58172 & 9.57162 & 0.00238 \\
2452986.58564 & 9.56299 & 0.00240 \\
2452986.58975 & 9.57080 & 0.00251 \\
2452986.59367 & 9.56885 & 0.00252 \\
2452986.59759 & 9.57038 & 0.00248 \\
2452986.60152 & 9.56973 & 0.00239 \\
2452986.60562 & 9.56966 & 0.00244 \\
2452986.60953 & 9.57331 & 0.00244 \\
2452986.61352 & 9.57070 & 0.00246 \\
2452986.61746 & 9.57467 & 0.00253 \\
2452986.62150 & 9.56941 & 0.00254 \\
2452986.62544 & 9.57980 & 0.00243 \\
2452986.62934 & 9.57293 & 0.00275 \\
2452986.63333 & 9.56945 & 0.00251 \\
2452986.63740 & 9.57390 & 0.00253 \\
2452986.64134 & 9.57297 & 0.00262 \\
2452986.64533 & 9.57633 & 0.00254 \\
2452986.64924 & 9.57597 & 0.00256 \\
2452986.65335 & 9.54325 & 0.00247 \\
2452986.65729 & 9.57537 & 0.00246 \\
2452986.66116 & 9.56701 & 0.00244 \\
2452986.66911 & 9.57332 & 0.00277 \\
2452986.67309 & 9.57596 & 0.00261 \\
2452986.67701 & 9.56994 & 0.00244 \\
2452986.68101 & 9.56867 & 0.00264 \\
2452986.68512 & 9.56960 & 0.00265 \\
2452986.69692 & 9.57084 & 0.00272 \\
2452986.70099 & 9.57882 & 0.00263 \\
2452986.70489 & 9.57574 & 0.00276 \\
2452986.70886 & 9.56787 & 0.00268 \\
2452987.56328 & 9.55602 & 0.00998 \\
2452987.56719 & 9.56320 & 0.00640 \\
2452987.57107 & 9.56206 & 0.00981 \\
2452987.57508 & 9.58748 & 0.00589 \\
2452987.57905 & 9.57141 & 0.00754 \\
2452987.58302 & 9.57509 & 0.00624 \\
2452987.58691 & 9.55590 & 0.00514 \\
2452987.59096 & 9.55789 & 0.00500 \\
2452987.59494 & 9.56372 & 0.00587 \\
2452987.59890 & 9.55585 & 0.00451 \\
2452987.60278 & 9.56772 & 0.00571 \\
2452987.60688 & 9.56033 & 0.00466 \\
2452987.61083 & 9.57810 & 0.00501 \\
2452987.61481 & 9.57141 & 0.00529 \\
2452987.61873 & 9.56327 & 0.00411 \\
2452987.62283 & 9.56880 & 0.00640 \\
2452987.62679 & 9.57030 & 0.00523 \\
2452987.63070 & 9.56932 & 0.00413 \\
2452987.63466 & 9.56818 & 0.00430 \\
2452987.63870 & 9.58436 & 0.00353 \\
2452987.64264 & 9.56056 & 0.00411 \\
2452987.64655 & 9.57262 & 0.00356 \\
2452987.65053 & 9.56404 & 0.00328 \\
2452987.65459 & 9.57089 & 0.00518 \\
2452987.65850 & 9.56283 & 0.00540 \\
2452987.66245 & 9.57029 & 0.00805 \\
2452987.67435 & 9.56021 & 0.00629 \\
2452987.67825 & 9.57085 & 0.00594 \\
2452987.68214 & 9.55221 & 0.00719 \\
2452987.69417 & 9.56594 & 0.00589 \\
2452987.69814 & 9.57550 & 0.00601 \\
2452987.70219 & 9.57413 & 0.00553 \\
2452988.56342 & 9.56557 & 0.00282 \\
2452988.56730 & 9.56603 & 0.00272 \\
2452988.57130 & 9.57516 & 0.00279 \\
2452988.57535 & 9.56743 & 0.00260 \\
2452988.57932 & 9.57473 & 0.00270 \\
2452988.58325 & 9.57821 & 0.00251 \\
2452988.67620 & 9.57306 & 0.00282 \\
2452988.69214 & 9.57749 & 0.00277 \\
2452988.69606 & 9.58287 & 0.00283 \\
2452988.69995 & 9.57954 & 0.00279 \\
2452988.70391 & 9.58185 & 0.00272 \\
2452989.58982 & 9.58535 & 0.00818 \\
2452989.59377 & 9.57685 & 0.00556 \\
2452989.59768 & 9.56579 & 0.00729 \\
2452989.60162 & 9.57724 & 0.00585 \\
2452989.60570 & 9.56011 & 0.00560 \\
2452989.60967 & 9.56411 & 0.00502 \\
2452989.61357 & 9.56233 & 0.00474 \\
2452989.61753 & 9.56828 & 0.00544 \\
2452989.62158 & 9.58153 & 0.00497 \\
2452989.62553 & 9.56032 & 0.00561 \\
2452989.62949 & 9.57624 & 0.00474 \\
2452989.63340 & 9.57070 & 0.00427 \\
2452989.63751 & 9.56141 & 0.00465 \\
2452989.64144 & 9.56305 & 0.00487 \\
2452989.64535 & 9.56478 & 0.00388 \\
2452989.64927 & 9.56277 & 0.00345 \\
2452989.66130 & 9.57185 & 0.00304 \\
2452989.66528 & 9.57937 & 0.00287 \\
2452989.66938 & 9.56902 & 0.00264 \\
2452989.67332 & 9.56782 & 0.00255 \\
2452989.67732 & 9.57544 & 0.00258 \\
2452989.68930 & 9.56745 & 0.00249 \\
2452989.69322 & 9.56809 & 0.00267 \\
2452989.69720 & 9.57209 & 0.00250 \\
2452989.70132 & 9.56637 & 0.00269 \\
2452990.55975 & 9.57576 & 0.00293 \\
2452990.56367 & 9.57049 & 0.00279 \\
2452990.56761 & 9.56673 & 0.00265 \\
2452990.57153 & 9.57163 & 0.00282 \\
2452990.57558 & 9.56977 & 0.00286 \\
2452990.57955 & 9.56593 & 0.00271 \\
2452990.58351 & 9.57286 & 0.00287 \\
2452990.58750 & 9.56947 & 0.00274 \\
2452990.59154 & 9.57486 & 0.00265 \\
2452990.59553 & 9.57293 & 0.00264 \\
2452990.59946 & 9.56292 & 0.00275 \\
2452990.60344 & 9.56694 & 0.00269 \\
2452990.60755 & 9.57455 & 0.00270 \\
2452990.61146 & 9.56936 & 0.00271 \\
2452990.61545 & 9.56952 & 0.00265 \\
2452990.61944 & 9.57146 & 0.00257 \\
2452990.62355 & 9.56475 & 0.00262 \\
2452990.62747 & 9.57688 & 0.00278 \\
2452990.63142 & 9.57281 & 0.00291 \\
2452990.63534 & 9.57155 & 0.00261 \\
2452990.63946 & 9.57635 & 0.00271 \\
2452990.64345 & 9.57061 & 0.00264 \\
2452990.64739 & 9.56743 & 0.00258 \\
2452990.65132 & 9.57367 & 0.00295 \\
2452990.65936 & 9.58198 & 0.00284 \\
2452990.66333 & 9.57314 & 0.00300 \\
2452990.66731 & 9.57908 & 0.00257 \\
2452990.67131 & 9.57225 & 0.00277 \\
2452990.68309 & 9.57219 & 0.00290 \\
2452990.68719 & 9.57076 & 0.00263 \\
2452990.69112 & 9.56838 & 0.00283 \\
2452990.69509 & 9.57102 & 0.00306 \\
2452991.56398 & 9.57285 & 0.00300 \\
2452991.56789 & 9.57224 & 0.00296 \\
2452991.57187 & 9.57126 & 0.00287 \\
2452991.57986 & 9.57427 & 0.00271 \\
2452991.58385 & 9.57162 & 0.00310 \\
2452991.58779 & 9.57069 & 0.00280 \\
2452991.59182 & 9.57434 & 0.00280 \\
2452991.59575 & 9.57229 & 0.00298 \\
2452991.59974 & 9.56823 & 0.00288 \\
2452991.60371 & 9.55980 & 0.00301 \\
2452991.60778 & 9.56592 & 0.00280 \\
2452991.61170 & 9.57936 & 0.00285 \\
2452991.61561 & 9.57129 & 0.00272 \\
2452991.61959 & 9.57692 & 0.00282 \\
2452991.62758 & 9.56619 & 0.00265 \\
2452991.63151 & 9.56957 & 0.00262 \\
2452991.63547 & 9.57007 & 0.00277 \\
2452991.63952 & 9.56871 & 0.00310 \\
2452991.64351 & 9.57090 & 0.00261 \\
2452991.64747 & 9.56907 & 0.00273 \\
2452991.65556 & 9.56592 & 0.00279 \\
2452991.65948 & 9.57015 & 0.00302 \\
2452991.66337 & 9.56397 & 0.00290 \\
2452991.66730 & 9.57294 & 0.00271 \\
2452991.67142 & 9.56535 & 0.00265 \\
2452991.68324 & 9.58222 & 0.00307 \\
2452991.68736 & 9.57472 & 0.00301 \\
2452991.69135 & 9.56586 & 0.00274 \\
2452995.56103 & 9.57640 & 0.00302 \\
2452995.56498 & 9.57294 & 0.00285 \\
2452995.56889 & 9.56827 & 0.00267 \\
2452995.57281 & 9.56631 & 0.00262 \\
2452995.57687 & 9.56468 & 0.00254 \\
2452995.58085 & 9.57306 & 0.00272 \\
2452995.58482 & 9.56679 & 0.00271 \\
2452995.58884 & 9.56395 & 0.00242 \\
2452995.59295 & 9.57585 & 0.00275 \\
2452995.59693 & 9.56612 & 0.00263 \\
2452995.60091 & 9.56763 & 0.00266 \\
2452995.60482 & 9.56797 & 0.00260 \\
2452995.60887 & 9.56704 & 0.00262 \\
2452995.61279 & 9.57394 & 0.00263 \\
2452995.61670 & 9.56976 & 0.00267 \\
2452995.62061 & 9.57370 & 0.00264 \\
2452995.62471 & 9.56625 & 0.00257 \\
2452995.62864 & 9.57333 & 0.00264 \\
2452995.63255 & 9.56553 & 0.00268 \\
2452995.63654 & 9.56590 & 0.00250 \\
2452995.64067 & 9.57114 & 0.00281 \\
2452995.64459 & 9.56687 & 0.00281 \\
2452995.64851 & 9.57634 & 0.00270 \\
2452995.65245 & 9.57334 & 0.00281 \\
2452995.65657 & 9.57539 & 0.00285 \\
2452995.66054 & 9.56511 & 0.00255 \\
2452995.66846 & 9.57124 & 0.00272 \\
2452995.67252 & 9.57634 & 0.00294 \\
2452995.67644 & 9.57298 & 0.00266 \\
2452995.68043 & 9.57612 & 0.00281 \\
2452995.68436 & 9.57039 & 0.00264 \\
2452996.59889 & 9.57510 & 0.00438 \\
2452996.60282 & 9.57710 & 0.00493 \\
2452996.62251 & 9.57255 & 0.00916 \\
2452996.62640 & 9.56994 & 0.00688 \\
2452996.64617 & 9.57688 & 0.00704 \\
2452996.65012 & 9.58420 & 0.01050 \\
2453001.59404 & 9.56389 & 0.00355 \\
2453001.60200 & 9.57436 & 0.00307 \\
2453001.60598 & 9.57158 & 0.00276 \\
2453001.61002 & 9.57414 & 0.00321 \\
2453001.61394 & 9.57115 & 0.00440 \\
2453001.61791 & 9.57064 & 0.00470 \\
2453001.62185 & 9.56509 & 0.00317 \\
2453001.62592 & 9.58223 & 0.00297 \\
2453001.62982 & 9.57519 & 0.00304 \\
2453001.63379 & 9.57458 & 0.00275 \\
2453001.63778 & 9.57009 & 0.00283 \\
2453001.64190 & 9.57517 & 0.00254 \\
2453001.64584 & 9.56375 & 0.00259 \\
2453001.65373 & 9.57601 & 0.00278 \\
2453001.65778 & 9.57904 & 0.00283 \\
2453001.66176 & 9.56723 & 0.00278 \\
2453001.66570 & 9.57183 & 0.00252 \\
2453002.56317 & 9.57446 & 0.00390 \\
2453002.57097 & 9.56605 & 0.00313 \\
2453002.57494 & 9.57903 & 0.00269 \\
2453002.57899 & 9.57242 & 0.00295 \\
2453002.58291 & 9.56532 & 0.00278 \\
2453002.58683 & 9.57122 & 0.00243 \\
2453002.59074 & 9.57135 & 0.00290 \\
2453002.59875 & 9.56735 & 0.00252 \\
2453002.60263 & 9.56787 & 0.00259 \\
2453002.60653 & 9.57441 & 0.00257 \\
2453002.61060 & 9.57368 & 0.00252 \\
2453002.61458 & 9.56921 & 0.00268 \\
2453002.61850 & 9.55979 & 0.00254 \\
2453002.62646 & 9.57120 & 0.00269 \\
2453002.63044 & 9.56932 & 0.00268 \\
2453002.63435 & 9.57441 & 0.00261 \\
2453002.63827 & 9.56586 & 0.00291 \\
2453002.64232 & 9.56824 & 0.00297 \\
2453002.65424 & 9.57085 & 0.00263 \\
2453002.65835 & 9.56797 & 0.00277 \\
2453002.66233 & 9.56594 & 0.00263 \\
2453009.57783 & 9.57510 & 0.00303 \\
2453009.58183 & 9.57338 & 0.00341 \\
2453009.58574 & 9.58157 & 0.00314 \\
2453009.58966 & 9.57277 & 0.00339 \\
2453009.59364 & 9.57783 & 0.00319 \\
2453009.59775 & 9.57696 & 0.00315 \\
2453009.60559 & 9.57240 & 0.00298 \\
2453009.60960 & 9.56973 & 0.00274 \\
2453009.61366 & 9.57318 & 0.00259 \\
2453009.61763 & 9.56196 & 0.00289 \\
2453009.62959 & 9.57568 & 0.00266 \\
2453009.63747 & 9.57292 & 0.00322 \\
2453009.64135 & 9.56579 & 0.00289 \\
2453009.64541 & 9.57027 & 0.00265 \\
2453011.57089 & 9.56685 & 0.00286 \\
2453011.57483 & 9.57933 & 0.00283 \\
2453011.57873 & 9.56879 & 0.00296 \\
2453011.58265 & 9.57163 & 0.00275 \\
2453011.58675 & 9.57390 & 0.00270 \\
2453011.59073 & 9.57608 & 0.00296 \\
2453011.59467 & 9.56943 & 0.00297 \\
2453011.59859 & 9.56904 & 0.00292 \\
2453011.60269 & 9.57446 & 0.00291 \\
2453011.60661 & 9.57290 & 0.00294 \\
2453011.61057 & 9.57509 & 0.00284 \\
2453011.61455 & 9.57121 & 0.00279 \\
2453011.62655 & 9.56905 & 0.00268 \\
2453011.63046 & 9.57199 & 0.00309 \\
2453011.63452 & 9.57398 & 0.00281 \\
2453011.63840 & 9.57595 & 0.00301 \\
2453014.61004 & 9.56227 & 0.00282 \\
2453014.61795 & 9.57818 & 0.00325 \\
2453014.62187 & 9.56823 & 0.00281 \\
2453014.62600 & 9.56735 & 0.00281 \\
2453014.62993 & 9.56271 & 0.00310 \\
2453014.63385 & 9.57583 & 0.00302 \\
2453017.56837 & 9.56501 & 0.00297 \\
2453017.58021 & 9.57629 & 0.00279 \\
2453017.58425 & 9.57464 & 0.00289 \\
2453017.58817 & 9.57000 & 0.00266 \\
2453017.59215 & 9.57483 & 0.00258 \\
2453017.59608 & 9.57167 & 0.00272 \\
2453017.60013 & 9.56676 & 0.00264 \\
2453017.61199 & 9.57587 & 0.00291 \\
2453017.61605 & 9.56601 & 0.00274 \\
2453017.61996 & 9.57296 & 0.00282 \\
2453017.62394 & 9.57320 & 0.00279 \\
2453022.57197 & 9.57859 & 0.00287 \\
2453022.57597 & 9.57329 & 0.00261 \\
2453022.57989 & 9.58000 & 0.00274 \\
2453022.58388 & 9.56561 & 0.00265 \\
2453022.59584 & 9.57295 & 0.00281 \\
2453022.59977 & 9.58347 & 0.00253 \\
2453022.60382 & 9.57972 & 0.00284 \\
2453022.60779 & 9.58149 & 0.00267 \\
2453022.61172 & 9.57892 & 0.00251 \\
2453023.57251 & 9.57236 & 0.00271 \\
2453023.57652 & 9.56520 & 0.00257 \\
2453023.58049 & 9.56168 & 0.00253 \\
2453023.58844 & 9.56602 & 0.00266 \\
2453023.59634 & 9.57041 & 0.00264 \\
2453023.60028 & 9.57383 & 0.00280 \\
2453023.60441 & 9.56924 & 0.00265 \\
2453023.61228 & 9.57580 & 0.00262 \\
2453031.57660 & 9.56694 & 0.00596 \\
2453031.58054 & 9.56642 & 0.00276 \\
2453031.58453 & 9.56588 & 0.00285 \\
2453032.57718 & 9.57214 & 0.00310 \\
2453032.58505 & 9.57951 & 0.00776 \\
2453033.57731 & 9.56308 & 0.00363 \\
2453034.57793 & 9.56243 & 0.00339 \\
2453035.57840 & 9.56511 & 0.00327 \\
2452926.58193 & 9.57148 & 0.00262 \\
2452926.58588 & 9.56873 & 0.00257 \\
2452926.58983 & 9.56271 & 0.00252 \\
2452926.59377 & 9.56223 & 0.00236 \\
2452926.59785 & 9.56657 & 0.00250 \\
2452926.60178 & 9.57448 & 0.00253 \\
2452926.60572 & 9.57865 & 0.00252 \\
2452926.60965 & 9.56274 & 0.00250 \\
2452926.61372 & 9.57251 & 0.00249 \\
2452926.61767 & 9.57040 & 0.00262 \\
2452926.62550 & 9.56825 & 0.00247 \\
2452926.62956 & 9.56493 & 0.00257 \\
2452926.63349 & 9.57211 & 0.00248 \\
2452926.63743 & 9.57398 & 0.00268 \\
2452926.64137 & 9.56999 & 0.00254 \\
2452978.56167 & 9.57570 & 0.00268 \\
2452978.57312 & 9.57307 & 0.00280 \\
2452978.58840 & 9.56980 & 0.00263 \\
2452978.59216 & 9.58063 & 0.00261 \\
2452978.59989 & 9.57761 & 0.00260 \\
2452978.60365 & 9.57073 & 0.00252 \\
2452978.60753 & 9.57705 & 0.00274 \\
2452978.61140 & 9.57180 & 0.00257 \\
2452978.61517 & 9.56691 & 0.00262 \\
2452978.61904 & 9.56861 & 0.00254 \\
2452978.62292 & 9.56057 & 0.00261 \\
2452978.62668 & 9.57287 & 0.00255 \\
2452978.63056 & 9.56526 & 0.00261 \\
2452978.63445 & 9.58316 & 0.00268 \\
2452978.63821 & 9.57370 & 0.00248 \\
2452978.64211 & 9.56990 & 0.00260 \\
2452978.64598 & 9.56106 & 0.00266 \\
2452978.64975 & 9.57820 & 0.00271 \\
2452978.65362 & 9.57729 & 0.00263 \\
2452978.65750 & 9.55931 & 0.00258 \\
2452978.66126 & 9.57314 & 0.00261 \\
2452978.66513 & 9.57078 & 0.00259 \\
2452978.66901 & 9.57477 & 0.00269 \\
2452978.67277 & 9.57242 & 0.00261 \\
2452978.67664 & 9.56772 & 0.00259 \\
2452978.68428 & 9.57049 & 0.00262 \\
2452978.68816 & 9.57138 & 0.00272 \\
2452978.69203 & 9.56930 & 0.00243 \\
2452978.69965 & 9.56455 & 0.00285 \\
2452978.70351 & 9.58148 & 0.00270 \\
2452978.70727 & 9.56738 & 0.00272 \\
2452978.71115 & 9.56743 & 0.00267 \\
2452978.71502 & 9.55412 & 0.00274 \\
2452978.71878 & 9.56854 & 0.00267 \\
2452978.72265 & 9.57121 & 0.00270 \\
2452978.72651 & 9.56508 & 0.00265 \\
2452978.73027 & 9.56500 & 0.00270 \\
2452978.73413 & 9.56545 & 0.00283 \\
2452978.73800 & 9.58098 & 0.00283 \\
2452918.63027 & 9.57571 & 0.00260 \\
2452918.63430 & 9.57203 & 0.00277 \\
2452918.63834 & 9.57039 & 0.00253 \\
2452918.64237 & 9.57130 & 0.00265 \\
2452918.64658 & 9.56390 & 0.00277 \\
2452918.65062 & 9.57178 & 0.00265 \\
2452918.65467 & 9.56695 & 0.00429 \\
2452918.65868 & 9.57593 & 0.00388 \\
2452918.66270 & 9.57811 & 0.00335 \\
2452918.66662 & 9.57044 & 0.00286 \\
2452918.67055 & 9.57547 & 0.00266 \\
2452918.67448 & 9.56750 & 0.00264 \\
2452918.67856 & 9.57006 & 0.00251 \\
2452918.68248 & 9.57018 & 0.00270 \\
2452918.68641 & 9.56464 & 0.00250 \\
2452918.69035 & 9.57529 & 0.00257 \\
2452918.69443 & 9.57440 & 0.00295 \\
2452918.69835 & 9.55838 & 0.00306 \\
2452918.70228 & 9.56429 & 0.00273 \\
2452918.70622 & 9.56377 & 0.00278 \\
2452918.71027 & 9.56619 & 0.00264 \\
2452918.71422 & 9.57491 & 0.00274 \\
2452918.71815 & 9.57260 & 0.00254 \\
2452918.72208 & 9.57308 & 0.00264 \\
2452918.72613 & 9.56891 & 0.00272 \\
2452918.73007 & 9.57255 & 0.00263 \\
2452918.73400 & 9.56223 & 0.00276 \\
2452918.73791 & 9.56419 & 0.00270 \\
2452918.74198 & 9.56068 & 0.00273 \\
2452918.74591 & 9.57891 & 0.00287 \\
2452918.74985 & 9.57379 & 0.00265 \\
2452918.75378 & 9.56962 & 0.00306 \\
2452918.75783 & 9.58119 & 0.00267 \\
2452918.76175 & 9.56710 & 0.00270 \\
2452918.76569 & 9.57379 & 0.00268 \\
2452918.76962 & 9.57153 & 0.00267 \\
2452918.77370 & 9.57714 & 0.00258 \\
2452918.77763 & 9.57188 & 0.00253 \\
2452918.78158 & 9.56481 & 0.00260 \\
2452918.78553 & 9.57440 & 0.00252 \\
2452918.78961 & 9.56255 & 0.00257 \\
2452918.79354 & 9.56971 & 0.00268 \\
2452918.79748 & 9.56381 & 0.00271 \\
2452918.80548 & 9.57057 & 0.00256 \\
2452918.80941 & 9.57437 & 0.00271 \\
2452918.81335 & 9.57781 & 0.00266 \\
2452918.81727 & 9.56938 & 0.00256 \\
2452918.82134 & 9.57478 & 0.00269 \\
2452918.82526 & 9.55862 & 0.00257 \\
2452918.82921 & 9.57004 & 0.00261 \\
2452918.83312 & 9.56400 & 0.00261 \\
2452918.83719 & 9.57430 & 0.00264 \\
2452918.84114 & 9.55959 & 0.00257 \\
2452918.84508 & 9.57425 & 0.00255 \\
2452918.84903 & 9.58603 & 0.00262 \\
2452918.85310 & 9.56845 & 0.00252 \\
2452918.85705 & 9.56902 & 0.00249 \\
2452918.86101 & 9.57088 & 0.00268 \\
2452918.86494 & 9.57209 & 0.00263 \\
2452918.86901 & 9.58661 & 0.00283 \\
2452918.87292 & 9.56137 & 0.00280 \\
2452918.87685 & 9.57143 & 0.00263 \\
2452918.88078 & 9.57941 & 0.00268 \\
2452918.88486 & 9.56383 & 0.00263 \\
2452918.88880 & 9.56968 & 0.00268 \\
2452925.59176 & 9.57919 & 0.00283 \\
2452925.59570 & 9.56833 & 0.00260 \\
2452925.59964 & 9.57087 & 0.00293 \\
2452925.60357 & 9.56757 & 0.00248 \\
2452925.60763 & 9.56501 & 0.00269 \\
2452925.61159 & 9.57175 & 0.00264 \\
2452925.61552 & 9.57527 & 0.00273 \\
2452925.61946 & 9.57425 & 0.00253 \\
2452925.62353 & 9.56373 & 0.00273 \\
2452925.62747 & 9.57254 & 0.00256 \\
2452925.63141 & 9.58418 & 0.00275 \\
2452925.63536 & 9.57064 & 0.00246 \\
2452925.63944 & 9.57073 & 0.00270 \\
2452925.64339 & 9.57489 & 0.00260 \\
2452925.64734 & 9.56956 & 0.00278 \\
2452925.65129 & 9.57199 & 0.00263 \\
2452925.65537 & 9.56050 & 0.00263 \\
2452925.65930 & 9.57775 & 0.00248 \\
2452925.66319 & 9.56693 & 0.00256 \\
2452925.66717 & 9.56933 & 0.00264 \\
2452925.67127 & 9.57622 & 0.00274 \\
2452925.67520 & 9.56899 & 0.00270 \\
2452925.67915 & 9.55605 & 0.00255 \\
2452925.68307 & 9.57135 & 0.00258 \\
2452925.68711 & 9.55997 & 0.00260 \\
2452925.69104 & 9.57702 & 0.00248 \\
2452925.69496 & 9.57272 & 0.00272 \\
2452925.69888 & 9.56965 & 0.00263 \\
2452925.70293 & 9.57087 & 0.00284 \\
2452925.70684 & 9.57608 & 0.00285 \\
2452925.71076 & 9.56108 & 0.00263 \\
2452925.71469 & 9.57193 & 0.00256 \\
2452925.71872 & 9.57642 & 0.00265 \\
2452925.72266 & 9.57730 & 0.00258 \\
2452925.72661 & 9.56333 & 0.00260 \\
2452925.73054 & 9.56424 & 0.00257 \\
2452925.73459 & 9.56298 & 0.00264 \\
2452925.73851 & 9.57400 & 0.00254 \\
2452925.74246 & 9.57206 & 0.00267 \\
2452925.74639 & 9.57494 & 0.00275 \\
2452925.75046 & 9.57033 & 0.00273 \\
2452925.75438 & 9.57437 & 0.00273 \\
2452925.75832 & 9.58204 & 0.00264 \\
2452925.76224 & 9.56734 & 0.00264 \\
2452925.76632 & 9.57529 & 0.00259 \\
2452925.77024 & 9.56725 & 0.00250 \\
2452925.77418 & 9.56955 & 0.00260 \\
2452925.77810 & 9.56672 & 0.00243 \\
2452925.78216 & 9.54598 & 0.00257 \\
2452925.78608 & 9.57206 & 0.00256 \\
2452925.79001 & 9.57671 & 0.00265 \\
2452925.79394 & 9.56999 & 0.00257 \\
2452925.79801 & 9.56977 & 0.00279 \\
2452925.80193 & 9.56966 & 0.00270 \\
2452925.80588 & 9.57391 & 0.00266 \\
2452925.80980 & 9.56602 & 0.00252 \\
2452925.81387 & 9.57301 & 0.00269 \\
2452925.81778 & 9.57648 & 0.00256 \\
2452925.82175 & 9.57593 & 0.00272 \\
2452925.82569 & 9.56872 & 0.00267 \\
2452925.82976 & 9.57254 & 0.00263 \\
2452925.83369 & 9.56771 & 0.00257 \\
2452925.83762 & 9.56592 & 0.00280 \\
2452925.84155 & 9.57141 & 0.00267 \\
2452925.84562 & 9.56927 & 0.00276 \\
2452925.84953 & 9.57234 & 0.00273 \\
2452925.85346 & 9.57424 & 0.00268 \\
2452925.85737 & 9.56837 & 0.00266 \\
2452925.86143 & 9.56576 & 0.00259 \\
2452925.86536 & 9.55982 & 0.00259 \\
2452925.86931 & 9.57210 & 0.00286 \\
2452925.87323 & 9.57302 & 0.00270 \\
2452952.83911 & 9.57283 & 0.00270 \\
2452952.84318 & 9.57112 & 0.00265 \\
2452952.84710 & 9.56868 & 0.00281 \\
2452952.85105 & 9.57008 & 0.00277 \\
2452952.85498 & 9.57477 & 0.00262 \\
2452952.85906 & 9.57203 & 0.00267 \\
2452952.86300 & 9.57258 & 0.00259 \\
2452952.86693 & 9.56393 & 0.00263 \\
2452952.87089 & 9.56619 & 0.00278 \\
2452952.87496 & 9.57522 & 0.00267 \\
2452952.87889 & 9.56344 & 0.00255 \\
2452952.88283 & 9.56592 & 0.00268 \\
2452952.88676 & 9.55793 & 0.00255 \\
2452952.89082 & 9.57018 & 0.00299 \\
2452952.89476 & 9.57287 & 0.00267 \\
2452952.89869 & 9.57314 & 0.00272 \\
2452953.69635 & 9.57326 & 0.00259 \\
2452953.70029 & 9.56672 & 0.00272 \\
2452953.70422 & 9.56588 & 0.00275 \\
2452953.70817 & 9.57162 & 0.00266 \\
2452953.71225 & 9.56914 & 0.00276 \\
2452953.71619 & 9.57050 & 0.00254 \\
2452953.72013 & 9.56329 & 0.00256 \\
2452953.72407 & 9.56690 & 0.00267 \\
2452953.72815 & 9.56852 & 0.00279 \\
2452953.73208 & 9.57295 & 0.00252 \\
2452953.73602 & 9.57339 & 0.00257 \\
2452953.73995 & 9.56717 & 0.00240 \\
2452953.74402 & 9.57690 & 0.00248 \\
2452953.74795 & 9.56323 & 0.00253 \\
2452953.75190 & 9.56832 & 0.00256 \\
2452953.75584 & 9.56528 & 0.00269 \\
2452953.75991 & 9.57106 & 0.00263 \\
2452953.76385 & 9.57061 & 0.00247 \\
2452953.76780 & 9.55913 & 0.00241 \\
2452953.77175 & 9.57433 & 0.00259 \\
2452953.77581 & 9.57031 & 0.00255 \\
2452953.77975 & 9.56044 & 0.00266 \\
2452953.78369 & 9.56848 & 0.00254 \\
2452953.78763 & 9.56359 & 0.00251 \\
2452953.79169 & 9.57254 & 0.00252 \\
2452953.79563 & 9.56671 & 0.00246 \\
2452953.79953 & 9.56465 & 0.00256 \\
2452953.80350 & 9.56852 & 0.00255 \\
2452953.80756 & 9.56761 & 0.00244 \\
2452953.81152 & 9.57344 & 0.00251 \\
2452953.81546 & 9.57109 & 0.00250 \\
2452953.81941 & 9.57059 & 0.00259 \\
2452953.82740 & 9.56532 & 0.00237 \\
2452953.83132 & 9.57148 & 0.00259 \\
2452953.83526 & 9.56972 & 0.00252 \\
2452953.83933 & 9.56106 & 0.00237 \\
2452953.84326 & 9.56636 & 0.00252 \\
2452953.84720 & 9.57086 & 0.00240 \\
2452953.85112 & 9.57117 & 0.00253 \\
2452953.85520 & 9.57046 & 0.00245 \\
2452953.85914 & 9.57158 & 0.00267 \\
2452953.86308 & 9.56926 & 0.00260 \\
2452953.86702 & 9.56740 & 0.00270 \\
2452953.87111 & 9.56737 & 0.00255 \\
2452953.87503 & 9.57447 & 0.00285 \\
2452953.87897 & 9.56530 & 0.00264 \\
2452953.88292 & 9.56772 & 0.00267 \\
2452953.88700 & 9.56986 & 0.00259 \\
2452953.89093 & 9.56712 & 0.00259 \\
2452953.89485 & 9.57196 & 0.00255 \\
2452954.69608 & 9.56347 & 0.00280 \\
2452954.70002 & 9.57589 & 0.00261 \\
2452954.70396 & 9.57752 & 0.00255 \\
2452954.70792 & 9.56196 & 0.00270 \\
2452954.71198 & 9.56708 & 0.00262 \\
2452954.71593 & 9.57674 & 0.00265 \\
2452954.71985 & 9.56618 & 0.00264 \\
2452954.72378 & 9.57335 & 0.00253 \\
2452954.72785 & 9.57359 & 0.00255 \\
2452954.73179 & 9.57334 & 0.00247 \\
2452954.73573 & 9.57362 & 0.00260 \\
2452954.73967 & 9.57087 & 0.00255 \\
2452954.74375 & 9.56643 & 0.00252 \\
2452954.74770 & 9.56901 & 0.00257 \\
2452954.75165 & 9.56987 & 0.00260 \\
2452954.75560 & 9.56756 & 0.00248 \\
2452954.75966 & 9.57053 & 0.00255 \\
2452954.76361 & 9.56706 & 0.00260 \\
2452954.76754 & 9.56736 & 0.00249 \\
2452954.77148 & 9.57061 & 0.00255 \\
2452954.77555 & 9.56620 & 0.00239 \\
2452954.77949 & 9.56413 & 0.00253 \\
2452954.78342 & 9.56638 & 0.00246 \\
2452954.78734 & 9.56573 & 0.00241 \\
2452954.79141 & 9.56726 & 0.00270 \\
2452954.79535 & 9.56516 & 0.00261 \\
2452954.79930 & 9.56568 & 0.00240 \\
2452954.80324 & 9.56972 & 0.00253 \\
2452954.80731 & 9.57722 & 0.00256 \\
2452954.81125 & 9.57961 & 0.00249 \\
2452954.81518 & 9.57997 & 0.00245 \\
2452954.81911 & 9.57976 & 0.00256 \\
2452954.82318 & 9.57588 & 0.00245 \\
2452954.82712 & 9.57908 & 0.00256 \\
2452954.83107 & 9.57268 & 0.00244 \\
2452954.83503 & 9.58170 & 0.00249 \\
2452954.83910 & 9.58112 & 0.00273 \\
2452954.84305 & 9.57233 & 0.00252 \\
2452954.84699 & 9.57809 & 0.00247 \\
2452954.85092 & 9.58174 & 0.00256 \\
2452954.85890 & 9.57793 & 0.00247 \\
2452954.86284 & 9.57558 & 0.00247 \\
2452954.86679 & 9.57867 & 0.00255 \\
2452954.87085 & 9.58069 & 0.00257 \\
2452954.87479 & 9.57257 & 0.00270 \\
2452954.87874 & 9.57980 & 0.00260 \\
2452954.88268 & 9.58228 & 0.00264 \\
2452954.88675 & 9.57626 & 0.00249 \\
2452954.89069 & 9.57488 & 0.00252 \\
2452954.89463 & 9.57833 & 0.00262 \\
2452954.89857 & 9.57878 & 0.00271 \\
2452954.90264 & 9.57602 & 0.00261 \\
2452954.91050 & 9.57110 & 0.00261 \\
2452954.91444 & 9.57859 & 0.00263 \\
2452954.91850 & 9.57996 & 0.00248 \\
2452954.92243 & 9.57663 & 0.00268 \\
2452954.92637 & 9.58027 & 0.00259 \\
2452955.69575 & 9.57685 & 0.00269 \\
2452955.69969 & 9.56593 & 0.00256 \\
2452955.70363 & 9.56735 & 0.00253 \\
2452955.70757 & 9.57501 & 0.00237 \\
2452955.71163 & 9.57482 & 0.00232 \\
2452955.71558 & 9.57505 & 0.00238 \\
2452955.71952 & 9.57826 & 0.00249 \\
2452955.72346 & 9.57461 & 0.00251 \\
2452955.72755 & 9.56777 & 0.00239 \\
2452955.73149 & 9.56566 & 0.00237 \\
2452955.73545 & 9.57332 & 0.00238 \\
2452955.73939 & 9.56426 & 0.00230 \\
2452955.74343 & 9.56329 & 0.00233 \\
2452955.74736 & 9.56831 & 0.00234 \\
2452955.75131 & 9.56804 & 0.00264 \\
2452955.75525 & 9.57098 & 0.00251 \\
2452955.75934 & 9.56709 & 0.00254 \\
2452955.76327 & 9.57384 & 0.00236 \\
2452955.76721 & 9.56834 & 0.00242 \\
2452955.77115 & 9.56655 & 0.00242 \\
2452955.77522 & 9.56979 & 0.00245 \\
2452955.77917 & 9.56714 & 0.00243 \\
2452955.78312 & 9.56815 & 0.00251 \\
2452955.78706 & 9.56705 & 0.00238 \\
2452955.79112 & 9.57334 & 0.00255 \\
2452955.79507 & 9.56792 & 0.00241 \\
2452955.79901 & 9.56600 & 0.00244 \\
2452955.80295 & 9.56790 & 0.00254 \\
2452955.80702 & 9.56783 & 0.00248 \\
2452955.81096 & 9.57142 & 0.00252 \\
2452955.81490 & 9.56913 & 0.00250 \\
2452955.81884 & 9.56910 & 0.00245 \\
2452955.82288 & 9.57515 & 0.00247 \\
2452955.82681 & 9.57048 & 0.00256 \\
2452955.83075 & 9.57332 & 0.00243 \\
2452955.83470 & 9.57039 & 0.00236 \\
2452955.83878 & 9.57289 & 0.00254 \\
2452955.84271 & 9.56554 & 0.00246 \\
2452955.84667 & 9.56341 & 0.00249 \\
2452955.85061 & 9.57491 & 0.00249 \\
2452955.85468 & 9.56716 & 0.00241 \\
2452955.85862 & 9.57317 & 0.00257 \\
2452955.86257 & 9.56881 & 0.00242 \\
2452955.86651 & 9.57122 & 0.00236 \\
2452955.87056 & 9.57278 & 0.00244 \\
2452955.87451 & 9.57419 & 0.00246 \\
2452955.87844 & 9.57110 & 0.00251 \\
2452955.88239 & 9.56669 & 0.00251 \\
2452955.88647 & 9.56902 & 0.00252 \\
2452955.89042 & 9.56901 & 0.00232 \\
2452955.89437 & 9.57094 & 0.00240 \\
2452955.89831 & 9.57763 & 0.00258 \\
2452955.90238 & 9.58158 & 0.00254 \\
2452955.90633 & 9.56824 & 0.00260 \\
2452955.91027 & 9.56467 & 0.00272 \\
2452955.91423 & 9.56820 & 0.00253 \\
2452955.91831 & 9.57271 & 0.00263 \\
2452955.92224 & 9.57127 & 0.00247 \\
2452956.71979 & 9.57359 & 0.00246 \\
2452956.72374 & 9.56893 & 0.00255 \\
2452956.72769 & 9.57182 & 0.00247 \\
2452956.73176 & 9.56971 & 0.00261 \\
2452956.73573 & 9.56619 & 0.00245 \\
2452956.73966 & 9.57088 & 0.00251 \\
2452956.74766 & 9.57210 & 0.00252 \\
2452956.75160 & 9.56929 & 0.00242 \\
2452956.75555 & 9.56962 & 0.00246 \\
2452956.75949 & 9.57603 & 0.00237 \\
2452956.76356 & 9.56699 & 0.00241 \\
2452956.76750 & 9.57552 & 0.00238 \\
2452956.77145 & 9.56988 & 0.00233 \\
2452956.77539 & 9.56890 & 0.00235 \\
2452956.77948 & 9.56836 & 0.00230 \\
2452956.78341 & 9.56553 & 0.00234 \\
2452956.78735 & 9.57042 & 0.00237 \\
2452956.79132 & 9.57710 & 0.00244 \\
2452956.79538 & 9.56961 & 0.00241 \\
2452956.79931 & 9.57286 & 0.00246 \\
2452956.80327 & 9.57180 & 0.00242 \\
2452956.80727 & 9.56721 & 0.00237 \\
2452958.69525 & 9.57082 & 0.00253 \\
2452958.69919 & 9.56563 & 0.00255 \\
2452958.70313 & 9.56702 & 0.00395 \\
2452958.70706 & 9.57547 & 0.00435 \\
2452958.71118 & 9.57426 & 0.00274 \\
2452958.71513 & 9.57615 & 0.00260 \\
2452958.71905 & 9.56879 & 0.00251 \\
2452958.72299 & 9.56982 & 0.00242 \\
2452958.72706 & 9.56626 & 0.00253 \\
2452958.73102 & 9.57028 & 0.00250 \\
2452958.73497 & 9.56821 & 0.00248 \\
2452958.73888 & 9.56481 & 0.00240 \\
2452958.74295 & 9.56951 & 0.00239 \\
2452958.74689 & 9.56382 & 0.00238 \\
2452958.75082 & 9.56557 & 0.00250 \\
2452958.75476 & 9.57216 & 0.00240 \\
2452958.75884 & 9.56444 & 0.00257 \\
2452958.76278 & 9.56917 & 0.00257 \\
2452958.76672 & 9.56390 & 0.00245 \\
2452958.77066 & 9.56382 & 0.00238 \\
2452958.77474 & 9.57236 & 0.00244 \\
2452958.77870 & 9.57321 & 0.00243 \\
2452958.78264 & 9.56668 & 0.00261 \\
2452958.78658 & 9.57560 & 0.00534 \\
2452958.79063 & 9.56462 & 0.00327 \\
2452958.79456 & 9.56165 & 0.00392 \\
2452958.79849 & 9.56953 & 0.00273 \\
2452958.80243 & 9.57237 & 0.00252 \\
2452958.80649 & 9.57332 & 0.00266 \\
2452958.81041 & 9.56573 & 0.00248 \\
2452958.81436 & 9.56049 & 0.00336 \\
2452958.81830 & 9.57374 & 0.00334 \\
2452958.82236 & 9.57701 & 0.00295 \\
2452958.82629 & 9.56966 & 0.00279 \\
2452958.83023 & 9.57170 & 0.00294 \\
2452958.83416 & 9.57392 & 0.00263 \\
2452958.83823 & 9.56529 & 0.00258 \\
2452958.84219 & 9.56414 & 0.00251 \\
2452958.84613 & 9.56508 & 0.00279 \\
2452958.85007 & 9.58374 & 0.00273 \\
2452958.85415 & 9.56094 & 0.00542 \\
2452958.85808 & 9.57382 & 0.00303 \\
2452958.86201 & 9.57489 & 0.00280 \\
2452958.86595 & 9.57562 & 0.00258 \\
2452958.87002 & 9.56182 & 0.00316 \\
2452958.87397 & 9.56330 & 0.00264 \\
2452958.87788 & 9.57004 & 0.00251 \\
2452958.88183 & 9.57638 & 0.00245 \\
2452958.88589 & 9.57222 & 0.00292 \\
2452958.88980 & 9.56627 & 0.00261 \\
2452958.89375 & 9.57891 & 0.00254 \\
2452958.89769 & 9.56550 & 0.00262 \\
2452961.69462 & 9.57249 & 0.00289 \\
2452961.69857 & 9.55861 & 0.00267 \\
2452961.70251 & 9.56981 & 0.00262 \\
2452961.70644 & 9.56880 & 0.00247 \\
2452961.71052 & 9.57712 & 0.00263 \\
2452961.71446 & 9.57404 & 0.00263 \\
2452961.71841 & 9.56730 & 0.00236 \\
2452961.72234 & 9.56695 & 0.00247 \\
2452961.72641 & 9.56906 & 0.00244 \\
2452961.73035 & 9.57012 & 0.00252 \\
2452961.73426 & 9.57423 & 0.00238 \\
2452961.73819 & 9.57075 & 0.00259 \\
2452961.74227 & 9.57582 & 0.00259 \\
2452961.74622 & 9.57429 & 0.00250 \\
2452961.75017 & 9.56937 & 0.00244 \\
2452961.75411 & 9.56934 & 0.00267 \\
2452961.75819 & 9.57093 & 0.00243 \\
2452961.76214 & 9.56542 & 0.00246 \\
2452961.76609 & 9.57669 & 0.00255 \\
2452961.77006 & 9.56872 & 0.00255 \\
2452961.77414 & 9.57161 & 0.00243 \\
2452961.77809 & 9.56767 & 0.00250 \\
2452961.78203 & 9.57130 & 0.00241 \\
2452961.78598 & 9.57269 & 0.00257 \\
2452961.79004 & 9.56947 & 0.00252 \\
2452961.79398 & 9.56274 & 0.00243 \\
2452961.79794 & 9.56330 & 0.00249 \\
2452961.80189 & 9.57256 & 0.00238 \\
2452961.80596 & 9.56706 & 0.00263 \\
2452961.80989 & 9.57324 & 0.00251 \\
2452961.81383 & 9.56752 & 0.00256 \\
2452961.81774 & 9.56505 & 0.00250 \\
2452961.82180 & 9.57226 & 0.00262 \\
2452961.82574 & 9.56921 & 0.00262 \\
2452961.82967 & 9.56661 & 0.00253 \\
2452961.83362 & 9.57757 & 0.00251 \\
2452961.83768 & 9.57155 & 0.00255 \\
2452961.84161 & 9.57251 & 0.00243 \\
2452961.84555 & 9.56781 & 0.00236 \\
2452961.84949 & 9.57783 & 0.00244 \\
2452961.85356 & 9.57234 & 0.00251 \\
2452961.85751 & 9.56821 & 0.00240 \\
2452961.86145 & 9.57554 & 0.00244 \\
2452961.86539 & 9.56844 & 0.00251 \\
2452961.86946 & 9.56483 & 0.00248 \\
2452961.87341 & 9.57116 & 0.00258 \\
2452961.87734 & 9.56737 & 0.00241 \\
2452961.88130 & 9.56241 & 0.00241 \\
2452961.88538 & 9.58013 & 0.00246 \\
2452961.88932 & 9.57221 & 0.00240 \\
2452961.89326 & 9.57017 & 0.00247 \\
2452961.89720 & 9.57127 & 0.00254 \\
2452961.90126 & 9.56551 & 0.00241 \\
2452961.90521 & 9.56984 & 0.00259 \\
2452961.90916 & 9.56826 & 0.00242 \\
2452962.69445 & 9.57427 & 0.00273 \\
2452962.69839 & 9.56950 & 0.00253 \\
2452962.70234 & 9.57106 & 0.00256 \\
2452962.70627 & 9.56610 & 0.00253 \\
2452962.71033 & 9.56940 & 0.00263 \\
2452962.71426 & 9.56740 & 0.00254 \\
2452962.71821 & 9.56639 & 0.00253 \\
2452962.72215 & 9.56902 & 0.00240 \\
2452962.72621 & 9.56758 & 0.00249 \\
2452962.73016 & 9.57150 & 0.00241 \\
2452962.73410 & 9.56812 & 0.00236 \\
2452962.73804 & 9.57064 & 0.00238 \\
2452962.74603 & 9.56909 & 0.00235 \\
2452962.74998 & 9.57027 & 0.00245 \\
2452962.75394 & 9.56811 & 0.00231 \\
2452962.75798 & 9.57029 & 0.00237 \\
2452962.76194 & 9.56923 & 0.00235 \\
2452962.76589 & 9.56308 & 0.00235 \\
2452962.76983 & 9.56980 & 0.00239 \\
2452962.77390 & 9.56326 & 0.00245 \\
2452962.77784 & 9.57570 & 0.00243 \\
2452962.78178 & 9.57030 & 0.00244 \\
2452962.78572 & 9.56590 & 0.00235 \\
2452962.78981 & 9.57180 & 0.00225 \\
2452962.79374 & 9.56969 & 0.00240 \\
2452962.79769 & 9.57162 & 0.00238 \\
2452962.80163 & 9.57217 & 0.00226 \\
2452962.80570 & 9.57461 & 0.00238 \\
2452962.80965 & 9.57396 & 0.00239 \\
2452962.81359 & 9.56981 & 0.00236 \\
2452962.81754 & 9.57065 & 0.00227 \\
2452962.82161 & 9.56832 & 0.00239 \\
2452962.82556 & 9.57098 & 0.00234 \\
2452962.82949 & 9.57126 & 0.00239 \\
2452962.83340 & 9.56768 & 0.00235 \\
2452962.83747 & 9.57191 & 0.00235 \\
2452962.84143 & 9.56766 & 0.00234 \\
2452962.84537 & 9.56349 & 0.00235 \\
2452962.84932 & 9.57217 & 0.00225 \\
2452962.85336 & 9.56909 & 0.00235 \\
2452962.85730 & 9.56884 & 0.00232 \\
2452962.86125 & 9.56698 & 0.00242 \\
2452962.86518 & 9.56928 & 0.00235 \\
2452962.86925 & 9.57319 & 0.00248 \\
2452962.87319 & 9.57238 & 0.00245 \\
2452962.87713 & 9.57524 & 0.00238 \\
2452962.88108 & 9.57096 & 0.00236 \\
2452962.88515 & 9.57952 & 0.00235 \\
2452962.88908 & 9.57442 & 0.00236 \\
2452962.89302 & 9.56963 & 0.00245 \\
2452962.89696 & 9.57004 & 0.00243 \\
2452962.90103 & 9.56676 & 0.00245 \\
2452962.90499 & 9.57740 & 0.00245 \\
2452963.69448 & 9.58287 & 0.00274 \\
2452963.69838 & 9.56552 & 0.00260 \\
2452963.70226 & 9.57533 & 0.00264 \\
2452963.70613 & 9.57704 & 0.00240 \\
2452963.71012 & 9.56860 & 0.00247 \\
2452963.71400 & 9.57155 & 0.00229 \\
2452963.71790 & 9.56568 & 0.00241 \\
2452963.72178 & 9.57312 & 0.00237 \\
2452963.72580 & 9.57437 & 0.00236 \\
2452963.72967 & 9.57534 & 0.00246 \\
2452963.73355 & 9.56994 & 0.00231 \\
2452963.73743 & 9.57038 & 0.00235 \\
2452963.74531 & 9.56777 & 0.00240 \\
2452963.74920 & 9.56588 & 0.00237 \\
2452963.75313 & 9.57257 & 0.00248 \\
2452963.75715 & 9.56853 & 0.00240 \\
2452963.76104 & 9.56508 & 0.00244 \\
2452963.76493 & 9.57378 & 0.00241 \\
2452963.76883 & 9.57329 & 0.00238 \\
2452963.77285 & 9.56950 & 0.00246 \\
2452963.77674 & 9.56886 & 0.00239 \\
2452963.78062 & 9.56872 & 0.00244 \\
2452963.78451 & 9.57133 & 0.00241 \\
2452963.78851 & 9.56883 & 0.00244 \\
2452963.79240 & 9.55959 & 0.00246 \\
2452963.79630 & 9.57338 & 0.00244 \\
2452963.80016 & 9.56825 & 0.00254 \\
2452963.80417 & 9.56837 & 0.00244 \\
2452963.80806 & 9.56899 & 0.00231 \\
2452963.81195 & 9.56730 & 0.00245 \\
2452963.81584 & 9.57346 & 0.00240 \\
2452963.81986 & 9.56300 & 0.00255 \\
2452963.82374 & 9.57361 & 0.00236 \\
2452963.82761 & 9.57114 & 0.00253 \\
2452963.83151 & 9.56846 & 0.00243 \\
2452963.83553 & 9.58077 & 0.00266 \\
2452963.83941 & 9.56632 & 0.00251 \\
2452963.84329 & 9.57232 & 0.00248 \\
2452963.84717 & 9.54820 & 0.00257 \\
2452963.85119 & 9.58428 & 0.00317 \\
2452963.85892 & 9.56721 & 0.00307 \\
2452963.86280 & 9.54960 & 0.00312 \\
2452963.86681 & 9.56801 & 0.00240 \\
2452963.87068 & 9.57670 & 0.00259 \\
2452949.80119 & 9.56887 & 0.00250 \\
2452963.87456 & 9.57152 & 0.00253 \\
2452963.87846 & 9.57128 & 0.00240 \\
2452963.88244 & 9.57457 & 0.00264 \\
2452963.88638 & 9.56793 & 0.00256 \\
2452963.89028 & 9.57576 & 0.00243 \\
2452963.89417 & 9.56499 & 0.00242 \\
2452963.89820 & 9.57467 & 0.00242 \\
2452963.90209 & 9.56469 & 0.00270 \\
2452949.80514 & 9.57067 & 0.00253 \\
2452949.80906 & 9.57009 & 0.00240 \\
2452949.81300 & 9.56730 & 0.00249 \\
2452949.81707 & 9.56602 & 0.00251 \\
2452949.82102 & 9.57888 & 0.00270 \\
2452949.82496 & 9.57580 & 0.00278 \\
2452949.82889 & 9.56761 & 0.00252 \\
2452949.83297 & 9.56447 & 0.00243 \\
2452949.83691 & 9.57546 & 0.00243 \\
2452949.84243 & 9.57312 & 0.00251 \\
2452949.84639 & 9.56949 & 0.00256 \\
2452949.85034 & 9.56569 & 0.00248 \\
2452949.85428 & 9.56398 & 0.00268 \\
2452949.85836 & 9.56792 & 0.00260 \\
2452949.86229 & 9.56494 & 0.00267 \\
2452949.86623 & 9.56577 & 0.00254 \\
2452949.87017 & 9.56755 & 0.00271 \\
2452964.69437 & 9.56516 & 0.00269 \\
2452964.69824 & 9.56850 & 0.00263 \\
2452964.70212 & 9.57496 & 0.00237 \\
2452964.70599 & 9.57278 & 0.00253 \\
2452964.71001 & 9.58017 & 0.00241 \\
2452964.71389 & 9.56832 & 0.00251 \\
2452964.71779 & 9.57319 & 0.00244 \\
2452964.72167 & 9.57323 & 0.00255 \\
2452949.87424 & 9.56658 & 0.00262 \\
2452964.72567 & 9.56816 & 0.00249 \\
2452964.73341 & 9.56855 & 0.00264 \\
2452964.73732 & 9.57170 & 0.00241 \\
2452964.74132 & 9.56965 & 0.00237 \\
2452964.74521 & 9.57041 & 0.00250 \\
2452964.74908 & 9.57231 & 0.00240 \\
2452964.75298 & 9.56797 & 0.00249 \\
2452964.75698 & 9.57109 & 0.00241 \\
2452964.76088 & 9.56682 & 0.00245 \\
2452964.76476 & 9.56486 & 0.00238 \\
2452964.76865 & 9.57295 & 0.00235 \\
2452964.77266 & 9.57083 & 0.00242 \\
2452964.77654 & 9.57229 & 0.00242 \\
2452964.78041 & 9.56879 & 0.00243 \\
2452964.78429 & 9.56803 & 0.00235 \\
2452964.78832 & 9.57233 & 0.00252 \\
2452964.79221 & 9.57188 & 0.00242 \\
2452964.79609 & 9.57150 & 0.00247 \\
2452964.79996 & 9.56782 & 0.00239 \\
2452964.80397 & 9.57229 & 0.00239 \\
2452964.80784 & 9.57242 & 0.00241 \\
2452964.81172 & 9.56874 & 0.00254 \\
2452964.81560 & 9.56782 & 0.00244 \\
2452964.81962 & 9.57381 & 0.00246 \\
2452964.82351 & 9.57221 & 0.00240 \\
2452964.82740 & 9.57486 & 0.00249 \\
2452964.83128 & 9.56799 & 0.00246 \\
2452964.83529 & 9.57255 & 0.00253 \\
2452964.83917 & 9.56542 & 0.00257 \\
2452964.84305 & 9.57174 & 0.00254 \\
2452964.84693 & 9.57226 & 0.00246 \\
2452964.85096 & 9.57632 & 0.00251 \\
2452964.85484 & 9.56897 & 0.00249 \\
2452964.85873 & 9.57360 & 0.00250 \\
2452964.86262 & 9.57119 & 0.00242 \\
2452964.86663 & 9.56990 & 0.00245 \\
2452964.87051 & 9.57109 & 0.00246 \\
2452964.87440 & 9.57171 & 0.00245 \\
2452964.87828 & 9.57149 & 0.00280 \\
2452964.88228 & 9.57537 & 0.00337 \\
2452964.88614 & 9.56512 & 0.00324 \\
2452964.89002 & 9.56820 & 0.00294 \\
2452964.89389 & 9.58456 & 0.00398 \\
2452964.89789 & 9.56941 & 0.00304 \\
2452965.69425 & 9.56997 & 0.00281 \\
2452965.69813 & 9.57417 & 0.00280 \\
2452965.70201 & 9.57243 & 0.00254 \\
2452965.70590 & 9.56886 & 0.00237 \\
2452965.70991 & 9.57251 & 0.00254 \\
2452965.71380 & 9.57099 & 0.00265 \\
2452965.71769 & 9.56243 & 0.00260 \\
2452965.72158 & 9.56535 & 0.00249 \\
2452965.72561 & 9.56732 & 0.00261 \\
2452965.72949 & 9.57904 & 0.00255 \\
2452965.73338 & 9.56253 & 0.00256 \\
2452965.73726 & 9.57669 & 0.00258 \\
2452965.74127 & 9.57287 & 0.00260 \\
2452965.74515 & 9.57054 & 0.00264 \\
2452965.74904 & 9.57048 & 0.00253 \\
2452965.75294 & 9.57133 & 0.00263 \\
2452965.75696 & 9.56578 & 0.00236 \\
2452965.76086 & 9.56727 & 0.00241 \\
2452965.76474 & 9.57076 & 0.00241 \\
2452965.76865 & 9.56772 & 0.00258 \\
2452965.77267 & 9.57546 & 0.00254 \\
2452965.77655 & 9.57172 & 0.00253 \\
2452965.78042 & 9.57604 & 0.00243 \\
2452965.78432 & 9.57307 & 0.00244 \\
2452965.78833 & 9.57095 & 0.00243 \\
2452965.79222 & 9.56831 & 0.00240 \\
2452965.79610 & 9.57174 & 0.00238 \\
2452965.79999 & 9.56633 & 0.00239 \\
2452965.80399 & 9.57053 & 0.00236 \\
2452965.81181 & 9.57101 & 0.00241 \\
2452965.81570 & 9.56679 & 0.00250 \\
2452965.81971 & 9.56482 & 0.00250 \\
2452965.82360 & 9.57207 & 0.00242 \\
2452965.82747 & 9.57053 & 0.00244 \\
2452965.83135 & 9.57389 & 0.00244 \\
2452965.83537 & 9.56428 & 0.00248 \\
2452965.83926 & 9.56145 & 0.00252 \\
2452965.84314 & 9.57128 & 0.00246 \\
2452965.84702 & 9.56641 & 0.00238 \\
2452965.85104 & 9.56646 & 0.00240 \\
2452965.85493 & 9.56406 & 0.00253 \\
2452965.85886 & 9.57468 & 0.00244 \\
2452965.86276 & 9.55781 & 0.00257 \\
2452965.86677 & 9.56726 & 0.00250 \\
2452965.87067 & 9.56871 & 0.00237 \\
2452965.87455 & 9.57623 & 0.00249 \\
2452965.87843 & 9.56983 & 0.00246 \\
2452965.88244 & 9.57256 & 0.00249 \\
2452965.88632 & 9.57612 & 0.00249 \\
2452965.89022 & 9.57188 & 0.00247 \\
2452965.89410 & 9.56999 & 0.00240 \\
2452965.89812 & 9.56102 & 0.00251 \\
2452966.69419 & 9.56991 & 0.00263 \\
2452966.69808 & 9.56949 & 0.00245 \\
2452966.70197 & 9.57118 & 0.00251 \\
2452966.70588 & 9.56715 & 0.00249 \\
2452966.70989 & 9.56992 & 0.00248 \\
2452966.71377 & 9.57032 & 0.00249 \\
2452966.71767 & 9.56438 & 0.00249 \\
2452966.72156 & 9.56913 & 0.00238 \\
2452966.72557 & 9.56985 & 0.00242 \\
2452966.72945 & 9.57339 & 0.00243 \\
2452966.73333 & 9.57042 & 0.00247 \\
2452966.73722 & 9.57215 & 0.00236 \\
2452966.74123 & 9.56583 & 0.00249 \\
2452966.74511 & 9.57443 & 0.00245 \\
2452966.74900 & 9.56824 & 0.00246 \\
2452966.75688 & 9.57033 & 0.00245 \\
2452966.76075 & 9.56635 & 0.00247 \\
2452966.76463 & 9.57199 & 0.00244 \\
2452966.76853 & 9.56867 & 0.00233 \\
2452966.77260 & 9.57305 & 0.00240 \\
2452966.77648 & 9.57089 & 0.00246 \\
2452966.78037 & 9.57332 & 0.00243 \\
2452966.78427 & 9.56771 & 0.00239 \\
2452966.78835 & 9.57475 & 0.00242 \\
2452966.79222 & 9.57032 & 0.00245 \\
2452966.79610 & 9.56498 & 0.00236 \\
2452966.79998 & 9.56979 & 0.00251 \\
2452966.80400 & 9.57858 & 0.00252 \\
2452966.80788 & 9.57666 & 0.00243 \\
2452966.81178 & 9.57189 & 0.00242 \\
2452966.81567 & 9.57031 & 0.00242 \\
2452966.81965 & 9.57215 & 0.00245 \\
2452966.82354 & 9.56605 & 0.00235 \\
2452966.82742 & 9.57293 & 0.00232 \\
2452966.83130 & 9.57201 & 0.00250 \\
2452966.83530 & 9.57131 & 0.00236 \\
2452966.83919 & 9.56772 & 0.00241 \\
2452966.84307 & 9.56914 & 0.00253 \\
2452966.84696 & 9.56755 & 0.00245 \\
2452966.85098 & 9.56775 & 0.00246 \\
2452966.85493 & 9.57122 & 0.00250 \\
2452966.85883 & 9.56984 & 0.00252 \\
2452966.86271 & 9.56613 & 0.00273 \\
2452966.86669 & 9.57234 & 0.00242 \\
2452966.87058 & 9.56372 & 0.00274 \\
2452966.87445 & 9.57635 & 0.00253 \\
2452966.87833 & 9.57374 & 0.00264 \\
2452966.88621 & 9.56314 & 0.00246 \\
2452966.89010 & 9.57073 & 0.00272 \\
2452966.89398 & 9.56940 & 0.00257 \\
2452967.69407 & 9.56616 & 0.00291 \\
2452967.69796 & 9.56822 & 0.00253 \\
2452967.70186 & 9.56238 & 0.00250 \\
2452967.70575 & 9.57077 & 0.00257 \\
2452967.70975 & 9.57190 & 0.00259 \\
2452967.71363 & 9.57203 & 0.00248 \\
2452967.71750 & 9.56736 & 0.00253 \\
2452967.72141 & 9.56771 & 0.00244 \\
2452967.72543 & 9.56493 & 0.00247 \\
2452967.72931 & 9.57392 & 0.00260 \\
2452967.73319 & 9.56413 & 0.00262 \\
2452967.73709 & 9.56371 & 0.00251 \\
2452967.74109 & 9.57582 & 0.00280 \\
2452967.74498 & 9.56865 & 0.00257 \\
2452967.74886 & 9.57302 & 0.00258 \\
2452967.75273 & 9.57226 & 0.00242 \\
2452967.75674 & 9.56845 & 0.00253 \\
2452967.76063 & 9.57464 & 0.00261 \\
2452967.76452 & 9.56839 & 0.00253 \\
2452967.76840 & 9.56684 & 0.00260 \\
2452967.77240 & 9.57430 & 0.00247 \\
2452967.77629 & 9.57168 & 0.00256 \\
2452967.78017 & 9.56605 & 0.00264 \\
2452967.78405 & 9.56501 & 0.00258 \\
2452967.78807 & 9.56997 & 0.00255 \\
2452967.79198 & 9.57518 & 0.00251 \\
2452967.79586 & 9.57228 & 0.00253 \\
2452967.79975 & 9.57277 & 0.00253 \\
2452967.80378 & 9.57468 & 0.00249 \\
2452967.80766 & 9.57199 & 0.00270 \\
2452967.81155 & 9.56787 & 0.00245 \\
2452967.81543 & 9.56347 & 0.00273 \\
2452967.81944 & 9.57691 & 0.00257 \\
2452967.82331 & 9.56859 & 0.00261 \\
2452967.82719 & 9.57222 & 0.00257 \\
2452967.83107 & 9.57325 & 0.00252 \\
2452967.83508 & 9.57113 & 0.00261 \\
2452967.83896 & 9.56801 & 0.00242 \\
2452967.84283 & 9.56978 & 0.00254 \\
2452967.84671 & 9.57435 & 0.00250 \\
2452967.85072 & 9.57125 & 0.00273 \\
2452967.85460 & 9.56789 & 0.00263 \\
2452967.85848 & 9.57401 & 0.00267 \\
2452967.86237 & 9.56580 & 0.00262 \\
2452967.86640 & 9.56786 & 0.00272 \\
2452967.87027 & 9.56604 & 0.00276 \\
2452967.87416 & 9.56808 & 0.00263 \\
2452967.87804 & 9.58310 & 0.00252 \\
2452967.88206 & 9.56407 & 0.00252 \\
2452967.88596 & 9.56985 & 0.00257 \\
2452967.88983 & 9.57512 & 0.00268 \\
2452968.69409 & 9.57843 & 0.00269 \\
2452968.69797 & 9.56471 & 0.00277 \\
2452968.70184 & 9.57366 & 0.00260 \\
2452968.70573 & 9.57123 & 0.00256 \\
2452968.70975 & 9.56818 & 0.00242 \\
2452968.71364 & 9.57258 & 0.00268 \\
2452968.71753 & 9.57072 & 0.00255 \\
2452968.72142 & 9.57420 & 0.00246 \\
2452968.72543 & 9.57346 & 0.00259 \\
2452968.72931 & 9.56967 & 0.00264 \\
2452968.73320 & 9.57520 & 0.00252 \\
2452968.73709 & 9.57393 & 0.00269 \\
2452968.74111 & 9.57333 & 0.00269 \\
2452968.74500 & 9.57499 & 0.00277 \\
2452968.74887 & 9.57188 & 0.00256 \\
2452968.75276 & 9.56817 & 0.00270 \\
2452978.69422 & 9.57294 & 0.00273 \\
2452978.69811 & 9.57456 & 0.00255 \\
2452978.70197 & 9.56969 & 0.00249 \\
2452978.70575 & 9.57204 & 0.00242 \\
2452978.70964 & 9.57940 & 0.00254 \\
2452978.71350 & 9.57718 & 0.00270 \\
2452978.71729 & 9.56514 & 0.00259 \\
2452978.72116 & 9.56778 & 0.00252 \\
2452978.72505 & 9.57687 & 0.00253 \\
2452978.72882 & 9.57768 & 0.00245 \\
2452978.73270 & 9.57169 & 0.00252 \\
2452978.73658 & 9.57365 & 0.00246 \\
2452978.74033 & 9.57393 & 0.00259 \\
2452978.74421 & 9.57170 & 0.00253 \\
2452978.74809 & 9.57530 & 0.00253 \\
2452978.75186 & 9.56686 & 0.00271 \\
2452978.75574 & 9.56783 & 0.00260 \\
2452978.75962 & 9.57627 & 0.00256 \\
2452978.76341 & 9.57561 & 0.00264 \\
2452978.76728 & 9.56952 & 0.00256 \\
2452978.77117 & 9.55618 & 0.00242 \\
2452978.77494 & 9.56450 & 0.00267 \\
2452978.77881 & 9.56523 & 0.00242 \\
2452978.78269 & 9.55992 & 0.00255 \\
2452978.78645 & 9.57464 & 0.00247 \\
2452978.79034 & 9.56810 & 0.00253 \\
2452978.79422 & 9.58503 & 0.00261 \\
2452978.79801 & 9.56492 & 0.00287 \\
2452978.80189 & 9.57205 & 0.00254 \\
2452978.80577 & 9.55952 & 0.00241 \\
2452978.80955 & 9.56750 & 0.00269 \\
2452978.81344 & 9.56633 & 0.00268 \\
2452978.81732 & 9.56484 & 0.00273 \\
2452978.82112 & 9.56765 & 0.00274 \\
2452978.82499 & 9.57153 & 0.00260 \\
2452978.82887 & 9.58015 & 0.00259 \\
2452978.83265 & 9.57322 & 0.00282 \\
2452978.83653 & 9.56946 & 0.00250 \\
2452978.84040 & 9.57021 & 0.00270 \\
2452978.84415 & 9.56959 & 0.00281 \\
2452978.84804 & 9.56999 & 0.00274 \\
2452978.85191 & 9.57095 & 0.00256 \\
2452978.85570 & 9.56531 & 0.00272 \\
2452978.85955 & 9.56175 & 0.00260 \\
2452978.86343 & 9.57614 & 0.00281 \\
2452979.69439 & 9.56497 & 0.00253 \\
2452979.69828 & 9.56792 & 0.00252 \\
2452979.70218 & 9.56335 & 0.00253 \\
2452979.70606 & 9.57958 & 0.00281 \\
2452979.71007 & 9.58085 & 0.00243 \\
2452979.71396 & 9.56936 & 0.00259 \\
2452979.71783 & 9.57455 & 0.00260 \\
2452979.72172 & 9.56961 & 0.00254 \\
2452979.72573 & 9.57813 & 0.00232 \\
2452979.72961 & 9.57163 & 0.00242 \\
2452979.73347 & 9.56805 & 0.00245 \\
2452979.73736 & 9.57376 & 0.00268 \\
2452979.74137 & 9.56538 & 0.00273 \\
2452979.74526 & 9.56766 & 0.00256 \\
2452979.74914 & 9.57323 & 0.00258 \\
2452979.75303 & 9.57787 & 0.00259 \\
2452979.75705 & 9.56577 & 0.00253 \\
2452979.76093 & 9.57065 & 0.00242 \\
2452979.76481 & 9.57269 & 0.00247 \\
2452979.76869 & 9.57350 & 0.00243 \\
2452979.77270 & 9.56962 & 0.00268 \\
2452979.77659 & 9.56625 & 0.00249 \\
2452979.78047 & 9.57126 & 0.00262 \\
2452979.78435 & 9.57398 & 0.00242 \\
2452979.78836 & 9.56285 & 0.00244 \\
2452979.79226 & 9.57162 & 0.00256 \\
2452979.79614 & 9.57081 & 0.00241 \\
2452979.80002 & 9.57012 & 0.00252 \\
2452979.80403 & 9.56984 & 0.00270 \\
2452979.80793 & 9.57120 & 0.00264 \\
2452979.81184 & 9.57428 & 0.00264 \\
2452979.81573 & 9.57205 & 0.00261 \\
2452979.81974 & 9.58180 & 0.00281 \\
2452979.82362 & 9.56987 & 0.00264 \\
2452979.82751 & 9.57209 & 0.00281 \\
2452979.83139 & 9.56954 & 0.00266 \\
2452979.83539 & 9.57037 & 0.00268 \\
2452979.83929 & 9.57366 & 0.00272 \\
2452979.84318 & 9.56574 & 0.00272 \\
2452979.84706 & 9.56941 & 0.00280 \\
2452979.85107 & 9.57454 & 0.00296 \\
2452979.85495 & 9.56992 & 0.00253 \\
2452979.85884 & 9.56779 & 0.00267 \\
2452980.69476 & 9.56214 & 0.00266 \\
2452980.69865 & 9.57207 & 0.00256 \\
2452980.70253 & 9.56657 & 0.00249 \\
2452980.70641 & 9.56742 & 0.00241 \\
2452980.71043 & 9.56787 & 0.00262 \\
2452980.71433 & 9.56917 & 0.00245 \\
2452980.71822 & 9.57922 & 0.00252 \\
2452980.72210 & 9.56206 & 0.00244 \\
2452980.72613 & 9.57272 & 0.00251 \\
2452980.73001 & 9.56528 & 0.00251 \\
2452980.73389 & 9.56874 & 0.00262 \\
2452980.73778 & 9.56190 & 0.00239 \\
2452980.74180 & 9.56825 & 0.00258 \\
2452980.74570 & 9.57240 & 0.00258 \\
2452980.74959 & 9.56719 & 0.00261 \\
2452980.75347 & 9.56906 & 0.00251 \\
2452980.75749 & 9.56666 & 0.00246 \\
2452980.76138 & 9.57403 & 0.00260 \\
2452980.76525 & 9.57228 & 0.00252 \\
2452980.76913 & 9.56833 & 0.00259 \\
2452980.77314 & 9.56491 & 0.00235 \\
2452980.77702 & 9.56720 & 0.00247 \\
2452980.78091 & 9.56715 & 0.00257 \\
2452980.78479 & 9.57661 & 0.00254 \\
2452980.78880 & 9.57380 & 0.00273 \\
2452980.79268 & 9.56997 & 0.00260 \\
2452980.79656 & 9.56349 & 0.00244 \\
2452980.80045 & 9.56853 & 0.00266 \\
2452980.80443 & 9.56974 & 0.00249 \\
2452980.80831 & 9.57147 & 0.00256 \\
2452980.81219 & 9.56422 & 0.00258 \\
2452980.81607 & 9.56734 & 0.00250 \\
2452980.82008 & 9.56745 & 0.00252 \\
2452980.82395 & 9.57422 & 0.00266 \\
2452980.82784 & 9.57207 & 0.00257 \\
2452980.83173 & 9.56880 & 0.00259 \\
2452980.83574 & 9.57349 & 0.00256 \\
2452980.83963 & 9.56701 & 0.00253 \\
2452980.84351 & 9.56226 & 0.00276 \\
2452980.84739 & 9.55831 & 0.00262 \\
2452980.85528 & 9.57149 & 0.00269 \\
2452981.69453 & 9.55745 & 0.00270 \\
2452981.69846 & 9.56832 & 0.00264 \\
2452981.70234 & 9.56601 & 0.00242 \\
2452981.70621 & 9.57367 & 0.00257 \\
2452981.71411 & 9.56495 & 0.00236 \\
2452981.71800 & 9.57011 & 0.00249 \\
2452981.72189 & 9.56155 & 0.00265 \\
2452981.72590 & 9.57313 & 0.00240 \\
2452981.72977 & 9.56400 & 0.00254 \\
2452981.73366 & 9.56772 & 0.00236 \\
2452981.73755 & 9.56583 & 0.00252 \\
2452981.74154 & 9.56780 & 0.00243 \\
2452981.74542 & 9.56599 & 0.00247 \\
2452981.74930 & 9.56729 & 0.00238 \\
2452981.75319 & 9.57106 & 0.00260 \\
2452981.75720 & 9.56964 & 0.00250 \\
2452981.76108 & 9.57679 & 0.00242 \\
2452981.76498 & 9.56941 & 0.00255 \\
2452981.76884 & 9.57447 & 0.00257 \\
2452981.77284 & 9.56812 & 0.00250 \\
2452981.77674 & 9.56599 & 0.00247 \\
2452981.78062 & 9.56537 & 0.00252 \\
2452981.78450 & 9.56892 & 0.00272 \\
2452981.78853 & 9.56937 & 0.00242 \\
2452981.79239 & 9.57367 & 0.00265 \\
2452981.79627 & 9.57106 & 0.00275 \\
2452981.80015 & 9.56981 & 0.00257 \\
2452981.80416 & 9.56694 & 0.00277 \\
2452981.80805 & 9.57177 & 0.00260 \\
2452981.81193 & 9.57352 & 0.00282 \\
2452981.81581 & 9.57323 & 0.00263 \\
2452981.81982 & 9.57428 & 0.00254 \\
2452981.82371 & 9.56834 & 0.00282 \\
2452981.82760 & 9.56740 & 0.00266 \\
2452981.83149 & 9.57328 & 0.00277 \\
2452981.83555 & 9.57134 & 0.00252 \\
2452981.83943 & 9.56351 & 0.00261 \\
2452981.84332 & 9.56960 & 0.00274 \\
2452981.84720 & 9.56759 & 0.00267 \\
2452981.85120 & 9.57212 & 0.00266 \\
2452984.69503 & 9.57366 & 0.00249 \\
2452984.69893 & 9.56943 & 0.00252 \\
2452984.70280 & 9.57541 & 0.00242 \\
2452984.70668 & 9.57543 & 0.00258 \\
2452984.71068 & 9.57546 & 0.00254 \\
2452984.71458 & 9.56767 & 0.00248 \\
2452984.71846 & 9.56577 & 0.00238 \\
2452984.72235 & 9.56657 & 0.00259 \\
2452984.72635 & 9.56532 & 0.00248 \\
2452984.73024 & 9.57175 & 0.00249 \\
2452984.73413 & 9.57549 & 0.00249 \\
2452984.73803 & 9.57110 & 0.00237 \\
2452984.74204 & 9.57416 & 0.00260 \\
2452984.74592 & 9.57125 & 0.00240 \\
2452984.74982 & 9.57800 & 0.00254 \\
2452984.75372 & 9.57317 & 0.00239 \\
2452984.75773 & 9.56629 & 0.00264 \\
2452984.76161 & 9.57129 & 0.00269 \\
2452984.76551 & 9.56781 & 0.00251 \\
2452984.76940 & 9.57071 & 0.00252 \\
2452984.77341 & 9.57166 & 0.00256 \\
2452984.77730 & 9.56474 & 0.00260 \\
2452984.78119 & 9.56844 & 0.00255 \\
2452984.78506 & 9.56793 & 0.00263 \\
2452984.78908 & 9.57157 & 0.00262 \\
2452984.79297 & 9.56664 & 0.00268 \\
2452984.79686 & 9.56694 & 0.00268 \\
2452984.80074 & 9.56815 & 0.00282 \\
2452984.80475 & 9.55922 & 0.00274 \\
2452984.80864 & 9.56912 & 0.00270 \\
2452984.81252 & 9.56979 & 0.00354 \\
2452950.71012 & 9.57127 & 0.00304 \\
2452950.71406 & 9.56351 & 0.00254 \\
2452950.71799 & 9.55993 & 0.00264 \\
2452950.72194 & 9.57021 & 0.00249 \\
2452950.72600 & 9.56326 & 0.00254 \\
2452950.72993 & 9.56991 & 0.00252 \\
2452950.73387 & 9.57128 & 0.00267 \\
2452950.73781 & 9.56742 & 0.00246 \\
2452950.74187 & 9.57072 & 0.00269 \\
2452950.74580 & 9.56277 & 0.00245 \\
2452950.74975 & 9.56999 & 0.00252 \\
2452950.75369 & 9.57009 & 0.00250 \\
2452950.75776 & 9.57004 & 0.00244 \\
2452950.76170 & 9.57110 & 0.00253 \\
2452950.76564 & 9.57353 & 0.00244 \\
2452950.77364 & 9.56774 & 0.00252 \\
2452950.77757 & 9.56705 & 0.00274 \\
2452950.78151 & 9.56639 & 0.00245 \\
2452950.78544 & 9.56898 & 0.00261 \\
2452950.78951 & 9.56525 & 0.00255 \\
2452950.79345 & 9.57007 & 0.00259 \\
2452950.79739 & 9.56931 & 0.00247 \\
2452950.80132 & 9.56132 & 0.00266 \\
2452950.88007 & 9.56677 & 0.00278 \\
2452950.88413 & 9.57239 & 0.00261 \\
2452950.88806 & 9.56455 & 0.00260 \\
2452950.89202 & 9.56261 & 0.00281 \\
2452950.89596 & 9.56716 & 0.00252 \\
2452950.90003 & 9.56849 & 0.00263 \\
2452950.90397 & 9.57587 & 0.00285 \\
2452951.69680 & 9.57152 & 0.00281 \\
2452951.70074 & 9.57110 & 0.00268 \\
2452951.70468 & 9.56698 & 0.00263 \\
2452951.70859 & 9.56748 & 0.00256 \\
2452951.71266 & 9.57502 & 0.00278 \\
2452951.71660 & 9.57339 & 0.00278 \\
2452951.72053 & 9.56845 & 0.00268 \\
2452951.72446 & 9.57718 & 0.00260 \\
2452951.72853 & 9.57680 & 0.00246 \\
2452951.73246 & 9.57791 & 0.00262 \\
2452951.73643 & 9.57436 & 0.00258 \\
2452951.74037 & 9.58207 & 0.00272 \\
2452951.74443 & 9.57951 & 0.00249 \\
2452951.74837 & 9.57748 & 0.00259 \\
2452951.75232 & 9.58075 & 0.00266 \\
2452951.75626 & 9.58067 & 0.00249 \\
2452951.76032 & 9.57268 & 0.00251 \\
2452951.76426 & 9.58141 & 0.00254 \\
2452951.76820 & 9.56852 & 0.00266 \\
2452951.77214 & 9.57309 & 0.00245 \\
2452951.77620 & 9.57968 & 0.00270 \\
2452951.78015 & 9.57499 & 0.00249 \\
2452951.78408 & 9.57679 & 0.00262 \\
2452951.78802 & 9.57932 & 0.00264 \\
2452951.79208 & 9.58397 & 0.00259 \\
2452951.79603 & 9.57496 & 0.00275 \\
2452951.79996 & 9.57178 & 0.00240 \\
2452951.80391 & 9.57605 & 0.00278 \\
2452951.80798 & 9.57862 & 0.00259 \\
2452951.81192 & 9.57690 & 0.00256 \\
2452951.81586 & 9.58311 & 0.00262 \\
2452951.81978 & 9.57579 & 0.00283 \\
2452951.82383 & 9.57835 & 0.00290 \\
2452951.82779 & 9.57210 & 0.00262 \\
2452951.83174 & 9.58324 & 0.00275 \\
2452951.83567 & 9.57592 & 0.00254 \\
2452951.83974 & 9.57613 & 0.00251 \\
2452951.84367 & 9.57469 & 0.00271 \\
2452951.84762 & 9.58722 & 0.00266 \\
2452951.85156 & 9.56470 & 0.00284 \\
2452951.85564 & 9.57408 & 0.00247 \\
2452951.85959 & 9.57788 & 0.00267 \\
2452951.86353 & 9.58446 & 0.00256 \\
2452951.86747 & 9.56806 & 0.00274 \\
2452951.87153 & 9.57166 & 0.00274 \\
2452951.87546 & 9.56520 & 0.00272 \\
2452951.87942 & 9.57251 & 0.00263 \\
2452951.88335 & 9.56745 & 0.00276 \\
2452951.88741 & 9.56861 & 0.00289 \\
2452951.89134 & 9.56548 & 0.00280 \\
2452951.89527 & 9.56353 & 0.00271 \\
2452951.89921 & 9.56682 & 0.00280 \\
2452952.76377 & 9.57111 & 0.00261 \\
2452952.76771 & 9.57053 & 0.00258 \\
2452952.77166 & 9.56874 & 0.00276 \\
2452952.77557 & 9.56794 & 0.00263 \\
2452952.77963 & 9.56881 & 0.00282 \\
2452952.78357 & 9.57092 & 0.00258 \\
2452952.78751 & 9.57475 & 0.00270 \\
2452952.79145 & 9.56496 & 0.00273 \\
2452952.79553 & 9.56961 & 0.00263 \\
2452952.79946 & 9.56620 & 0.00271 \\
2452952.80341 & 9.56774 & 0.00250 \\
2452952.80736 & 9.57012 & 0.00249 \\
2452952.81142 & 9.56246 & 0.00249 \\
2452952.81535 & 9.57253 & 0.00259 \\
2452952.81929 & 9.56707 & 0.00260 \\
2452952.82323 & 9.56890 & 0.00254 \\
2452952.82730 & 9.57023 & 0.00263 \\
2452952.83123 & 9.57506 & 0.00267 \\
2452952.83517 & 9.56921 & 0.00279 \\
2453922.88684 & 9.57063 & 0.00340 \\
2453922.89068 & 9.57042 & 0.00351 \\
2453922.89447 & 9.54321 & 0.00311 \\
2453922.89826 & 9.57865 & 0.00333 \\
2453922.90203 & 9.57589 & 0.00329 \\
2453922.90585 & 9.56816 & 0.00315 \\
2453922.90963 & 9.56831 & 0.00338 \\
2453922.91720 & 9.56810 & 0.00308 \\
2453922.92098 & 9.56723 & 0.00308 \\
2453922.92497 & 9.56501 & 0.00307 \\
2453922.92879 & 9.56891 & 0.00318 \\
2453922.93257 & 9.56563 & 0.00313 \\
2453922.94016 & 9.56909 & 0.00293 \\
2453922.94397 & 9.57383 & 0.00285 \\
2453922.94780 & 9.56200 & 0.00286 \\
2453922.95160 & 9.55833 & 0.00299 \\
2453922.95540 & 9.56605 & 0.00290 \\
2453922.95919 & 9.57359 & 0.00282 \\
2453922.96297 & 9.56861 & 0.00281 \\
2453922.96676 & 9.56962 & 0.00273 \\
2453922.97055 & 9.57578 & 0.00296 \\
2453922.97433 & 9.56828 & 0.00282 \\
2453922.97811 & 9.57053 & 0.00275 \\
2453922.98206 & 9.56758 & 0.00295 \\
2453922.98586 & 9.57213 & 0.00278 \\
2453922.98968 & 9.57040 & 0.00269 \\
2453922.99348 & 9.56300 & 0.00288 \\
2453922.99728 & 9.57250 & 0.00286 \\
2453923.00107 & 9.57335 & 0.00284 \\
2453923.00485 & 9.57299 & 0.00283 \\
2453923.00864 & 9.56617 & 0.00260 \\
2453923.01245 & 9.56880 & 0.00265 \\
2453923.01624 & 9.56762 & 0.00264 \\
2453923.02004 & 9.57078 & 0.00262 \\
2453923.02764 & 9.56792 & 0.00268 \\
2453923.03144 & 9.57178 & 0.00271 \\
2453923.03523 & 9.56787 & 0.00257 \\
2453923.03915 & 9.56742 & 0.00260 \\
2453923.04295 & 9.56221 & 0.00262 \\
2453923.04675 & 9.57165 & 0.00261 \\
2453923.05053 & 9.56958 & 0.00263 \\
2453923.05433 & 9.56520 & 0.00270 \\
2453923.05812 & 9.56966 & 0.00249 \\
2453923.06192 & 9.56581 & 0.00271 \\
2453923.06572 & 9.56726 & 0.00260 \\
2453923.06957 & 9.57046 & 0.00267 \\
2453923.07337 & 9.56662 & 0.00264 \\
2453923.07716 & 9.56512 & 0.00258 \\
2453923.11307 & 9.56966 & 0.00249 \\
2453923.11688 & 9.56194 & 0.00267 \\
2453923.87954 & 9.58656 & 0.00322 \\
2453923.88715 & 9.58005 & 0.00337 \\
2453923.89094 & 9.57933 & 0.00319 \\
2453923.89473 & 9.58348 & 0.00327 \\
2453923.89854 & 9.57345 & 0.00327 \\
2453923.90236 & 9.58376 & 0.00309 \\
2453923.90614 & 9.58231 & 0.00331 \\
2453923.90993 & 9.57559 & 0.00334 \\
2453923.91373 & 9.57944 & 0.00325 \\
2453923.91752 & 9.58551 & 0.00317 \\
2453923.92130 & 9.58679 & 0.00308 \\
2453923.92527 & 9.57096 & 0.00289 \\
2453923.92904 & 9.58008 & 0.00319 \\
2453923.93288 & 9.58522 & 0.00318 \\
2453923.93665 & 9.57567 & 0.00302 \\
2453923.94043 & 9.57852 & 0.00299 \\
2453923.94423 & 9.57246 & 0.00327 \\
2453923.94802 & 9.57853 & 0.00316 \\
2453923.95181 & 9.57974 & 0.00297 \\
2453923.95561 & 9.58170 & 0.00290 \\
2453923.95939 & 9.57684 & 0.00298 \\
2453923.96326 & 9.57276 & 0.00284 \\
2453923.96708 & 9.57479 & 0.00301 \\
2453923.97092 & 9.56813 & 0.00273 \\
2453923.97471 & 9.57686 & 0.00286 \\
2453923.97849 & 9.57907 & 0.00292 \\
2453923.98249 & 9.58211 & 0.00289 \\
2453923.98627 & 9.58218 & 0.00298 \\
2453923.99005 & 9.58012 & 0.00276 \\
2453923.99387 & 9.57386 & 0.00280 \\
2453923.99769 & 9.57587 & 0.00281 \\
2453924.00164 & 9.56850 & 0.00283 \\
2453924.00543 & 9.57148 & 0.00272 \\
2453924.00924 & 9.56894 & 0.00268 \\
2453924.01304 & 9.56828 & 0.00281 \\
2453924.01684 & 9.57175 & 0.00281 \\
2453924.02441 & 9.56514 & 0.00281 \\
2453924.02843 & 9.56756 & 0.00264 \\
2453924.03224 & 9.56850 & 0.00275 \\
2453924.03603 & 9.56910 & 0.00268 \\
2453924.04001 & 9.56508 & 0.00267 \\
2453924.04381 & 9.56388 & 0.00271 \\
2453924.04760 & 9.56626 & 0.00260 \\
2453924.05140 & 9.55854 & 0.00278 \\
2453924.05520 & 9.56730 & 0.00269 \\
2453924.05900 & 9.57245 & 0.00259 \\
2453924.06306 & 9.56706 & 0.00261 \\
2453924.06687 & 9.57032 & 0.00268 \\
2453924.07067 & 9.57103 & 0.00267 \\
2453924.07447 & 9.57049 & 0.00266 \\
2453924.10742 & 9.57150 & 0.00267 \\
2453924.11121 & 9.56736 & 0.00274 \\
2453924.11499 & 9.57155 & 0.00271 \\
2453924.11877 & 9.56290 & 0.00270 \\
2453924.87503 & 9.57027 & 0.00335 \\
2453924.87886 & 9.56190 & 0.00309 \\
2453924.88263 & 9.56616 & 0.00310 \\
2453924.88641 & 9.57163 & 0.00332 \\
2453924.89019 & 9.57484 & 0.00326 \\
2453924.89397 & 9.57097 & 0.00319 \\
2453924.89775 & 9.56170 & 0.00320 \\
2453924.90153 & 9.57133 & 0.00334 \\
2453924.90531 & 9.57049 & 0.00303 \\
2453924.90909 & 9.56779 & 0.00321 \\
2453924.91288 & 9.56759 & 0.00296 \\
2453924.91667 & 9.56603 & 0.00301 \\
2453924.92045 & 9.56543 & 0.00307 \\
2453924.92437 & 9.56975 & 0.00292 \\
2453924.92814 & 9.56801 & 0.00290 \\
2453924.93193 & 9.56552 & 0.00304 \\
2453924.93571 & 9.56996 & 0.00307 \\
2453924.93948 & 9.56674 & 0.00308 \\
2453924.94327 & 9.57339 & 0.00315 \\
2453924.94705 & 9.57128 & 0.00273 \\
2453924.95083 & 9.57335 & 0.00287 \\
2453924.95461 & 9.56451 & 0.00280 \\
2453924.95839 & 9.56462 & 0.00311 \\
2453924.96218 & 9.56679 & 0.00301 \\
2453924.96597 & 9.56123 & 0.00301 \\
2453924.96975 & 9.57252 & 0.00302 \\
2453924.97353 & 9.56172 & 0.00292 \\
2453924.97732 & 9.56732 & 0.00293 \\
2453924.98123 & 9.57233 & 0.00284 \\
2453924.98503 & 9.57212 & 0.00274 \\
2453924.98882 & 9.56500 & 0.00263 \\
2453924.99261 & 9.56958 & 0.00290 \\
2453924.99639 & 9.57106 & 0.00299 \\
2453925.00017 & 9.56422 & 0.00287 \\
2453925.00395 & 9.56481 & 0.00294 \\
2453925.00773 & 9.56678 & 0.00259 \\
2453925.01151 & 9.56232 & 0.00270 \\
2453925.01530 & 9.57284 & 0.00270 \\
2453925.01909 & 9.57028 & 0.00265 \\
2453925.02288 & 9.56443 & 0.00261 \\
2453925.02666 & 9.56654 & 0.00274 \\
2453925.03045 & 9.56934 & 0.00260 \\
2453925.03423 & 9.56804 & 0.00273 \\
2453925.03815 & 9.56733 & 0.00258 \\
2453925.04193 & 9.56893 & 0.00263 \\
2453925.04572 & 9.56864 & 0.00277 \\
2453925.04951 & 9.57010 & 0.00263 \\
2453925.05329 & 9.57284 & 0.00268 \\
2453925.05707 & 9.56842 & 0.00255 \\
2453925.06086 & 9.57028 & 0.00262 \\
2453925.06464 & 9.56863 & 0.00278 \\
2453925.06842 & 9.56961 & 0.00271 \\
2453925.07221 & 9.57494 & 0.00261 \\
2453925.10738 & 9.56638 & 0.00261 \\
2453925.11117 & 9.56868 & 0.00263 \\
2453925.11495 & 9.56540 & 0.00273 \\
2453925.11873 & 9.56117 & 0.00293 \\
2453925.87510 & 9.56705 & 0.00361 \\
2453925.87893 & 9.57215 & 0.00366 \\
2453925.88271 & 9.56314 & 0.00389 \\
2453925.88649 & 9.57070 & 0.00346 \\
2453925.89028 & 9.57054 & 0.00355 \\
2453925.89406 & 9.56496 & 0.00342 \\
2453925.89784 & 9.58029 & 0.00329 \\
2453925.90161 & 9.56538 & 0.00354 \\
2453925.90538 & 9.56437 & 0.00309 \\
2453925.90915 & 9.56995 & 0.00323 \\
2453925.91293 & 9.57094 & 0.00330 \\
2453925.91671 & 9.56313 & 0.00319 \\
2453925.92049 & 9.57311 & 0.00339 \\
2453925.92440 & 9.56460 & 0.00299 \\
2453925.92819 & 9.56606 & 0.00318 \\
2453925.93198 & 9.57050 & 0.00309 \\
2453925.93575 & 9.57029 & 0.00312 \\
2453925.93953 & 9.56974 & 0.00326 \\
2453925.94331 & 9.56756 & 0.00320 \\
2453925.94710 & 9.55782 & 0.00295 \\
2453925.95088 & 9.56677 & 0.00321 \\
2453925.95467 & 9.56134 & 0.00285 \\
2453925.95845 & 9.57110 & 0.00320 \\
2453925.96223 & 9.57268 & 0.00303 \\
2453925.96601 & 9.57563 & 0.00299 \\
2453925.96979 & 9.57219 & 0.00298 \\
2453925.97357 & 9.57119 & 0.00310 \\
2453925.97736 & 9.56583 & 0.00300 \\
2453925.98128 & 9.57193 & 0.00298 \\
2453925.98508 & 9.57272 & 0.00287 \\
2453925.98886 & 9.57238 & 0.00284 \\
2453925.99266 & 9.57554 & 0.00295 \\
2453925.99645 & 9.56426 & 0.00275 \\
2453926.00023 & 9.57262 & 0.00293 \\
2453926.00402 & 9.56967 & 0.00288 \\
2453926.00780 & 9.56497 & 0.00284 \\
2453926.01160 & 9.57295 & 0.00292 \\
2453926.01539 & 9.57542 & 0.00278 \\
2453926.01917 & 9.56957 & 0.00287 \\
2453926.02296 & 9.57119 & 0.00304 \\
2453926.02675 & 9.57577 & 0.00303 \\
2453926.03053 & 9.57190 & 0.00311 \\
2453926.03433 & 9.56870 & 0.00284 \\
2453926.03824 & 9.56851 & 0.00283 \\
2453926.04203 & 9.56692 & 0.00287 \\
2453926.04581 & 9.57008 & 0.00287 \\
2453926.04960 & 9.56831 & 0.00301 \\
2453926.05339 & 9.57094 & 0.00279 \\
2453926.05720 & 9.57349 & 0.00278 \\
2453926.06098 & 9.57611 & 0.00280 \\
2453926.06477 & 9.57114 & 0.00287 \\
2453926.06855 & 9.56877 & 0.00265 \\
2453926.10386 & 9.56896 & 0.00289 \\
2453926.10769 & 9.56870 & 0.00281 \\
2453926.11147 & 9.56705 & 0.00286 \\
2453926.11526 & 9.56741 & 0.00285 \\
2453926.11905 & 9.57123 & 0.00285 \\
2453926.87140 & 9.57946 & 0.00376 \\
2453926.87523 & 9.57078 & 0.00343 \\
2453926.87901 & 9.56909 & 0.00340 \\
2453926.88279 & 9.57112 & 0.00377 \\
2453926.88657 & 9.55869 & 0.00348 \\
2453926.89035 & 9.56272 & 0.00325 \\
2453926.89413 & 9.57065 & 0.00341 \\
2453926.89791 & 9.57116 & 0.00325 \\
2453926.90170 & 9.56231 & 0.00341 \\
2453926.90548 & 9.57429 & 0.00325 \\
2453926.90925 & 9.56556 & 0.00341 \\
2453926.91304 & 9.56342 & 0.00343 \\
2453926.91681 & 9.56601 & 0.00343 \\
2453926.92060 & 9.57084 & 0.00298 \\
2453926.92451 & 9.56654 & 0.00322 \\
2453926.92829 & 9.57749 & 0.00361 \\
2453926.93207 & 9.56994 & 0.00321 \\
2453926.93585 & 9.57037 & 0.00324 \\
2453926.93964 & 9.56361 & 0.00335 \\
2453926.94341 & 9.57153 & 0.00299 \\
2453926.94719 & 9.58001 & 0.00333 \\
2453926.95097 & 9.57831 & 0.00329 \\
2453926.95474 & 9.56427 & 0.00320 \\
2453926.95853 & 9.57070 & 0.00309 \\
2453926.96232 & 9.57172 & 0.00305 \\
2453926.96611 & 9.58418 & 0.00311 \\
2453926.96988 & 9.57987 & 0.00335 \\
2453926.97366 & 9.56780 & 0.00317 \\
2453926.97744 & 9.57624 & 0.00291 \\
2453926.98135 & 9.57605 & 0.00295 \\
2453926.98513 & 9.57328 & 0.00316 \\
2453926.98892 & 9.57873 & 0.00294 \\
2453926.99270 & 9.57634 & 0.00293 \\
2453926.99648 & 9.58321 & 0.00302 \\
2453927.00026 & 9.57412 & 0.00289 \\
2453927.00404 & 9.57743 & 0.00289 \\
2453927.00783 & 9.58620 & 0.00305 \\
2453927.01162 & 9.57744 & 0.00300 \\
2453927.01540 & 9.57350 & 0.00277 \\
2453927.01919 & 9.57810 & 0.00313 \\
2453927.02298 & 9.57920 & 0.00296 \\
2453927.02677 & 9.58232 & 0.00282 \\
2453927.03055 & 9.57501 & 0.00309 \\
2453927.03434 & 9.57211 & 0.00289 \\
2453927.03825 & 9.57506 & 0.00289 \\
2453927.04204 & 9.57165 & 0.00303 \\
2453927.04583 & 9.57810 & 0.00294 \\
2453927.04962 & 9.57837 & 0.00303 \\
2453927.05339 & 9.58040 & 0.00297 \\
2453927.05718 & 9.57238 & 0.00269 \\
2453927.06096 & 9.58209 & 0.00297 \\
2453927.06474 & 9.56928 & 0.00295 \\
2453927.06856 & 9.57505 & 0.00309 \\
2453927.10001 & 9.56802 & 0.00276 \\
2453927.10384 & 9.56475 & 0.00296 \\
2453927.10763 & 9.56406 & 0.00276 \\
2453927.11139 & 9.56778 & 0.00279 \\
2453927.11517 & 9.56804 & 0.00303 \\
2453927.11896 & 9.57102 & 0.00291 \\
2453927.86760 & 9.57324 & 0.00383 \\
2453927.87144 & 9.56858 & 0.00371 \\
2453927.87522 & 9.56125 & 0.00324 \\
2453927.87900 & 9.57186 & 0.00356 \\
2453927.88278 & 9.56546 & 0.00362 \\
2453927.88656 & 9.57390 & 0.00386 \\
2453927.89035 & 9.58493 & 0.00370 \\
2453927.89413 & 9.57897 & 0.00327 \\
2453927.89791 & 9.56845 & 0.00338 \\
2453927.90170 & 9.57347 & 0.00333 \\
2453927.90925 & 9.57351 & 0.00320 \\
2453927.91303 & 9.56811 & 0.00326 \\
2453927.92057 & 9.57062 & 0.00340 \\
2453927.92449 & 9.56629 & 0.00320 \\
2453927.92827 & 9.56895 & 0.00342 \\
2453927.93205 & 9.57409 & 0.00329 \\
2453927.93584 & 9.56727 & 0.00304 \\
2453927.93962 & 9.56886 & 0.00307 \\
2453927.94341 & 9.56655 & 0.00297 \\
2453927.94720 & 9.56909 & 0.00303 \\
2453927.95098 & 9.56872 & 0.00302 \\
2453927.95478 & 9.56771 & 0.00318 \\
2453927.95855 & 9.57010 & 0.00321 \\
2453927.96233 & 9.57441 & 0.00307 \\
2453927.96611 & 9.56992 & 0.00304 \\
2453927.96990 & 9.56312 & 0.00293 \\
2453927.97368 & 9.56399 & 0.00309 \\
2453927.97748 & 9.56063 & 0.00311 \\
2453927.98138 & 9.56757 & 0.00316 \\
2453927.98514 & 9.56702 & 0.00320 \\
2453927.98892 & 9.56951 & 0.00289 \\
2453927.99271 & 9.57272 & 0.00308 \\
2453927.99649 & 9.56792 & 0.00315 \\
2453928.00028 & 9.56806 & 0.00304 \\
2453928.00405 & 9.56861 & 0.00305 \\
2453928.00779 & 9.57865 & 0.00314 \\
2453928.01157 & 9.56531 & 0.00325 \\
2453928.01536 & 9.57351 & 0.00283 \\
2453928.01915 & 9.56965 & 0.00286 \\
2453928.02293 & 9.57556 & 0.00291 \\
2453928.02672 & 9.57097 & 0.00284 \\
2453928.03050 & 9.57455 & 0.00286 \\
2453928.03428 & 9.56712 & 0.00281 \\
2453928.03820 & 9.57244 & 0.00296 \\
2453928.04198 & 9.56917 & 0.00304 \\
2453928.04578 & 9.56418 & 0.00277 \\
2453928.04955 & 9.57326 & 0.00319 \\
2453928.05334 & 9.56721 & 0.00322 \\
2453928.05713 & 9.56643 & 0.00297 \\
2453928.06092 & 9.56738 & 0.00302 \\
2453928.06472 & 9.57056 & 0.00289 \\
2453928.09994 & 9.56861 & 0.00285 \\
2453928.10374 & 9.55994 & 0.00304 \\
2453928.10753 & 9.57420 & 0.00293 \\
2453928.11131 & 9.57678 & 0.00288 \\
2453928.11510 & 9.56295 & 0.00316 \\
2453928.11889 & 9.56787 & 0.00306 \\
2453928.86771 & 9.57081 & 0.00386 \\
2453928.87155 & 9.56893 & 0.00350 \\
2453928.87533 & 9.56221 & 0.00351 \\
2453928.87911 & 9.56634 & 0.00331 \\
2453928.88290 & 9.56084 & 0.00333 \\
2453928.88668 & 9.56883 & 0.00324 \\
2453928.89047 & 9.57521 & 0.00328 \\
2453928.89426 & 9.56190 & 0.00298 \\
2453928.89805 & 9.57787 & 0.00339 \\
2453928.90183 & 9.57812 & 0.00352 \\
2453928.90563 & 9.56863 & 0.00321 \\
2453928.90941 & 9.56800 & 0.00325 \\
2453928.91320 & 9.56857 & 0.00315 \\
2453928.91696 & 9.57576 & 0.00312 \\
2453928.92078 & 9.56121 & 0.00323 \\
2453928.92470 & 9.56702 & 0.00322 \\
2453928.92849 & 9.57105 & 0.00301 \\
2453928.93229 & 9.55898 & 0.00296 \\
2453928.93604 & 9.56150 & 0.00316 \\
2453928.93984 & 9.57167 & 0.00302 \\
2453928.94363 & 9.57100 & 0.00298 \\
2453928.94741 & 9.57449 & 0.00308 \\
2453928.95120 & 9.56804 & 0.00311 \\
2453928.95500 & 9.56357 & 0.00287 \\
2453928.95878 & 9.56864 & 0.00280 \\
2453928.96256 & 9.56626 & 0.00313 \\
2453928.96635 & 9.56729 & 0.00305 \\
2453928.97016 & 9.56721 & 0.00289 \\
2453928.97395 & 9.57041 & 0.00299 \\
2453928.97772 & 9.56295 & 0.00309 \\
2453928.98170 & 9.57309 & 0.00290 \\
2453928.98549 & 9.56373 & 0.00316 \\
2453928.98928 & 9.57400 & 0.00290 \\
2453928.99307 & 9.57481 & 0.00321 \\
2453928.99685 & 9.56768 & 0.00295 \\
2453929.00065 & 9.56780 & 0.00298 \\
2453929.00445 & 9.57350 & 0.00299 \\
2453929.00824 & 9.56209 & 0.00300 \\
2453929.01202 & 9.57101 & 0.00287 \\
2453929.01581 & 9.56658 & 0.00282 \\
2453929.01961 & 9.57381 & 0.00297 \\
2453929.02341 & 9.56687 & 0.00274 \\
2453929.02719 & 9.56177 & 0.00286 \\
2453929.03097 & 9.57051 & 0.00304 \\
2453929.03477 & 9.56905 & 0.00289 \\
2453929.03875 & 9.57639 & 0.00289 \\
2453929.04254 & 9.56700 & 0.00287 \\
2453929.04633 & 9.57073 & 0.00278 \\
2453929.05013 & 9.57759 & 0.00304 \\
2453929.05391 & 9.56587 & 0.00278 \\
2453929.05769 & 9.57333 & 0.00274 \\
2453929.06147 & 9.57271 & 0.00289 \\
2453929.10125 & 9.56931 & 0.00274 \\
2453929.10503 & 9.57816 & 0.00311 \\
2453929.10882 & 9.57007 & 0.00291 \\
2453929.11258 & 9.56596 & 0.00300 \\
2453929.11640 & 9.56418 & 0.00341 \\
2453929.12017 & 9.55397 & 0.00423 \\
2453929.86376 & 9.56954 & 0.00338 \\
2453929.86779 & 9.56745 & 0.00351 \\
2453929.87157 & 9.58819 & 0.00329 \\
2453929.87535 & 9.56424 & 0.00346 \\
2453929.87915 & 9.56343 & 0.00363 \\
2453929.88294 & 9.57556 & 0.00335 \\
2453929.88672 & 9.57018 & 0.00298 \\
2453929.89050 & 9.56985 & 0.00335 \\
2453929.89427 & 9.57204 & 0.00306 \\
2453929.89807 & 9.56579 & 0.00340 \\
2453929.90186 & 9.56935 & 0.00311 \\
2453929.90565 & 9.57708 & 0.00371 \\
2453929.90946 & 9.57085 & 0.00325 \\
2453929.91325 & 9.57418 & 0.00332 \\
2453929.91703 & 9.56799 & 0.00325 \\
2453929.92083 & 9.57187 & 0.00311 \\
2453929.92482 & 9.56869 & 0.00305 \\
2453929.92861 & 9.56168 & 0.00319 \\
2453929.93240 & 9.56578 & 0.00318 \\
2453929.93619 & 9.57148 & 0.00299 \\
2453929.93999 & 9.57247 & 0.00327 \\
2453929.94377 & 9.56266 & 0.00324 \\
2453929.94755 & 9.57218 & 0.00301 \\
2453929.95136 & 9.56374 & 0.00301 \\
2453929.95516 & 9.56908 & 0.00330 \\
2453929.95895 & 9.57030 & 0.00335 \\
2453929.96273 & 9.56996 & 0.00279 \\
2453929.96652 & 9.57345 & 0.00299 \\
2453929.97031 & 9.57188 & 0.00314 \\
2453929.97411 & 9.56772 & 0.00282 \\
2453929.97789 & 9.57158 & 0.00312 \\
2453929.98185 & 9.56797 & 0.00306 \\
2453929.98563 & 9.57084 & 0.00301 \\
2453929.98936 & 9.56939 & 0.00288 \\
2453929.99316 & 9.56943 & 0.00295 \\
2453929.99699 & 9.57516 & 0.00333 \\
2453930.00078 & 9.57571 & 0.00302 \\
2453930.00456 & 9.57524 & 0.00287 \\
2453930.00836 & 9.57589 & 0.00310 \\
2453930.01214 & 9.57302 & 0.00307 \\
2453930.01594 & 9.57552 & 0.00313 \\
2453930.01968 & 9.57714 & 0.00293 \\
2453930.02346 & 9.57823 & 0.00300 \\
2453930.02726 & 9.57563 & 0.00305 \\
2453930.03106 & 9.57671 & 0.00297 \\
2453930.03484 & 9.58190 & 0.00310 \\
2453930.03892 & 9.58997 & 0.00297 \\
2453930.04271 & 9.57921 & 0.00319 \\
2453930.04649 & 9.57322 & 0.00312 \\
2453930.05026 & 9.57276 & 0.00311 \\
2453930.05405 & 9.57974 & 0.00311 \\
2453930.05785 & 9.58292 & 0.00313 \\
2453930.09430 & 9.58265 & 0.00319 \\
2453930.09831 & 9.58297 & 0.00321 \\
2453930.10209 & 9.58008 & 0.00303 \\
2453930.10587 & 9.57836 & 0.00308 \\
2453930.10967 & 9.56504 & 0.00306 \\
2453930.11344 & 9.57730 & 0.00310 \\
2453930.11723 & 9.56995 & 0.00301 \\
2453930.12101 & 9.56744 & 0.00324 \\
2453930.86009 & 9.56670 & 0.00333 \\
2453930.86392 & 9.57707 & 0.00321 \\
2453930.86789 & 9.57487 & 0.00328 \\
2453930.87171 & 9.57158 & 0.00340 \\
2453930.87551 & 9.56573 & 0.00327 \\
2453930.87931 & 9.58061 & 0.00317 \\
2453930.88310 & 9.57701 & 0.00327 \\
2453930.88688 & 9.56596 & 0.00293 \\
2453930.89072 & 9.56640 & 0.00325 \\
2453930.89451 & 9.57161 & 0.00302 \\
2453930.89831 & 9.57128 & 0.00306 \\
2453930.90210 & 9.56637 & 0.00299 \\
2453930.90589 & 9.57563 & 0.00309 \\
2453930.90971 & 9.57124 & 0.00303 \\
2453930.91348 & 9.56716 & 0.00268 \\
2453930.91736 & 9.57748 & 0.00312 \\
2453930.92116 & 9.57443 & 0.00328 \\
2453930.92516 & 9.57415 & 0.00323 \\
2453930.92895 & 9.57196 & 0.00328 \\
2453930.93273 & 9.57235 & 0.00304 \\
2453930.93654 & 9.56584 & 0.00296 \\
2453930.94032 & 9.57014 & 0.00293 \\
2453930.94409 & 9.57264 & 0.00319 \\
2453930.94787 & 9.57607 & 0.00316 \\
2453930.95166 & 9.57143 & 0.00321 \\
2453930.95549 & 9.56367 & 0.00296 \\
2453930.95928 & 9.56568 & 0.00297 \\
2453930.96307 & 9.56807 & 0.00283 \\
2453930.96690 & 9.57456 & 0.00291 \\
2453930.97070 & 9.57849 & 0.00309 \\
2453930.97450 & 9.56917 & 0.00291 \\
2453930.97829 & 9.56490 & 0.00331 \\
2453930.98227 & 9.56735 & 0.00299 \\
2453930.98607 & 9.56151 & 0.00285 \\
2453930.98985 & 9.56946 & 0.00292 \\
2453930.99363 & 9.56881 & 0.00304 \\
2453930.99742 & 9.56744 & 0.00295 \\
2453931.00121 & 9.57453 & 0.00296 \\
2453931.00500 & 9.56295 & 0.00281 \\
2453931.00880 & 9.57120 & 0.00290 \\
2453931.01256 & 9.56477 & 0.00298 \\
2453931.01635 & 9.57231 & 0.00279 \\
2453931.02013 & 9.56585 & 0.00290 \\
2453931.02393 & 9.56925 & 0.00290 \\
2453931.02775 & 9.57400 & 0.00301 \\
2453931.03162 & 9.56587 & 0.00287 \\
2453931.03542 & 9.57447 & 0.00291 \\
2453931.03935 & 9.56523 & 0.00292 \\
2453931.04315 & 9.57598 & 0.00296 \\
2453931.04692 & 9.57409 & 0.00276 \\
2453931.05070 & 9.57599 & 0.00284 \\
2453931.05450 & 9.56414 & 0.00291 \\
2453931.05832 & 9.57197 & 0.00301 \\
2453931.10329 & 9.57325 & 0.00596 \\
2453931.10710 & 9.56829 & 0.00313 \\
2453931.11089 & 9.57762 & 0.00282 \\
2453931.11467 & 9.56504 & 0.00297 \\
2453931.11845 & 9.56175 & 0.00292 \\
2453931.12222 & 9.56852 & 0.00309 \\
2453931.85946 & 9.57341 & 0.00323 \\
2453931.86329 & 9.57226 & 0.00329 \\
2453931.86720 & 9.55792 & 0.00316 \\
2453931.87099 & 9.55754 & 0.00331 \\
2453931.87477 & 9.57253 & 0.00302 \\
2453931.87856 & 9.57316 & 0.00327 \\
2453931.88234 & 9.56906 & 0.00321 \\
2453931.88612 & 9.57694 & 0.00303 \\
2453931.88990 & 9.57877 & 0.00304 \\
2453931.89369 & 9.57412 & 0.00319 \\
2453931.89747 & 9.57413 & 0.00320 \\
2453931.90124 & 9.57239 & 0.00287 \\
2453931.90503 & 9.57289 & 0.00311 \\
2453931.90880 & 9.56839 & 0.00317 \\
2453931.91258 & 9.56609 & 0.00315 \\
2453931.91636 & 9.56721 & 0.00314 \\
2453931.92015 & 9.56126 & 0.00279 \\
2453931.92406 & 9.56985 & 0.00318 \\
2453931.92784 & 9.57216 & 0.00289 \\
2453931.93161 & 9.57214 & 0.00298 \\
2453931.93539 & 9.57745 & 0.00323 \\
2453931.93917 & 9.55871 & 0.00309 \\
2453931.94295 & 9.56656 & 0.00292 \\
2453931.94673 & 9.56429 & 0.00310 \\
2453931.95052 & 9.56638 & 0.00312 \\
2453931.95430 & 9.57417 & 0.00311 \\
2453931.95809 & 9.56724 & 0.00282 \\
2453931.96187 & 9.56809 & 0.00303 \\
2453931.96566 & 9.56859 & 0.00277 \\
2453931.96943 & 9.57100 & 0.00300 \\
2453931.97321 & 9.57283 & 0.00300 \\
2453931.97699 & 9.57134 & 0.00296 \\
2453931.98090 & 9.56591 & 0.00297 \\
2453931.98469 & 9.57383 & 0.00303 \\
2453931.98847 & 9.56652 & 0.00293 \\
2453931.99226 & 9.56550 & 0.00317 \\
2453931.99605 & 9.56930 & 0.00292 \\
2453931.99983 & 9.57051 & 0.00301 \\
2453932.00361 & 9.56098 & 0.00294 \\
2453932.00738 & 9.57148 & 0.00271 \\
2453932.01116 & 9.56356 & 0.00307 \\
2453932.01493 & 9.56489 & 0.00305 \\
2453932.01872 & 9.55826 & 0.00283 \\
2453932.02250 & 9.57475 & 0.00288 \\
2453932.02627 & 9.57054 & 0.00293 \\
2453932.03006 & 9.57059 & 0.00277 \\
2453932.03384 & 9.56973 & 0.00281 \\
2453932.03775 & 9.56950 & 0.00305 \\
2453932.04153 & 9.56739 & 0.00288 \\
2453932.04532 & 9.56749 & 0.00295 \\
2453932.04910 & 9.56572 & 0.00295 \\
2453932.05287 & 9.56969 & 0.00309 \\
2453932.08784 & 9.57377 & 0.00288 \\
2453932.09165 & 9.56534 & 0.00301 \\
2453932.09558 & 9.57366 & 0.00296 \\
2453932.09937 & 9.56503 & 0.00286 \\
2453932.10315 & 9.56716 & 0.00292 \\
2453932.10693 & 9.56664 & 0.00280 \\
2453932.11071 & 9.56757 & 0.00294 \\
2453932.11447 & 9.56829 & 0.00291 \\
2453932.11825 & 9.57484 & 0.00298 \\
2453932.12203 & 9.56485 & 0.00301 \\
2453932.85561 & 9.56112 & 0.00294 \\
2453932.85944 & 9.57414 & 0.00301 \\
2453932.86323 & 9.57249 & 0.00319 \\
2453932.86714 & 9.57826 & 0.00316 \\
2453932.87092 & 9.56922 & 0.00310 \\
2453932.87472 & 9.56979 & 0.00288 \\
2453932.87850 & 9.57236 & 0.00302 \\
2453932.88228 & 9.57504 & 0.00312 \\
2453932.88606 & 9.57417 & 0.00321 \\
2453932.88984 & 9.57011 & 0.00314 \\
2453932.89362 & 9.56871 & 0.00293 \\
2453932.89741 & 9.56863 & 0.00323 \\
2453932.90120 & 9.57415 & 0.00298 \\
2453932.90498 & 9.57491 & 0.00307 \\
2453932.90877 & 9.56293 & 0.00295 \\
2453932.91255 & 9.57360 & 0.00307 \\
2453932.91634 & 9.57248 & 0.00328 \\
2453932.92013 & 9.57469 & 0.00276 \\
2453932.92404 & 9.56904 & 0.00289 \\
2453932.92782 & 9.56841 & 0.00295 \\
2453932.93537 & 9.57287 & 0.00289 \\
2453932.93915 & 9.57812 & 0.00315 \\
2453932.94294 & 9.56920 & 0.00290 \\
2453932.94671 & 9.57017 & 0.00296 \\
2453932.95051 & 9.57690 & 0.00290 \\
2453932.95429 & 9.56886 & 0.00293 \\
2453932.95808 & 9.56873 & 0.00311 \\
2453932.96187 & 9.56483 & 0.00265 \\
2453932.96564 & 9.56526 & 0.00304 \\
2453932.96942 & 9.57206 & 0.00285 \\
2453932.97321 & 9.57510 & 0.00286 \\
2453932.97699 & 9.57087 & 0.00293 \\
2453932.98090 & 9.56635 & 0.00299 \\
2453932.98469 & 9.56838 & 0.00281 \\
2453932.98848 & 9.56620 & 0.00268 \\
2453932.99226 & 9.57270 & 0.00304 \\
2453932.99604 & 9.57658 & 0.00294 \\
2453933.00360 & 9.56578 & 0.00265 \\
2453933.00737 & 9.56720 & 0.00270 \\
2453933.01116 & 9.57851 & 0.00266 \\
2453933.01495 & 9.57428 & 0.00297 \\
2453933.01875 & 9.58163 & 0.00276 \\
2453933.02253 & 9.57146 & 0.00301 \\
2453933.02631 & 9.57025 & 0.00272 \\
2453933.03011 & 9.57389 & 0.00289 \\
2453933.03390 & 9.57616 & 0.00292 \\
2453933.03781 & 9.56915 & 0.00270 \\
2453933.04159 & 9.56645 & 0.00293 \\
2453933.04538 & 9.56817 & 0.00292 \\
2453933.04917 & 9.57300 & 0.00279 \\
2453933.05295 & 9.57307 & 0.00276 \\
2453933.08419 & 9.57420 & 0.00291 \\
2453933.08798 & 9.57114 & 0.00279 \\
2453933.09182 & 9.56975 & 0.00294 \\
2453933.09574 & 9.57769 & 0.00285 \\
2453933.09952 & 9.57674 & 0.00282 \\
2453933.10330 & 9.58455 & 0.00270 \\
2453933.10708 & 9.57625 & 0.00289 \\
2453933.11087 & 9.57338 & 0.00273 \\
2453933.11465 & 9.58110 & 0.00270 \\
2453933.11843 & 9.58479 & 0.00275 \\
2453933.12221 & 9.58301 & 0.00298 \\
2453933.85179 & 9.56979 & 0.00313 \\
2453933.85561 & 9.56603 & 0.00314 \\
2453933.85940 & 9.56767 & 0.00306 \\
2453933.86318 & 9.57065 & 0.00312 \\
2453933.86709 & 9.56737 & 0.00325 \\
2453933.87088 & 9.56986 & 0.00317 \\
2453933.87466 & 9.56977 & 0.00286 \\
2453933.87844 & 9.56620 & 0.00306 \\
2453933.88223 & 9.57450 & 0.00306 \\
2453933.88601 & 9.57253 & 0.00303 \\
2453933.88980 & 9.56545 & 0.00286 \\
2453933.89357 & 9.57692 & 0.00276 \\
2453933.89736 & 9.56949 & 0.00312 \\
2453933.90114 & 9.57273 & 0.00308 \\
2453933.90493 & 9.56618 & 0.00288 \\
2453933.90872 & 9.57031 & 0.00310 \\
2453933.91250 & 9.56747 & 0.00277 \\
2453933.91629 & 9.56201 & 0.00294 \\
2453933.92007 & 9.57633 & 0.00313 \\
2453933.92399 & 9.56812 & 0.00293 \\
2453933.92778 & 9.56291 & 0.00305 \\
2453933.93156 & 9.56925 & 0.00306 \\
2453933.93535 & 9.57083 & 0.00314 \\
2453933.93914 & 9.57040 & 0.00291 \\
2453933.94292 & 9.57082 & 0.00296 \\
2453933.94671 & 9.56415 & 0.00311 \\
2453933.95049 & 9.56542 & 0.00280 \\
2453933.95428 & 9.57189 & 0.00303 \\
2453933.95806 & 9.55811 & 0.00295 \\
2453933.96186 & 9.56889 & 0.00286 \\
2453933.96564 & 9.58164 & 0.00325 \\
2453933.96942 & 9.57099 & 0.00287 \\
2453933.97322 & 9.56461 & 0.00304 \\
2453933.97700 & 9.56359 & 0.00282 \\
2453933.98091 & 9.56502 & 0.00301 \\
2453933.98470 & 9.57000 & 0.00313 \\
2453933.98848 & 9.57125 & 0.00307 \\
2453933.99227 & 9.56590 & 0.00292 \\
2453933.99604 & 9.57014 & 0.00292 \\
2453933.99983 & 9.56905 & 0.00304 \\
2453934.00361 & 9.56456 & 0.00286 \\
2453934.00739 & 9.56807 & 0.00272 \\
2453934.01117 & 9.56697 & 0.00276 \\
2453934.01496 & 9.56350 & 0.00294 \\
2453934.01874 & 9.57206 & 0.00293 \\
2453934.02252 & 9.56995 & 0.00282 \\
2453934.02630 & 9.57633 & 0.00284 \\
2453934.03009 & 9.56758 & 0.00299 \\
2453934.03387 & 9.57036 & 0.00285 \\
2453934.03778 & 9.55918 & 0.00268 \\
2453934.04157 & 9.56549 & 0.00291 \\
2453934.04537 & 9.56997 & 0.00294 \\
2453934.04916 & 9.56363 & 0.00268 \\
2453934.08415 & 9.56640 & 0.00281 \\
2453934.08793 & 9.57424 & 0.00299 \\
2453934.09178 & 9.57447 & 0.00273 \\
2453934.09571 & 9.56771 & 0.00272 \\
2453934.09947 & 9.56679 & 0.00271 \\
2453934.10329 & 9.57047 & 0.00270 \\
2453934.10707 & 9.56991 & 0.00287 \\
2453934.11086 & 9.56565 & 0.00267 \\
2453934.11463 & 9.57314 & 0.00297 \\
2453934.11841 & 9.57158 & 0.00268 \\
2453934.12220 & 9.56510 & 0.00294 \\
2452978.69841 & 9.56562 & 0.00339 \\
2452978.70229 & 9.57650 & 0.00305 \\
2452978.70606 & 9.56973 & 0.00304 \\
2452978.70994 & 9.57758 & 0.00321 \\
2452978.71381 & 9.58096 & 0.00309 \\
2452978.71760 & 9.57422 & 0.00310 \\
2452978.72148 & 9.57407 & 0.00331 \\
2452978.72536 & 9.57336 & 0.00279 \\
2452978.72914 & 9.56637 & 0.00326 \\
2452978.73302 & 9.56766 & 0.00301 \\
2452978.73691 & 9.57674 & 0.00305 \\
2452978.74069 & 9.57368 & 0.00333 \\
2452978.74456 & 9.56583 & 0.00292 \\
2452978.74843 & 9.57188 & 0.00309 \\
2452978.75224 & 9.56966 & 0.00321 \\
2452978.75610 & 9.56329 & 0.00326 \\
2452978.75998 & 9.56966 & 0.00292 \\
2452978.76377 & 9.57662 & 0.00357 \\
2452978.76766 & 9.56653 & 0.00315 \\
2452978.77533 & 9.57489 & 0.00357 \\
2452978.77921 & 9.56944 & 0.00302 \\
2452978.78308 & 9.56616 & 0.00319 \\
2452978.78686 & 9.57096 & 0.00347 \\
2452978.79074 & 9.57323 & 0.00312 \\
2452978.79466 & 9.57018 & 0.00295 \\
2452978.79846 & 9.56493 & 0.00317 \\
2452978.80624 & 9.57220 & 0.00288 \\
2452978.81000 & 9.56913 & 0.00340 \\
2452978.81394 & 9.56917 & 0.00341 \\
2452978.81782 & 9.57588 & 0.00326 \\
2452978.82161 & 9.57189 & 0.00328 \\
2452978.82554 & 9.57060 & 0.00317 \\
2452978.82946 & 9.57917 & 0.00309 \\
2452978.83325 & 9.56895 & 0.00325 \\
2452978.83713 & 9.56966 & 0.00340 \\
2452978.84100 & 9.56773 & 0.00322 \\
2452978.84481 & 9.56692 & 0.00326 \\
2452978.84869 & 9.56920 & 0.00325 \\
2452978.85258 & 9.57092 & 0.00327 \\
2452978.85637 & 9.56540 & 0.00323 \\
2452978.86025 & 9.57441 & 0.00350 \\
2452978.86418 & 9.56773 & 0.00349 \\
\enddata
\label{tab:hatnet}
\tablecomments{
column (1): Barycentric Julian Day, \\
column (2): Best detrended HATNet magnitude, \\
column (3): Estimated error in the best magnitude.}
\tablecomments{
Table 9 is presented in its entirety in the electronic edition
of the Astrophysical Journal. A portion is shown here for guidance
regarding its form and content.} \\
\end{deluxetable}

